Multiple zeta values and their q-analogues

We explore the theory of multiple zeta values (MZVs) and some of their $q$-generalisations. Multiple zeta values are numerical quantities that satisfy several combinatorial relations over the rationals. These relations include two multiplicative relations, which arise naturally from comparison of the MZVs with an underlying algebraic structure. We generalise these concepts by introducing the parameter $q$ in such a way that as $q\to 1^-$ we return to the ordinary MZVs. Our special interest lies in two $q$-models recently introduced by H. Bachmann. He further conjectures that the $\mathbb{Q}$-spaces generated by these $q$-generalisations coincide. In this thesis we establish a particular case of Bachmann's conjecture.

==> Derivative.tex <==
\begin{theorem}
\label{invarianceofd}
The operator $d=q\frac{d}{dq}$ satisfies
\begin{equation*}
    d\colon \fil_{k,l}^{W,L}(\MD)\to \fil_{k+2,l+1}^{W,L}(\MD).
\end{equation*}
\end{theorem}
We introduce the generating functions of the mono-brackets
\begin{equation*}
    T(X_1,\dots,X_l)=\sum_{s_1,\dots,s_l>0}[s_1,\dots,s_l]X_1^{s_1-1}\cdots X_l^{s_l-1}.
\end{equation*}
We can rewrite these generating functions as stated in the next lemma.

\begin{lemma}
\label{generatingmono}
We have
\begin{equation*}
    T(X_1,\dots,X_l)=\sum_{n_1,\dots,n_l>0}\prod_{j=1}^l\frac{e^{n_jX_j}q^{n_1+\dots+n_j}}{1-q^{n_1+\dots+n_j}}.
\end{equation*}
\end{lemma}
\begin{proof}
By definition we have
\begin{align*}
    T(X_1,\dots,X_l)&=\sum_{s_1,\dots,s_l>0}\left(\sum_{\substack{u_1>\cdots>u_l>0\\n_1,\dots,n_1>0}}\frac{n_1^{s_1-1}\cdots n_l^{s_l-1}}{(s_1-1)!\cdots(s_l-1)!}q^{u_1n_1+\dots+u_ln_l}\right)X_1^{s_1-1}\cdots X_l^{s_l-1}\\
    &=\sum_{s_1,\dots,s_l\geq0}\left(\sum_{\substack{u_1>\cdots>u_l>0\\n_1,\dots,n_1>0}}\frac{n_1^{s_1}\cdots n_l^{s_l}}{s_1!\cdots s_l!}q^{u_1n_1+\dots+u_ln_l}\right)X_1^{s_1}\cdots X_l^{s_l}.
\end{align*}
The statement $u_1>u_2>\dots>u_{l-1}>u_l>0$ means that for every $1\leq k\leq l-1$ there exists an integer $v_k$ such that $u_k=u_{k+1}+v_k$. When we set $v_l=u_l$, we get
\begin{align*}
    u_l&=v_l\\
    u_{l-1}&=u_l+v_{l-1}=v_l+v_{l-1}\\
    u_{l-2}&=u_{l-1}+v_{l-2}=v_l+v_{l-1}+v_{l-2}\\
    \vdots\\
    u_1&=u_2+v_1=v_l+\dots+v_2+v_1.
\end{align*}
With this transformation, our generating function becomes
\begin{align*}
    T(X_1,\dots,X_l)&=\sum_{s_1,\dots,s_l\geq0}\left(\sum_{\substack{v_1,\cdots,v_l>0\\n_1,\dots,n_1>0}}\frac{n_1^{s_1}\cdots n_l^{s_l}}{s_1!\cdots s_l!}q^{(v_1+\dots+v_l)n_1+(v_2
    +\dots+v_l)n_2+\dots+v_ln_l}\right)X_1^{s_1}\cdots X_l^{s_l}\\
    &=\sum_{s_1,\dots,s_l\geq0}\left(\sum_{\substack{v_1,\cdots,v_l>0\\n_1,\dots,n_1>0}}\frac{n_1^{s_1}\cdots n_l^{s_l}}{s_1!\cdots s_l!}q^{v_l(n_1+\dots+n_l)+v_{l-1}(n_1+\dots+n_{l-1})+\dots+v_1n_1}\right)X_1^{s_1}\cdots X_l^{s_l}\\
    &=\sum_{n_1,\dots,n_l\geq0}\prod_{j=1}^l\sum_{s_j\geq0}\frac{n_j^{s_j}}{s_j!}X^{s_j}\sum_{v_j>0}q^{v_j(n_1+\dots+n_j)}\\
    &=\sum_{n_1,\dots,n_l\geq0}\prod_{j=1}^le^{n_jX_j}\frac{q^{n_1+\dots+n_j}}{1-q^{n_1+\dots+n_j}}.
    \end{align*}
This completes the proof.
\end{proof}




\begin{proof}[Proof (Theorem \ref{invarianceofd})]
Using Lemma \ref{generatingmono}, we are able to calculate
\begin{align*}
    T(X)\cdot T(X_1,\dots,X_l)&=\sum_{m,n_1,\dots,n_l>0}e^{mX+n_1X_1+\dots+n_lX_l}\frac{q^m}{1-q^m}\prod_{j=1}^l \frac{q^{n_1+\dots+n_j}}{1-q^{n_1+\dots+n_j}}
\end{align*}
The RHS can be split according to the cases $n_1+\dots+n_k>m>n_1+\dots+n_{k-1}$ and $m=n_1+\dots+n_k$ for $1\leq k\leq l$, and when $m>n_1+\dots+n_l$.\\

First, consider the case when $m>n_1+\dots+n_l$. Then with $M=m-n_1-\dots-n_l$ we have
\begin{align*}
    \Sigma_1&\coloneqq \sum_{\substack{m,n_1,\dots,n_l>0\\m>n_1+\dots+n_l}}e^{mX+n_1X_1+\dots+n_lX_l}\frac{q^m}{1-q^m}\prod_{j=1}^l \frac{q^{n_1+\dots+n_j}}{1-q^{n_1+\dots+n_j}}\\
    &=\sum_{n_1,\dots,n_l,M>0}e^{(n_1+\dots+n_l+M)X+n_1X_1+\dots+n_lX_l}\frac{q^{n_1+\dots+n_l+M}}{1-q^{n_1+\dots+n_l+M}}\prod_{j=1}^l \frac{q^{n_1+\dots+n_j}}{1-q^{n_1+\dots+n_j}}\\
    &=T(X_1+X,\dots,X_l+X,X).
\end{align*}
Now consider the cases when $n_1+\dots+n_k>m>n_1+\dots+n_{k-1}$ for some $1\leq k\leq l$. Then there exist some integers $M,N$ such that $m=n_1+\dots+n_{k-1}+M$ and $n_1+\dots+n_k=m+N$. When we apply these transformations we see that
\begin{align*}
    mX+n_1X_1+\dots+n_lX_l&=(n_1+\dots+n_{k-1}+M)X+n_1X_1+\dots+n_{k-1}X_{k-1}\\
    &\qquad+(M+N)X_k+n_{k+1}X_{k+1}+\dots+n_lX_l\\
    &=n_1(X_1+X)+\dots+n_{k-1}(X_{k-1}+X)+M(X_k+X)\\
    &\qquad+NX_k+n_{k+1}X_{k+1}+\dots+n_lX_l,
\end{align*}
that $q^m=q^{n_1+\dots+n_{k-1}+M}$ and finally, that 
\begin{equation*}
    q^{n_1+\dots+n_{k-1}+n_k+n_{k+1}+\dots+n_i}=q^{n_1+\dots+n_{k-1}+M+N+n_{k+1}+\dots+n_i}
\end{equation*}
for $i\geq k+1$.

Combining these parts give us
\begin{align*}
    \Sigma_2&\coloneqq\sum_{k=1}^l \sum_{\substack{m,n_1,\dots,n_l>0\\m>n_1+\dots+n_{k-1}\\m<n_1+\dots+n_{k}}}e^{mX+n_1X_1+\dots+n_lX_l}\frac{q^m}{1-q^m}\prod_{j=1}^l \frac{q^{n_1+\dots+n_k}}{1-q^{n_1+\dots+n_k}}.\\
    &=T(X_1+X,\dots,X_k+X,X_{k},\dots,X_l).
\end{align*}

Finally, consider the cases where $m=n_1+\dots+n_k$ for some $1\leq k\leq l$. 
Using the equation $(\frac{q^m}{1-q^m})^2=\frac{q^m}{(1-q^m)^2}-\frac{q^m}{1-q^m}$ we get
\begin{align*}
    \Sigma_3&\coloneqq\sum_{k=1}^l \sum_{\substack{m,n_1,\dots,n_l>0\\m=n_1+\dots+n_{k}}}e^{mX+n_1X_1+\dots+n_lX_l}\frac{q^m}{1-q^m}\prod_{j=1}^l \frac{q^{n_1+\dots+n_k}}{1-q^{n_1+\dots+n_k}}\\
    &=\sum_{k=1}^l \sum_{n_1,\dots,n_l>0}e^{n_1(X+X_1)+\dots+n_k(X+X_k)+n_{k+1}X_{k+1}+\dots+n_lX_l}\prod_{j=1}^l\left(\frac{q^{n_1+\dots+n_j}}{1-q^{n_1+\dots+n_j}}\right)^{1+\delta_{k,j}}\\
    &=\sum_{k=1}^l \sum_{n_1,\dots,n_l>0}e^{n_1(X+X_1)+\dots+n_k(X+X_k)+n_{k+1}X_{k+1}+\dots+n_lX_l}\prod_{j=1}^l\frac{q^{n_1+\dots+n_j}}{(1-q^{n_1+\dots+n_j})^{1+\delta_{k,j}}}\\
    &\qquad-\sum_{k=1}^lT(X_1+X,\dots,X_{k}+X,X_{k+1},\dots,X_l)\\
    &\eqqcolon R_l+\Sigma_4.
\end{align*}
Define the operator $D(f)=\restr{\left(\frac{d}{dX}f\right)}{X=0}$. We claim that $D(R_l)=dT(X_1,\dots,X_l)$. Namely, we have
\begin{align*}
    dT(X_1,\dots,X_l)&=\sum_{n_1,\dots,n_l>0}q\frac{d}{dq}\left(\prod_{j=1}^le^{n_jX_j}\frac{q^{n_1+\dots+n_j}}{1-q^{n_1+\dots+n_j}}\right)\\
    &=\sum_{n_1,\dots,n_l>0}\sum_{k=1}^l(n_1+\dots+n_k)\prod_{j=1}^le^{n_jX_j}\frac{q^{n_1+\dots+n_j}}{(1-q^{n_1+\dots+n_j})^{\delta_{i,j}}}\\
    &=\sum_{k=1}^l\sum_{n_1,\dots,n_l>0}(n_1+\dots+n_k)e^{n_1X_1+\dots+n_lX_l}\prod_{j=1}^l\frac{q^{n_1+\dots+n_j}}{(1-q^{n_1+\dots+n_j})^{1+\delta_{k,j}}}\\
    &=D(R_l),
\end{align*}
where we used the equation
\begin{equation*}
    q\frac{d}{dq}\left(\frac{q^m}{1-q^m}\right)=\frac{mq^m}{(1-q^m)^2}.
\end{equation*}
This means that if we apply $D$ to the equation
\begin{equation*}
    T(X)\cdot T(X_1,\dots,X_l)=\Sigma_1+\Sigma_2+R_l+\Sigma_4,
\end{equation*}
the LHS becomes $[2]T(X_1,\dots,X_l)$. For the RHS, note that the terms in $D(\Sigma_1+\Sigma_2+\Sigma_4)$ are again linear combinations of terms of the form $T(W_1,\dots,W_r)$. Finally, because $D(R_l)=dT(X_1,\dots,X_l)$ we can write $dT(X_1,\dots,X_l)$ as a linear combination of generating functions. This means that, by looking at the individual coefficients of both sides of the equation, we see that $d$ maps $\fil_{k,l}^{W,L}(\MD)$ to $\fil_{k+2,l+1}^{W,L}(\MD)$.
\end{proof}

==> DimKer.tex <==
\section{Kernels}


Define the matrices
\begin{align*}
    U(S,R)&\coloneqq
    \begin{cases}\begin{pmatrix}
&&&&&&\\
&&&P_{S-1}\otimes Q_{R+1}+(P_{S-1}\otimes Q_{R+1})^{\rho}&&&\\
&&&&&&\\
\hline&&&\vline&&&\\
&&&I\quad\qquad\qquad\ \ \vline\quad\qquad\qquad I^\rho&&&\\
&&&\vline&&&
\end{pmatrix}&\text{ if either }S\text{ or }R\text{ is odd}\\
\begin{pmatrix}
&&&&&&\\
&&&P_{S-1}\otimes Q_{R+1}+(P_{S-1}\otimes Q_{R+1})^{\rho}&&&\\
&&&&&&\\
\hline&&&\vline \quad \vline&&&\\
&&&I\quad\qquad\qquad\ \ \vline\ 0\ \vline\quad\qquad\qquad I^\rho&&&\\
&&&\vline \quad \vline&&&\\
\hline&&& 0\quad\qquad\qquad\ \  1\  \quad\qquad\qquad0 &&&
\end{pmatrix}&\text{ if both }S\text{ and }R\text{ are even} 
\end{cases},\\
\intertext{and (!!de matrix van $S,R$ even is lelijk, verbeter hem!!)}
    T(S,R)&\coloneqq P_{S-1}\otimes Q_{R+1}-(P_{S-1}\otimes Q_{R+1})^{\rho\sigma}.
\end{align*}
They represent the linear system induced by the shuffle- and stuffle-product $\begin{bmatrix}j\\k\end{bmatrix}\cdot\begin{bmatrix}S-j\\R-k\end{bmatrix}$, and its reduced version, respectively.
For weight $S+R$ odd, we have shown that both matrices are full in rank. However, for even weight, computer calculations show that this is (almost) never the case. The dimension of the kernel of either matrix represents the lack of relations between length $l=2$ bi-brackets. The table below shows the dimensions of $\ker U(S,R)$.

\begin{table}[H]
\begin{tabular}{l|lllllllllllllllllllll}
S\textbackslash{}R & 0 & 1 & 2 & 3 & 4 & 5  & 6  & 7  & 8  & 9  & 10 & 11 & 12 & 13 & 14 & 15 & 16  & 17 & 18 & 19      \\ \hline
2                  & 0 & 0 & 0 & 0 & 0  & 0  & 1  & 0  & 1  & 0  & 1  & 0  & 2  & 0  & 2  & 0  & 2  & 0  & 3  & 0       \\
3                  & 0 & 1 & 0 & 1 & 0  & 2  & 0  & 3  & 0  & 3  & 0  & 4  & 0  & 5  & 0  & 5  & 0  & 6  & 0  & 7       \\
4                  & 0 & 0 & 1 & 0 & 2  & 0  & 3  & 0  & 4  & 0  & 5  & 0  & 6  & 0  & 7  & 0  & 8  & 0  & 9  & 0       \\
5                  & 0 & 1 & 0 & 3 & 0  & 4  & 0  & 5  & 0  & 7  & 0  & 8  & 0  & 9  & 0  & 11 & 0  & 12 & 0  & 13      \\
6                  & 0 & 0 & 2 & 0 & 4  & 0  & 5  & 0  & 7  & 0  & 9  & 0  & 10 & 0  & 12 & 0  & 14 & 0  & 15 & 0       \\
7                  & 0 & 2 & 0 & 4 & 0  & 6  & 0  & 8  & 0  & 10 & 0  & 12 & 0  & 14 & 0  & 16 & 0  & 18 & 0  & 20      \\
8                  & 1 & 0 & 3 & 0 & 5  & 0  & 8  & 0  & 10 & 0  & 12 & 0  & 15 & 0  & 17 & 0  & 19 & 0  & 22 & 0       \\
9                  & 0 & 3 & 0 & 5 & 0  & 8  & 0  & 11 & 0  & 13 & 0  & 16 & 0  & 19 & 0  & 21 & 0  & 24 & 0  & 27      \\
10                 & 1 & 0 & 4 & 0 & 7  & 0  & 10 & 0  & 13 & 0  & 16 & 0  & 19 & 0  & 22 & 0  & 25 & 0  & 28 & 0       \\
11                 & 0 & 3 & 0 & 7 & 0  & 10 & 0  & 13 & 0  & 17 & 0  & 20 & 0  & 23 & 0  & 27 & 0  & 30 & 0  & 33      \\
12                 & 1 & 0 & 5 & 0 & 9  & 0  & 12 & 0  & 16 & 0  & 20 & 0  & 23 & 0  & 27 & 0  & 31 & 0  & 34 & 0       \\
13                 & 0 & 4 & 0 & 8 & 0  & 12 & 0  & 15 & 0  & 20 & 0  & 24 & 0  & 28 & 0  & 32 & 0  & 36 & 0  & 40      \\
14                 & 2 & 0 & 6 & 0 & 10 & 0  & 15 & 0  & 19 & 0  & 23 & 0  & 28 & 0  & 32 & 0  & 36 & 0  & 41 & 0       
\end{tabular}
\caption{$\dim(\ker U(S,R))$.}
\label{dimkermetnullenU}
\end{table}
\clearpage
If we ignore the cases where $S+R$ is odd, the table reduces to the following table.
\setlength\tabcolsep{3.5pt}
\begin{table}[H]
\begin{tabular}{l|lllllllllllllllllllllllll}
S=2  & 0& 0& 0& 1 & 1 & 1 & 2 & 2 & 2 & 3 & 3& 3& 4& 4& 4  & 5  & 5  & 5  & 6  & 6  & 6  & 7  & 7  & 7  & 8\\
3  & 1& 1& 2& 3 & 3 & 4 & 5 & 5 & 6 & 7 & 7& 8& 9& 9& 10 & 11 & 11 & 12 & 13 & 13 & 14 & 15 & 15 & 16 & 17 \\
4  & 0& 1& 2& 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 \\
5  & 1& 3& 4& 5 & 7 & 8 & 9 & 11 & 12 & 13 & 15 & 16 & 17 & 19 & 20 & 21 & 23 & 24 & 25 & 27 & 28 & 29 & 31 & 32 & 33 \\
6  & 0& 2& 4& 5 & 7 & 9 & 10 & 12 & 14 & 15 & 17 & 19 & 20 & 22 & 24 & 25 & 27 & 29 & 30 & 32 & 34 & 35 & 37 & 39 & 40 \\
7  & 2& 4& 6& 8 & 10 & 12 & 14 & 16 & 18 & 20 & 22 & 24 & 26 & 28 & 30 & 32 & 34 & 36 & 38 & 40 & 42 & 44 & 46 & 48 & 50 \\
8  & 1& 3& 5& 8 & 10 & 12 & 15 & 17 & 19 & 22 & 24 & 26 & 29 & 31 & 33 & 36 & 38 & 40 & 43 & 45 & 47 & 50 & 52 & 54 & 57 \\
9  & 3& 5& 8& 11 & 13 & 16 & 19 & 21 & 24 & 27 & 29 & 32 & 35 & 37 & 40 & 43 & 45 & 48 & 51 & 53 & 56 & 59 & 61 & 64 & 67 \\
10 & 1& 4& 7& 10 & 13 & 16 & 19 & 22 & 25 & 28 & 31 & 34 & 37 & 40 & 43 & 46 & 49 & 52 & 55 & 58 & 61 & 64 & 67 & 70 & 73 \\
11 & 3& 7& 10& 13 & 17 & 20 & 23 & 27 & 30 & 33 & 37 & 40 & 43 & 47 & 50 & 53 & 57 & 60 & 63 & 67 & 70 & 73 & 77 & 80 & 83 \\
12 & 1& 5& 9& 12 & 16 & 20 & 23 & 27 & 31 & 34 & 38 & 42 & 45 & 49 & 53 & 56 & 60 & 64 & 67 & 71 & 75 & 78 & 82 & 86 & 89 \\
13 & 4& 8& 12& 16 & 20 & 24 & 28 & 32 & 36 & 40 & 44 & 48 & 52 & 56 & 60 & 64 & 68 & 72 & 76 & 80 & 84 & 88 & 92 & 96 & 100 \\
14 & 2& 6& 10& 15 & 19 & 23 & 28 & 32 & 36 & 41 & 45 & 49 & 54 & 58 & 62 & 67 & 71 & 75 & 80 & 84 & 88 & 93 & 97 & 101 & 106 
\end{tabular}
\caption{$\dim(\ker U(S,R))$ for $S+R$ odd. The horizontal values are increases of $R$ by $2$, starting at $R=0$ or $R=1$, if $S$ is even or odd, respectively.}
\end{table}

Looking at the difference $\dim(\ker U(S,R))-\dim(\ker U(S,R+2))$, we find the pattern
\setlength\tabcolsep{6pt}
\begin{table}[H]
\begin{tabular}{l|llllllllllllllllllllllll}
  S=2&  0 & 0 & 1 & 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0 & 1  \\
  3&  0 & 1 & 1 & 0 & 1 & 1 & 0 & 1 & 1 & 0 & 1 & 1 & 0 & 1 & 1 & 0 & 1 & 1 & 0 & 1 & 1 & 0 & 1 & 1 \\
  4&  1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1  \\
  5&  2 & 1 & 1 & 2 & 1 & 1 & 2 & 1 & 1 & 2 & 1 & 1 & 2 & 1 & 1 & 2 & 1 & 1 & 2 & 1 & 1 & 2 & 1 & 1 \\
  6&  2 & 2 & 1 & 2 & 2 & 1 & 2 & 2 & 1 & 2 & 2 & 1 & 2 & 2 & 1 & 2 & 2 & 1 & 2 & 2 & 1 & 2 & 2 & 1  \\
  7&  2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 \\
  8&  2 & 2 & 3 & 2 & 2 & 3 & 2 & 2 & 3 & 2 & 2 & 3 & 2 & 2 & 3 & 2 & 2 & 3 & 2 & 2 & 3 & 2 & 2 & 3  \\
  9&  2 & 3 & 3 & 2 & 3 & 3 & 2 & 3 & 3 & 2 & 3 & 3 & 2 & 3 & 3 & 2 & 3 & 3 & 2 & 3 & 3 & 2 & 3 & 3 \\
  10& 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3  \\
  11& 4 & 3 & 3 & 4 & 3 & 3 & 4 & 3 & 3 & 4 & 3 & 3 & 4 & 3 & 3 & 4 & 3 & 3 & 4 & 3 & 3 & 4 & 3 & 3 \\
  12& 4 & 4 & 3 & 4 & 4 & 3 & 4 & 4 & 3 & 4 & 4 & 3 & 4 & 4 & 3 & 4 & 4 & 3 & 4 & 4 & 3 & 4 & 4 & 3  \\
  13& 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 \\
  14& 4 & 4 & 5 & 4 & 4 & 5 & 4 & 4 & 5 & 4 & 4 & 5 & 4 & 4 & 5 & 4 & 4 & 5 & 4 & 4 & 5 & 4 & 4 & 5  
\end{tabular}
\caption{The differences $\dim(\ker U(S,R+2))-\dim(\ker U(S,R))$}
\label{dimkerverschillenU}
\end{table}



% OPSLAG




% [
%     [ 0, 0, 0, 1, 0, 0, 1, 0, 0, 1, 0, 0, 1, 0, 0, 1, 0, 0, 1, 0, 0, 1, 0, 0, 1, 0 ],
%     [ 0, 1, 1, 1, 0, 1, 1, 0, 1, 1, 0, 1, 1, 0, 1, 1, 0, 1, 1, 0, 1, 1, 0, 1, 1 ],
%     [ 0, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1 ],
%     [ 0, 3, 1, 1, 2, 1, 1, 2, 1, 1, 2, 1, 1, 2, 1, 1, 2, 1, 1, 2, 1, 1, 2, 1, 1 ],
%     [ 0, 2, 2, 1, 2, 2, 1, 2, 2, 1, 2, 2, 1, 2, 2, 1, 2, 2, 1, 2, 2, 1, 2, 2, 1, 2 ],
%     [ 0, 4, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2 ],
%     [ 0, 3, 2, 3, 2, 2, 3, 2, 2, 3, 2, 2, 3, 2, 2, 3, 2, 2, 3, 2, 2, 3, 2, 2, 3, 2 ],
%     [ 0, 5, 3, 3, 2, 3, 3, 2, 3, 3, 2, 3, 3, 2, 3, 3, 2, 3, 3, 2, 3, 3, 2, 3, 3 ],
%     [ 0, 4, 3, 3, 3, 3, 3, 3, 3, 3, 3, 3, 3, 3, 3, 3, 3, 3, 3, 3, 3, 3, 3, 3, 3, 3 ],
%     [ 0, 7, 3, 3, 4, 3, 3, 4, 3, 3, 4, 3, 3, 4, 3, 3, 4, 3, 3, 4, 3, 3, 4, 3, 3 ],
%     [ 0, 5, 4, 3, 4, 4, 3, 4, 4, 3, 4, 4, 3, 4, 4, 3, 4, 4, 3, 4, 4, 3, 4, 4, 3, 4 ],
%     [ 0, 8, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4 ],
%     [ 0, 6, 4, 5, 4, 4, 5, 4, 4, 5, 4, 4, 5, 4, 4, 5, 4, 4, 5, 4, 4, 5, 4, 4, 5, 4 ]
% ]

% [  1   0   1   0   1   0   3   0   3   0   3   0   5   0   5   0   5   0   7]
% [  0   2   0   2   0   4   0   6   0   6   0   8   0  10   0  10   0  12   0]
% [  1   0   3   0   5   0   7   0   9   0  11   0  13   0  15   0  17   0  19]
% [  0   2   0   6   0   8   0  10   0  14   0  16   0  18   0  22   0  24   0]
% [  1   0   5   0   9   0  11   0  15   0  19   0  21   0  25   0  29   0  31]
% [  0   4   0   8   0  12   0  16   0  20   0  24   0  28   0  32   0  36   0]
% [  3   0   7   0  11   0  17   0  21   0  25   0  31   0  35   0  39   0  45]
% [  0   6   0  10   0  16   0  22   0  26   0  32   0  38   0  42   0  48   0]
% [  3   0   9   0  15   0  21   0  27   0  33   0  39   0  45   0  51   0  57]
% [  0   6   0  14   0  20   0  26   0  34   0  40   0  46   0  54   0  60   0]
% [  3   0  11   0  19   0  25   0  33   0  41   0  47   0  55   0  63   0  69]
% [  0   8   0  16   0  24   0  32   0  40   0  48   0  56   0  64   0  72   0]
% [  5   0  13   0  21   0  31   0  39   0  47   0  57   0  65   0  73   0  83]
% [  0  10   0  18   0  28   0  38   0  46   0  56   0  66   0  74   0  84   0]
% [  5   0  15   0  25   0  35   0  45   0  55   0  65   0  75   0  85   0  95]
% [  0  10   0  22   0  32   0  42   0  54   0  64   0  74   0  86   0  96   0]
% [  5   0  17   0  29   0  39   0  51   0  63   0  73   0  85   0  97   0 107]
% [  0  12   0  24   0  36   0  48   0  60   0  72   0  84   0  96   0 108   0]
% [  7   0  19   0  31   0  45   0  57   0  69   0  83   0  95   0 107   0 121]
% [  0  14   0  26   0  40   0  54   0  66   0  80   0  94   0 106   0 120   0]
% [  7   0  21   0  35   0  49   0  63   0  77   0  91   0 105   0 119   0 133]


% 2 [ 1, 1, 1, 3, 3, 3, 5, 5, 5, 7, 7, 7, 9, 9, 9, 11, 11, 11, 13, 13, 13, 15, 15,
% 15, 17, 17 ]
% 3 [ 2, 2, 4, 6, 6, 8, 10, 10, 12, 14, 14, 16, 18, 18, 20, 22, 22, 24, 26, 26, 
% 28, 30, 30, 32, 34 ]
% 4 [ 1, 3, 5, 7, 9, 11, 13, 15, 17, 19, 21, 23, 25, 27, 29, 31, 33, 35, 37, 39, 41, 43, 45, 47, 49, 51 ]
% 5 [ 2, 6, 8, 10, 14, 16, 18, 22, 24, 26, 30, 32, 34, 38, 40, 42, 46, 48, 50, 54, 56, 58, 62, 64, 66 ]
% 6 [ 1, 5, 9, 11, 15, 19, 21, 25, 29, 31, 35, 39, 41, 45, 49, 51, 55, 59, 61, 65, 69, 71, 75, 79, 81, 85 ]
% 7 [ 4, 8, 12, 16, 20, 24, 28, 32, 36, 40, 44, 48, 52, 56, 60, 64, 68, 72, 76, 80, 84, 88, 92, 96, 100 ]
% 8 [ 3, 7, 11, 17, 21, 25, 31, 35, 39, 45, 49, 53, 59, 63, 67, 73, 77, 81, 87, 91, 95, 101, 105, 109, 115, 119 ]
% 9 [ 6, 10, 16, 22, 26, 32, 38, 42, 48, 54, 58, 64, 70, 74, 80, 86, 90, 96, 102, 106, 112, 118, 122, 128, 134 ]


% Dimker tess(s,r)- dimker tess(s,r+2)
% [ 0, 0, 2, 0, 0, 2, 0, 0, 2, 0, 0, 2, 0, 0, 2, 0, 0, 2, 0, 0, 2, 0, 0, 2 ]
% [ 0, 2, 2, 0, 2, 2, 0, 2, 2, 0, 2, 2, 0, 2, 2, 0, 2, 2, 0, 2, 2, 0, 2, 2 ]
% [ 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2 ]
% [ 4, 2, 2, 4, 2, 2, 4, 2, 2, 4, 2, 2, 4, 2, 2, 4, 2, 2, 4, 2, 2, 4, 2, 2 ]
% [ 4, 4, 2, 4, 4, 2, 4, 4, 2, 4, 4, 2, 4, 4, 2, 4, 4, 2, 4, 4, 2, 4, 4, 2 ]
% [ 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4 ]
% [ 4, 4, 6, 4, 4, 6, 4, 4, 6, 4, 4, 6, 4, 4, 6, 4, 4, 6, 4, 4, 6, 4, 4, 6 ]
% [ 4, 6, 6, 4, 6, 6, 4, 6, 6, 4, 6, 6, 4, 6, 6, 4, 6, 6, 4, 6, 6, 4, 6, 6 ]
% [ 6, 6, 6, 6, 6, 6, 6, 6, 6, 6, 6, 6, 6, 6, 6, 6, 6, 6, 6, 6, 6, 6, 6, 6 ]
% [ 8, 6, 6, 8, 6, 6, 8, 6, 6, 8, 6, 6, 8, 6, 6, 8, 6, 6, 8, 6, 6, 8, 6, 6 ]
% [ 8, 8, 6, 8, 8, 6, 8, 8, 6, 8, 8, 6, 8, 8, 6, 8, 8, 6, 8, 8, 6, 8, 8, 6 ]
% [ 8, 8, 8, 8, 8, 8, 8, 8, 8, 8, 8, 8, 8, 8, 8, 8, 8, 8, 8, 8, 8, 8, 8, 8 ]
% [ 8, 8, 10, 8, 8, 10, 8, 8, 10, 8, 8, 10, 8, 8, 10, 8, 8, 10, 8, 8, 10, 8, 8, 10 ]
% [ 8, 10, 10, 8, 10, 10, 8, 10, 10, 8, 10, 10, 8, 10, 10, 8, 10, 10, 8, 10, 10, 8, 10, 10 ]
% [ 10, 10, 10, 10, 10, 10, 10, 10, 10, 10, 10, 10, 10, 10, 10, 10, 10, 10, 10, 10, 10, 10, 10, 20 ]
\clearpage

We can do the same for $T$. We find similar dimensions (as shown in tables \ref{dimkermetnullenT}, \ref{dimkerverwijderd} and \ref{dimkerverschillenT}).
\begin{table}[H]
\begin{tabular}{l|llllllllllllllllllll}
S\textbackslash{}R & 0 & 1 & 2 & 3 & 4 & 5  & 6  & 7  & 8  & 9  & 10 & 11 & 12 & 13 & 14 & 15 & 16  & 17 & 18      \\ \hline
2 & 1&   0&   1&   0&   1&   0&   3&   0&   3&   0&   3&   0&   5&   0&   5&   0&   5&   0&   7\\
3 & 0&   2&   0&   2&   0&   4&   0&   6&   0&   6&   0&   8&   0&  10&   0&  10&   0&  12&   0\\
4 & 1&   0&   3&   0&   5&   0&   7&   0&   9&   0&  11&   0&  13&   0&  15&   0&  17&   0&  19\\
5 & 0&   2&   0&   6&   0&   8&   0&  10&   0&  14&   0&  16&   0&  18&   0&  22&   0&  24&   0\\
6 & 1&   0&   5&   0&   9&   0&  11&   0&  15&   0&  19&   0&  21&   0&  25&   0&  29&   0&  31\\
7 & 0&   4&   0&   8&   0&  12&   0&  16&   0&  20&   0&  24&   0&  28&   0&  32&   0&  36&   0\\
8 & 3&   0&   7&   0&  11&   0&  17&   0&  21&   0&  25&   0&  31&   0&  35&   0&  39&   0&  45\\
9 & 0&   6&   0&  10&   0&  16&   0&  22&   0&  26&   0&  32&   0&  38&   0&  42&   0&  48&   0\\
10 & 3&   0&   9&   0&  15&   0&  21&   0&  27&   0&  33&   0&  39&   0&  45&   0&  51&   0&  57\\
11 & 0&   6&   0&  14&   0&  20&   0&  26&   0&  34&   0&  40&   0&  46&   0&  54&   0&  60&   0\\
12 & 3&   0&  11&   0&  19&   0&  25&   0&  33&   0&  41&   0&  47&   0&  55&   0&  63&   0&  69\\
13 & 0&   8&   0&  16&   0&  24&   0&  32&   0&  40&   0&  48&   0&  56&   0&  64&   0&  72&   0\\
14 & 5&   0&  13&   0&  21&   0&  31&   0&  39&   0&  47&   0&  57&   0&  65&   0&  73&   0&  83\\
% 15 & 0&  10&   0&  18&   0&  28&   0&  38&   0&  46&   0&  56&   0&  66&   0&  74&   0&  84&   0\\
% 16 & 5&   0&  15&   0&  25&   0&  35&   0&  45&   0&  55&   0&  65&   0&  75&   0&  85&   0&  95\\
% 17 & 0&  10&   0&  22&   0&  32&   0&  42&   0&  54&   0&  64&   0&  74&   0&  86&   0&  96&   0\\
% 18 & 5&   0&  17&   0&  29&   0&  39&   0&  51&   0&  63&   0&  73&   0&  85&   0&  97&   0& 107\\
% 19 & 0&  12&   0&  24&   0&  36&   0&  48&   0&  60&   0&  72&   0&  84&   0&  96&   0& 108&   0\\
% 20 & 7&   0&  19&   0&  31&   0&  45&   0&  57&   0&  69&   0&  83&   0&  95&   0& 107&   0& 121\\
% 21 & 0&  14&   0&  26&   0&  40&   0&  54&   0&  66&   0&  80&   0&  94&   0& 106&   0& 120&   0\\
% 22 & 7&   0&  21&   0&  35&   0&  49&   0&  63&   0&  77&   0&  91&   0& 105&   0& 119&   0& 133\\
\end{tabular}
\caption{$\dim(\ker T(S,R))$.}
\label{dimkermetnullenT}
\end{table}




\setlength\tabcolsep{1.5pt}
\begin{table}[H]
\begin{tabular}{l|lllllllllllllllllllllllll}
S=2  & 1  &  1 &  1 &  3& 3& 3& 5& 5& 5& 7& 7& 7& 9& 9& 9& 11& 11& 11& 13& 13& 13& 15& 15& 15& 17\\
3  & 2  &  2 &  4 &  6& 6& 8& 10& 10& 12& 14& 14& 16& 18& 18& 20& 22& 22& 24& 26& 26& 28& 30& 30& 32& 34 \\
4  & 1  &  3 &  5 &  7& 9& 11& 13& 15& 17& 19& 21& 23& 25& 27& 29& 31& 33& 35& 37& 39& 41& 43& 45& 47& 49 \\
5  & 2  &  6 &  8 &  10& 14& 16& 18& 22& 24& 26& 30& 32& 34& 38& 40& 42& 46& 48& 50& 54& 56& 58& 62& 64& 66 \\
6  & 1  &  5 &  9 &  11& 15& 19& 21& 25& 29& 31& 35& 39& 41& 45& 49& 51& 55& 59& 61& 65& 69& 71& 75& 79& 81 \\
7  & 4  & 8& 12& 16& 20& 24& 28& 32& 36& 40& 44& 48& 52& 56& 60& 64& 68& 72& 76& 80& 84& 88& 92& 96& 100 \\
8  & 3  & 7& 11& 17& 21& 25& 31& 35& 39& 45& 49& 53& 59& 63& 67& 73& 77& 81& 87& 91& 95& 101& 105& 109& 115 \\
9  & 6  & 10& 16& 22& 26& 32& 38& 42& 48& 54& 58& 64& 70& 74& 80& 86& 90& 96& 102& 106& 112& 118& 122& 128& 134 \\
10 & 3  & 9& 15& 21& 27& 33& 39& 45& 51& 57& 63& 69& 75& 81& 87& 93& 99& 105& 111& 117& 123& 129& 135& 141& 147 \\
11 & 6  & 14& 20& 26& 34& 40& 46& 54& 60& 66& 74& 80& 86& 94& 100& 106& 114& 120& 126& 134& 140& 146& 154& 160& 166 \\
12 & 3  & 11& 19& 25& 33& 41& 47& 55& 63& 69& 77& 85& 91& 99& 107& 113& 121& 129& 135& 143& 151& 157& 165& 173& 179 \\
13 & 8  & 16& 24& 32& 40& 48& 56& 64& 72& 80& 88& 96& 104& 112& 120& 128& 136& 144& 152& 160& 168& 176& 184& 192& 200 \\
14 & 5  & 13& 21& 31& 39& 47& 57& 65& 73& 83& 91& 99& 109& 117& 125& 135& 143& 151& 161& 169& 177& 187& 195& 203& 213 \\
15 & 10 & 18& 28& 38& 46& 56& 66& 74& 84& 94& 102& 112& 122& 130& 140& 150& 158& 168& 178& 186& 196& 206& 214& 224& 234 \\
16 & 5  & 15& 25& 35& 45& 55& 65& 75& 85& 95& 105& 115& 125& 135& 145& 155& 165& 175& 185& 195& 205& 215& 225& 235& 255 
\end{tabular}
\caption{$\dim(\ker T(S,R))$ for $S+R$ odd. The horizontal values are increases of $R$ by $2$, starting at $R=0$ or $R=1$, if $S$ is even or odd, respectively.}
\label{dimkerverwijderd}
\end{table}



\setlength\tabcolsep{5pt}
\begin{table}[H]
\begin{tabular}{l|lllllllllllllllllllllllll}
S=2& 0& 0& 2& 0& 0& 2& 0& 0& 2& 0& 0& 2& 0& 0& 2& 0& 0& 2& 0& 0& 2& 0& 0& 2 \\
3& 0& 2& 2& 0& 2& 2& 0& 2& 2& 0& 2& 2& 0& 2& 2& 0& 2& 2& 0& 2& 2& 0& 2& 2 \\
4& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2 \\
5& 4& 2& 2& 4& 2& 2& 4& 2& 2& 4& 2& 2& 4& 2& 2& 4& 2& 2& 4& 2& 2& 4& 2& 2 \\
6& 4& 4& 2& 4& 4& 2& 4& 4& 2& 4& 4& 2& 4& 4& 2& 4& 4& 2& 4& 4& 2& 4& 4& 2 \\
7& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4 \\
8& 4& 4& 6& 4& 4& 6& 4& 4& 6& 4& 4& 6& 4& 4& 6& 4& 4& 6& 4& 4& 6& 4& 4& 6 \\
9& 4& 6& 6& 4& 6& 6& 4& 6& 6& 4& 6& 6& 4& 6& 6& 4& 6& 6& 4& 6& 6& 4& 6& 6 \\
10& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6 \\
11& 8& 6& 6& 8& 6& 6& 8& 6& 6& 8& 6& 6& 8& 6& 6& 8& 6& 6& 8& 6& 6& 8& 6& 6 \\
12& 8& 8& 6& 8& 8& 6& 8& 8& 6& 8& 8& 6& 8& 8& 6& 8& 8& 6& 8& 8& 6& 8& 8& 6 \\
13& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8 \\
14& 8& 8& 10& 8& 8& 10& 8& 8& 10& 8& 8& 10& 8& 8& 10& 8& 8& 10& 8& 8& 10& 8& 8& 10 
% 15& 8& 10& 10& 8& 10& 10& 8& 10& 10& 8& 10& 10& 8& 10& 10& 8& 10& 10& 8& 10& 10& 8& 10& 10 \\
% 16& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 20 
\end{tabular}
\caption{The differences $\dim(\ker T(S,R+2))-\dim(\ker T(S,R))$}
\label{dimkerverschillenT}
\end{table}
















































\subsubsection{Notes}
\begin{enumerate}
    \item Table \ref{dimkermetnullenU} is symmetric along the diagonal $S=R-2$. This suggests that $\dim (\ker U(S,R))=\dim (\ker U(R+2,S-2)$. This identity follows from the partition relation
    \begin{equation*}
        \begin{bmatrix}
    s_1,s_2\\
    r_1,r_2
    \end{bmatrix}=\sum_{\substack{0\leq j\leq r_1\\0\leq k\leq s_2-1}}(-1)^k{{s_1-1+k}\choose k}{{r_2+j}\choose j}\begin{bmatrix}
    r_2+j+1,r_1-j+1\\
    s_2-1-k,s_1-1+k
    \end{bmatrix},
    \end{equation*}
    because this identity induces a bijection between the spaces spanned by bi-brackets of weight $S,R$ and by weight $R-2,S+2$. (!!Formuleer precies!!)
    \item All values in table \ref{dimkerverschillenT} are twice that of table \ref{dimkerverschillenU}. This suggests that
    \begin{equation*}
        \dim (\ker U(S,R+2))-\dim (\ker U(S,R))=2\big(\dim (\ker T(S,R+2))-\dim (\ker T(S,R))\big).
    \end{equation*}
    This can be explained by the symmetry arising from $\begin{bmatrix}j\\k\end{bmatrix}\begin{bmatrix}S-j\\R-k\end{bmatrix}=\begin{bmatrix}S-j\\R-k\end{bmatrix}\begin{bmatrix}j\\k\end{bmatrix}$.\\
    \item We have the apparent equality $\dim( \ker T(6,2R))=\dim S_{2R}^{\operatorname{new}}(\Gamma_0(45))$. Since the differences $\dim S_{2R+2}^{\operatorname{new}}(\Gamma_0(N))-\dim S_{2R}^{\operatorname{new}}(\Gamma_0(N))$ appear to be similar as those in table \ref{dimkerverschillenU} and \ref{dimkerverschillenT}, this seems to be a \textit{coincidence}.
\end{enumerate}


==> Introductie.tex <==
Dingen die ge\"introduceerd moeten worden:
\begin{enumerate}
    \item De multiple zeta values $\zeta(s_1,\dots,s_l)$ and the relations between them and the shuffle and stuffle algebras.
    \item Relaties tussen multiple zeta values, problemen stellen over multiple zeta values. Waarom hebben we de $q$-analogen nodig?
    \item Verscheidene $q$-analogen: $\tilde{\zeta_q},\zeta_q\mathfrak{z}_q$. Ook de brackets van Wadim introduceren en de directe link tussen de brackets bewijzen. Zie MZF dictaat p83.
    \item Introductie over $\MD$ en $\BD$ (geintroduceerd door Bachmann). Laten zien dat dit ook een $q$-analoog is.
    \item Probleemstelling: $\MD=\BD$. Wat is er al bekend?
    \item Wat heb ik gevonden: $l=2$ en odd total weight.
\end{enumerate}

Ideeen:
\begin{enumerate}
    \item Misschien het bewijs van $l=2$, odd weight, aanpassen naar de algebra $Z=\{z_{s_1,r_1}\mid s_i,r_i\geq 1\}$. Vragen aan Wadim of dit netter is.
\end{enumerate}

==> Oddweight.tex <==
\begin{definition}
For $r_1,\dots,r_l\geq 0$ and $s_1,\dots,s_l>0$ we define the following $q$-series,
\begin{equation*}
    \begin{bmatrix}s_1,\dots,s_l\\r_1,\dots,r_l\end{bmatrix}\coloneqq \sum_{\substack{u_1>\dots>u_l>0\\v_1,\dots,v_l>0}}\frac{u_1^{r_1}\cdots u_l^{r_l}}{r_1!\cdots r_l!}\frac{v_1^{s_1-1}\cdots v_l^{s_l-1}}{(s_1-1)!\cdots(s_l-1)!}q^{u_1v_1+\dots+u_lv_l}.
\end{equation*}
\end{definition}
\begin{remark}
We have the following immediate relation between mono-brackets and bi-brackets $\begin{bmatrix}s_1,\dots,s_l\end{bmatrix}=\begin{bmatrix}s_1,\dots,s_l\\0,\dots,0\end{bmatrix}$.
\end{remark}
\begin{definition}
For fixed length $l$, we denote the generating functions of the bi-brackets as
\begin{equation*}
    \begin{vmatrix}X_1,\dots,X_l\\Y_1,\dots,Y_l\end{vmatrix}\coloneqq\sum_{\substack{s_1,\dots,s_l>0\\r_1,\dots,r_l\geq0}}\begin{bmatrix}s_1,\dots,s_l\\r_1,\dots,r_l\end{bmatrix}X_1^{s_1-1}\cdots X_l^{s_l-1}Y_1^{r_1}\cdots Y_l^{r_l}.
\end{equation*}
\end{definition}
\begin{proposition}
For an integer $n\in\N$ we define
\begin{equation*}
    E_n(X)\coloneqq e^{nX},\qquad\qquad L_n(X)\coloneqq \frac{e^Xq^n}{1-e^Xq^n}=\sum_{k>0}(e^Xq^n)^k.
\end{equation*}
Then we have the following two identities between generating functions:
\begin{align*}
    \begin{vmatrix}X_1,\dots,X_l\\Y_1,\dots,Y_l\end{vmatrix}&=\sum_{u_1>\dots>u_l>0}\prod_{j=1}^lE_{u_j}(Y_j)L_{u_j}(X_j)\\
    &=\sum_{u_1>\dots>u_l>0}\prod_{j=1}^lE_{u_j}(X_{l+1-j}-X_{l+2-j})L_{u_j}(Y_1+\dots+Y_{l-j+1}).
\end{align*}
The last relation gives us the immediate relation
\begin{equation*}
    \begin{vmatrix}X_1,\dots,X_l\\Y_1,\dots,Y_l\end{vmatrix}=\begin{vmatrix}Y_1+\dots+Y_l,\dots,Y_1+Y_2,Y_1\\X_l,X_{l-1}-X_l,\dots,X_1-X_2\end{vmatrix}.
\end{equation*}
\end{proposition}
\begin{proof}
We have
\begin{align*}
    \begin{vmatrix}X_1,\dots,X_l\\Y_1,\dots,Y_l\end{vmatrix}&=\sum_{\substack{s_1,\dots,s_l>0\\r_1,\dots,r_l\geq 0}}\sum_{\substack{u_1>\dots>u_l>0\\v_1,\dots,v_l>0}}\frac{u_1^{r_1}\cdots u_l^{r_l}}{r_1!\cdots r_l!}\frac{v_1^{s_1-1}\cdots v_l^{s_l-1}}{(s_1-1)!\cdots(s_l-1)!}q^{u_1v_1+\dots+u_lv_l}X_1^{s_1-1}\cdots X_l^{s_l-1}Y_1^{r_1}\cdots Y_l^{r_l}\\
    &=\sum_{\substack{u_1>\dots>u_l>0\\v_1,\dots,v_l>0}}\sum_{\substack{s_1,\dots,s_l>0\\r_1,\dots,r_l\geq 0}}\prod_{j=1}^l\frac{u_j^{r_j}}{r_j!}\frac{v_j^{s_j-1}}{(s_j-1)!}q^{u_jv_j}X_j^{s_j-1}Y_j^{r_j}\\
    &=\sum_{\substack{u_1>\dots>u_l>0\\v_1,\dots,v_l>0}}e^{u_jY_j}e^{v_jX_j}q^{u_jv_j}\\
    &=\sum_{\substack{u_1>\dots>u_l>0\\v_1,\dots,v_l>0}}e^{u_jY_j}\left(e^{X_j}q^{u_j}\right)^{v_j}\\
    &=\sum_{u_1>\dots>u_l>0}E_{u_j}(Y_j)L_{v_j}(X_j).
\end{align*}
This proves the first identity. For the second identity, we apply the transformations $u_j=u_1'+\dots+u_{l-j+1}'$ and $v_j=v_{l-j+1}'-v_{l-j+2}'$ to
\begin{align*}
    \begin{vmatrix}X_1,\dots,X_l\\Y_1,\dots,Y_l\end{vmatrix}&=\sum_{\substack{u_1>\dots>u_l>0\\v_1,\dots,v_l>0}}e^{u_jY_j}e^{v_jX_j}q^{u_jv_j}.
\end{align*}
Under these transformations, we have $v'_j=v_1+\dots+v_{l-j+1}$, so that
\begin{align*}
    q^{u_1v_1+\dots+u_lv_l}&=q^{(u_1'+\dots+u_l')v_1+(u_1'+\dots+u_{l-1}')v_1+\dots+(u_1'+u_2')v_{l-1}+u_1'v_l}\\
    &=q^{u_1'(v_1+\dots+v_l)+u_2'(v_1+\dots+v_{l-1})+\dots+u_{l-1}'(v_1+v_2)+u_l'v_l}\\
    &=q^{u_1'v_1'+u_2'v_2'+\dots+u_l'v_l'}.
\end{align*}
Additionally, the conditions $u_1>\dots>u_l>0$ and $v_1,\dots,v_l>0$ become $u_1',\dots,u_l'>0$ and $v_1'>\dots>v_l'>0$. So we have
\begin{align*}
    \begin{vmatrix}X_1,\dots,X_l\\Y_1,\dots,Y_l\end{vmatrix}&=\sum_{\substack{v_1'>\dots>v_l'>0\\u_1',\dots,u_l'>0}}e^{(v_{l-j+1}'-v_{l-j+2}')X_j}e^{(u_1'+\dots+u_{l-j+1}')Y_j}q^{u_j'v_j'}\\
    &=\sum_{\substack{v_1'>\dots>v_l'>0\\u_1',\dots,u_l'>0}}e^{v_j'(X_{l-j+1}-X_{l-j+2})}e^{u_j'(Y_1+\dots+Y_{l-j+1})}q^{u_j'v_j'}\\
    &=\sum_{\substack{v_1'>\dots>v_l'>0\\u_1',\dots,u_l'>0}}E_{v_j}(X_{l-j+1}-X_{l-j+2})L_{u_j}(Y_1+\dots+Y_{l-j+1})\\
    &=\begin{vmatrix}Y_1+\dots+Y_l,\dots,Y_1+Y_2,Y_1\\X_l,X_{l-1}-X_l,\dots,X_1-X_2\end{vmatrix}.
\end{align*}
\end{proof}

\begin{corollary}
\label{generatingpartitionexample}
For length $l=1$ and $l=2$, respectively, we have
\begin{equation*}
    \begin{vmatrix}X\\Y\end{vmatrix}=\begin{vmatrix}Y\\X\end{vmatrix},\qquad\qquad \begin{vmatrix}X_1,X_2\\Y_1,Y_2\end{vmatrix}=\begin{vmatrix}Y_1+Y_2,Y_1\\X_2,X_1-X_2\end{vmatrix}.
\end{equation*}
\end{corollary}
\begin{corollary}
\label{length1partition}
For $s>0$ and $r\geq 0$ we have $\begin{bmatrix}s\\r\end{bmatrix}=\begin{bmatrix}r+1\\s-1\end{bmatrix}$.
\end{corollary}
\begin{proof}
For length $l=1$, Corollary \ref{generatingpartitionexample} gives us
$\begin{vmatrix}X\\Y\end{vmatrix}=\begin{vmatrix}Y\\X\end{vmatrix}$. Considering the coefficient of $X^{s-1}Y^r$, we obtain the desired equation.
\end{proof}
\begin{proposition}
For $s>0$ and $r\geq 0$ we have $\begin{bmatrix}s\\r\end{bmatrix}\in \MD$.
\end{proposition}
\begin{proof}
Since we have $\begin{bmatrix}s\\r\end{bmatrix}=\begin{bmatrix}r+1\\s-1\end{bmatrix}$, we may assume that $s>r$. Then, after applying Proposition \ref{invarianceofd} several times, we get
\begin{equation*}
    \begin{bmatrix}s\\r\end{bmatrix}=d^r\begin{bmatrix}s-r\\0\end{bmatrix}=d^r[s-r]\in \MD
\end{equation*}
\end{proof}
\begin{proposition}
For $s_1,s_2>0$, $r_1,r_2\geq 0$ and for odd total weight $s_1+s_2+r_1+r_2$ we have
\begin{equation*}
    \begin{bmatrix}
    s_1,s_2\\
    r_1,r_2
    \end{bmatrix}\in \MD.
\end{equation*}
\end{proposition}
\noindent\textit{Proof.} We know that bi-brackets of length $l=1$ are contained in $\MD$. Hence the stuffle and shuffle analogues (modulo length $l=1$) for bi-brackets give rise to the following equations
\begin{align*}
    0&\equiv\begin{bmatrix}
    s_1,s_2\\
    r_1,r_2
    \end{bmatrix}+\begin{bmatrix}
    s_2,s_1\\
    r_2,r_1
    \end{bmatrix},\tag{$i$}\\
    0&\equiv\sum_{\substack{1\leq j\leq s_1\\ 0\leq k\leq r_2}}{s_1+s_2-j-1 \choose s_2-1}{r_1+r_2-k \choose r_1}(-1)^{r_2-k}\begin{bmatrix}
    s_1+s_2-j,j\\
    k,r_1+r_2-k
    \end{bmatrix}\tag{$ii$}\\
    &+\sum_{\substack{1\leq j\leq s_2\\ 0\leq k\leq r_1}}{s_1+s_2-j-1 \choose s_1-1}{r_1+r_2-k \choose r_2}(-1)^{r_1-k}\begin{bmatrix}
    s_1+s_2-j,j\\
    k,r_1+r_2-k
    \end{bmatrix}.\tag{$iii$}
\end{align*}
Then, by considering all products of fixed upper and lower weight
\begin{equation*}
    \begin{bmatrix}
    s_1+s_2-n\\
    r_1+r_2-m
    \end{bmatrix}\begin{bmatrix}
    n\\
    m
    \end{bmatrix}
\end{equation*}
for $1\leq n \leq s_1+s_2-1$ and $0\leq m\leq r_1+r_2$, we get a system of linear equations in terms of the bi-brackets of constant weight $s_1+s_2+r_1+r_2$:
\begin{equation*}
    \begin{bmatrix}
    s_1+s_2-j, j\\
    k, r_1+r_2-k
    \end{bmatrix}.
\end{equation*}
We will show that, for odd total weight, this system has a solution. Namely, if we apply the relation
\begin{equation*}
    \begin{bmatrix}
    s_1,s_2\\
    r_1,r_2
    \end{bmatrix}\equiv-\begin{bmatrix}
    s_2,s_1\\
    r_2,r_1
    \end{bmatrix}
\end{equation*}
to the terms in $(iii)$, use the fact that ${a \choose b}=0$ if $b>a$ or if $b<0$, and the apply the transformation $k\mapsto r_1+r_2-k+1$, we can show that the new system
\begin{align*}
0&\equiv\sum_{\substack{1\leq j\leq s_1+s_2\\ 1\leq k\leq r_1+r_2+1}}{s_1+s_2-j-1 \choose s_2-1}{k-1 \choose r_1}(-1)^{r_1+k+1}\begin{bmatrix}
    s_1+s_2-j,&j\\
    r_1+r_2-k+1,&k-1
    \end{bmatrix}\\
    &-\sum_{\substack{1\leq j\leq s_1+s_2\\ 1\leq k\leq r_1+r_2+1}}{s_1+s_2-j-1 \choose s_1-1}{k-1 \choose r_2}(-1)^{r_2+k+1}\begin{bmatrix}
    j,&s_1+s_2-j\\
    k-1,&r_1+r_2-k+1
    \end{bmatrix}\tag{$\ast$}
\end{align*}
has a solution.

Define the matrices $n\times n$-matrices $P_n$ and $Q_n$ by 
\begin{equation*}
    (P_n)_{i,j}={n-j\choose i-1},\qquad\qquad (Q_n)_{i,j}=(-1)^{i+j+n+1}{j-1 \choose n-i}.
\end{equation*}
For a $n\times n$-matrix $A$, define $\rho$ and $\sigma$ to be the horizontal and vertical reflections
\begin{equation*}
    (A^\rho)_{i,j}=A_{n+1-i,j},\qquad\qquad(A^\sigma)_{i,j}=A_{i,n+1-j}.
\end{equation*}
Then for fixed upper and lower weight $S=s_1+s_2$ and $R=r_1+r_2$, the system $(\ast)$ corresponds to the equation
\begin{equation*}
    \left(P_{S-1}\otimes Q_{R+1}-P_{S-1}^{\rho\sigma}\otimes Q_{R+1}^{\rho\sigma}\right)\vec{v}=\vec{0},
\end{equation*}
with 
\begin{equation*}
    \vec{v}=\left.\left(\begin{bmatrix}
    S-i,&i\\
    R+1-j,&j-1
    \end{bmatrix}\ \right|\ 1\leq i\leq S-1,\ 1\leq j\leq R+1 \right).
\end{equation*}
We claim that $P_{S-1}\otimes Q_{R+1}-P_{S-1}^{\rho\sigma}\otimes Q_{R+1}^{\rho\sigma}$ is invertible, with its inverse given by 
\begin{equation*}
    \frac{1}{2}\left(M_{S,R}+Q_{S-1}\otimes P_{R+1}-Q_{S-1}^{\rho\sigma}\otimes P_{R+1}^{\rho\sigma}\right).
\end{equation*}
Here, $M_{S,R}$ is the matrix defined by $M_{S,R}=J_{S-1}\otimes J_{R+1}$, with $(J_n)_{i,j}=\begin{cases}(-1)^{i+1}&\text{ if }i=j\\0&\text{ if } i\neq j\end{cases}$.

    
Consider the product
\begin{align*}
    \Sigma\coloneqq\left(P_{S-1}\otimes \right.&\left.Q_{R+1}-P_{S-1}^{\rho\sigma}\otimes\ Q_{R+1}^{\rho\sigma}\right)\left(Q_{S-1}\otimes P_{R+1}-Q_{S-1}^{\rho\sigma}\otimes P_{R+1}^{\rho\sigma}\right)=P_{S-1}Q_{S-1}\otimes Q_{R+1}P_{R+1}\\
    &-P_{S-1}Q_{S-1}^{\rho\sigma}\otimes Q_{R+1}P_{R+1}^{\rho\sigma}-P_{S-1}^{\rho\sigma}Q_{S-1}\otimes Q_{R+1}^{\rho\sigma}P_{R+1}+P_{S-1}^{\rho\sigma}Q_{S-1}^{\rho\sigma}\otimes Q_{R+1}^{\rho\sigma}P_{R+1}^{\rho\sigma}.
\end{align*}
We have the following equality's (for their proof see \ref{binomialidentities}):
\begin{align*}
    (P_{S-1}Q_{S-1})_{i,j}&=\sum_{k=1}^{S-1} (-1)^{k+j+S}{S-1-k \choose i-1}{j-1\choose S-1-k}=\begin{cases}1 & \qquad\text{ if }i=j\\
    0&\qquad\text{ if }i\neq j\end{cases},\\
    (Q_{R+1}P_{R+1})_{i,j}&=\sum_{k=1}^{R+1} (-1)^{k+i+R}{k-1 \choose R+1-i}{R+1-j\choose k-1}=\begin{cases}1 & \qquad\text{ if }i=j\\
    0&\qquad\text{ if }i\neq j\end{cases},\\
    (P_{S-1}Q^{\rho\sigma}_{S-1})_{i,j}&=\sum_{k=1}^{S-1} (-1)^{k+j+S}{S-1-k \choose i-1}{S-1-j\choose k-1}=(-1)^{j+S+1}{j-1\choose S-1-i},\\
    (Q_{R+1}P^{\rho\sigma}_{R+1})_{i,j}&=\sum_{k=1}^{R+1} (-1)^{k+i+R}{j-1\choose R+1-k}{k-1 \choose R+1-i}=(-1)^{i+1}{R+1-j\choose i-1},\\
    (P_{S-1}^{\rho\sigma}Q_{S-1})_{i,j}&=\sum_{k=1}^{S-1}(-1)^{k+j+S}{j-1\choose S-1-k}{k-1\choose S-1-i}=(-1)^{j+1}{S-1-j\choose i-1},\\
    (Q_{R+1}^{\rho\sigma}P_{R+1})_{i,j}&=\sum_{k=1}^{R+1}(-1)^{k+i+R}{R+1-k\choose i-1}{R+1-j\choose k-1}=(-1)^{i+R+1}{j-1\choose R+1-i},\\
    (P^{\rho\sigma}_{S-1}Q^{\rho\sigma}_{S-1})_{i,j}&=\sum_{k=1}^{S-1} (-1)^{k+j+S}{k-1 \choose S-1-i}{S-1-j\choose k-1}=\begin{cases}1 & \qquad\text{ if }i=j\\
    0&\qquad\text{ if }i\neq j\end{cases},\\
    (Q^{\rho\sigma}_{R+1}P^{\rho\sigma}_{R+1})_{i,j}&=\sum_{k=1}^{R+1} (-1)^{k+i+R}{R+1-k \choose i-1}{j-1\choose R+1-k}=\begin{cases}1 & \qquad\text{ if }i=j\\
    0&\qquad\text{ if }i\neq j\end{cases}.
\end{align*}
Note that the last four identities follow from the first four.
On the other hand, we have 
\begin{align*}
    (P_{S-1}J_{S-1})_{i,j}&=(-1)^{j+1}{S-1-j\choose i-1}\\
    (Q_{R+1}J_{R+1})_{i,j}&=(-1)^{i+R+1}{j-1\choose R+1-i}\\
    (P^{\rho\sigma}_{S-1}J_{S-1})_{i,j}&=(-1)^{j+1}{j-1\choose S-1-i}\\
    (Q^{\rho\sigma}_{R+1}J_{R+1})_{i,j}&=(-1)^{i+R+1}{R+1-j\choose i-1}.
\end{align*}
Since we require $S+R$ to be odd, either $S$ is even and $R$ is odd, or $S$ is odd and $R$ is even. In the first case we have $P_{S-1}Q^{\rho\sigma}_{S-1}=P^{\rho\sigma}_{S-1}J_{S-1}$ and $Q_{R+1}P^{\rho\sigma}_{R+1}=-Q^{\rho\sigma}_{R+1}J_{R+1}$. In the second case we get $P_{S-1}Q^{\rho\sigma}_{S-1}=-P^{\rho\sigma}_{S-1}J_{S-1}$ and $Q_{R+1}P^{\rho\sigma}_{R+1}=Q^{\rho\sigma}_{R+1}J_{R+1}$.
In either case, we have the following equality
\begin{equation*}
    P_{S-1}Q^{\rho\sigma}_{S-1}\otimes Q_{R+1}P^{\rho\sigma}_{R+1}=-P^{\rho\sigma}_{S-1}J_{S-1}\otimes Q^{\rho\sigma}_{R+1}J_{R+1}.
\end{equation*}
Additionally, we always have
\begin{equation*}
    P_{S-1}^{\rho\sigma}Q_{S-1}\otimes Q_{R+1}^{\rho\sigma}P_{R+1}=P_{S-1}J_{S-1}\otimes Q_{R+1}J_{R+1}.
\end{equation*}


Combining all the parts, we obtain
\begin{align*}
    \Sigma&=2I_{(S-1)(R+1)}-P_{S-1}Q_{S-1}^{\rho\sigma}\otimes Q_{R+1}P_{R+1}^{\rho\sigma}-P_{S-1}^{\rho\sigma}Q_{S-1}\otimes Q_{R+1}^{\rho\sigma}P_{R+1}\\
    &=2I_{(S-1)(R+1)}+P^{\rho\sigma}_{S-1}J_{S-1}\otimes Q^{\rho\sigma}_{R+1}J_{R+1}-P_{S-1}J_{S-1}\otimes Q_{R+1}J_{R+1}\\
    &=2I_{(S-1)(R+1)}-\left(P_{S-1}\otimes Q_{R+1}-P^{\rho\sigma}_{S-1}\otimes Q^{\rho\sigma}_{R+1}\right)M_{S,R}.
\end{align*}
This proves the desired claim:
\begin{equation*}
    \frac{1}{2}\left(P_{S-1}\otimes Q_{R+1}-P_{S-1}^{\rho\sigma}\otimes Q_{R+1}^{\rho\sigma}\right)\left(M_{S,R}+Q_{S-1}\otimes P_{R+1}-Q_{S-1}^{\rho\sigma}\otimes P_{R+1}^{\rho\sigma}\right)=I_{(S-1)(R+1)}.
\end{equation*}
\qed

\begin{lemma}
\label{binomialidentities}
For $n\geq1$ and $1\leq i,j\leq n$ integers we have
\begin{align*}
    \sum_{k=1}^n(-1)^{k+j+n+1} {n-k \choose i-1}{j-1\choose n-k}&=\begin{cases}1 & \qquad\text{ if }i=j\tag{1}\\
    0&\qquad\text{ if }i\neq j\end{cases}\\
    \sum_{k=1}^n (-1)^{k+i+n+1}{k-1 \choose n-i}{n-j\choose k-1}&=\begin{cases}1 & \qquad\text{ if }i=j\tag{2}\\
    0&\qquad\text{ if }i\neq j\end{cases}\\
    \sum_{k=1}^n (-1)^{k+j+n+1}{n-k \choose i-1}{n-j\choose k-1}&=(-1)^{j+n}{j-1\choose n-i}\tag{3}\\
    \sum_{k=1}^n (-1)^{k+i+n+1}{j-1\choose n-k}{k-1 \choose n-i}&=(-1)^{i+1}{n-j\choose i-1}.\tag{4}
\end{align*}
\end{lemma}
\begin{proof}
We prove all four equations by induction.\\
$(1)$: The case $n=1$ is clear. If $i=1$ we have 
\begin{equation*}
    \sum_{k=1}^{n+1}(-1)^{k+n+j}{n+1-k\choose i-1}{j-1 \choose n+1-k}=\sum_{k=1}^{n+1}(-1)^{k+n+j}{j-1 \choose n+1-k}=\begin{cases}1&\text{ if } j=1\\0&\text{ if } j\neq 1\end{cases},
\end{equation*}
where the second equality follows form $\sum_{k=0}^n(-1)^k{n \choose k}$ equals $0$ if $n>0$ and $1$ otherwise. If $j=1$, we have
\begin{equation*}
    \sum_{k=1}^{n+1}(-1)^{k+n+j}{n+1-k\choose i-1}{j-1 \choose n+1-k}={0\choose i-1}=\begin{cases}1&\text{ if } i=1\\0&\text{ if } i\neq 1\end{cases}.
\end{equation*}
Now suppose that $i>1$. We have
\begin{align*}
    \sum_{k=1}^{n+1}(-1)^{k+n+j}{n+1-k\choose i-1}{j-1 \choose n+1-k}&=(-1)^{j+1}{0 \choose i-1}{j-1\choose 0}+\sum_{k=1}^{n}(-1)^{k+n+j}{n-k+1\choose i-1}{j-1 \choose n-k+1}\\
    &=0+\frac{j-1}{i-1}\cdot\sum_{k=1}^n(-1)^{k+n+(j-1)+1}{n-k\choose i-2}{j-2\choose n-k}\\
    &=\begin{cases}1&\text{ if } i=j\\0&\text{ if } i\neq j\end{cases}.
\end{align*}
This shows $(1)$.\\
$(2)$: The case $n=1$ is clear. First suppose that $i=1$. Then, the required identity can be proven by the same argument as in $(1)$ with $i=1$. Now, if $j=1$ and $i>1$, we get
\begin{align*}
    (-1)^{k+i+n}{k-1 \choose n+1-i}{n\choose k-1}=(-1)^{k+i+n}\left[{k-1 \choose n+1-i}\right.&{n-1 \choose k-1}\\&+\left.{k-2 \choose n+1-i}{n-1 \choose k-2}+{k-2 \choose n-i}{n-1 \choose k-2}\right]
\end{align*}
Then, after the case distinction $i=n+1$ and $i<n+1$, we find that we must have
\begin{equation*}
    \sum_{k=1}^{n+1}(-1)^{k+i+n}{k-1 \choose n+1-i}{n\choose k-1}=0.
\end{equation*}

Finally, for $i,j>1$ we obtain
\begin{align*}
    \sum_{k=1}^{n+1} (-1)^{k+(i-1)+n+1}{k-1 \choose n+1-i}{n+1-j\choose k-1}&=0+\sum_{k=1}^{n} (-1)^{k+i+n}{k-1 \choose n-(i-1)}{n-(j-1)\choose k-1}\\
    &=\begin{cases}1&\text{ if } i=j\\0&\text{ if } i\neq j\end{cases}.
\end{align*}
This shows $(2)$.\\
$(3)$: If $n=1$, $i=1$ or $j=1$, one can easily check see that the equation holds. If $i,j>1$, we have
\begin{align*}
    \sum_{k=1}^{n+1} (-1)^{k+j+n}{n+1-k \choose i-1}{n+1-j\choose k-1}&=0+\sum_{k=1}^{n} (-1)^{k+j+n}{n+1-k \choose i-1}{n+1-j\choose k-1}\\
    &=\sum_{k=1}^{n} (-1)^{k+j+n}\left[{n-k \choose i-1}{n+1-j\choose k-1}+{n-k \choose i-2}{n+1-j\choose k-1}\right]\\
    &=(-1)^{j-1+n}\left[{j-2\choose n-i}+{j-2\choose n-i-1}\right]\\
    &=(-1)^{j+n+1}{j-1\choose n-i}.
\end{align*}
This shows $(3)$.\\
$(4)$: First we apply the transformation $k'=n+1-k$, so that we have to show
\begin{equation*}
    \sum_{k'=1}^n(-1)^{k'+i}{j-1 \choose k'-1}{n-k'\choose i-k'}=(-1)^{i+1}{n-j\choose i-1}.
\end{equation*}
The cases where $n=1$, $i=1$ or $i=n$ are easily deducible. So we may assume that $1<i<n+1$. We have
\begin{align*}
    \sum_{k'=1}^{n+1}(-1)^{k'+i}{j-1 \choose k'-1}{n+1-k'\choose i-k'}&=0+\sum_{k=1}^n(-1)^{k+i}\left[{j-1 \choose k'-1}{n-k'\choose i-k'}+{j-1 \choose k'-1}{n-k'\choose i-1-k'}\right]\\
    &=(-1)^{i+1}{n-j\choose i-1}-(-1)^{i}{n-j\choose i-2}\\
    &=(-1)^{i+1}{n+1-j\choose i-1}.
\end{align*}
This shows $(4)$ and finishes the proof.
\end{proof}

==> Partition.tex <==
\begin{definition}
For $r_1,\dots,r_l\geq 0$ and $s_1,\dots,s_l>0$, we define the following $q$-series,
\begin{equation*}
    \begin{bmatrix}s_1,\dots,s_l\\r_1,\dots,r_l\end{bmatrix}\coloneqq \sum_{\substack{u_1>\dots>u_l>0\\v_1,\dots,v_l>0}}\frac{u_1^{r_1}\cdots u_l^{r_l}}{r_1!\cdots r_l!}\frac{v_1^{s_1-1}\cdots v_l^{s_l-1}}{(s_1-1)!\cdots(s_l-1)!}q^{u_1v_1+\dots+u_lv_l}.
\end{equation*}
\end{definition}
\begin{remark}
We have the following immediate relation between mono-brackets and bi-brackets $\begin{bmatrix}s_1,\dots,s_l\end{bmatrix}=\begin{bmatrix}s_1,\dots,s_l\\0,\dots,0\end{bmatrix}$.
\end{remark}
\begin{definition}
For fixed length $l$, we denote the generating functions of the bi-brackets as
\begin{equation*}
    \begin{vmatrix}X_1,\dots,X_l\\Y_1,\dots,Y_l\end{vmatrix}\coloneqq\sum_{\substack{s_1,\dots,s_l>0\\r_1,\dots,r_l\geq0}}\begin{bmatrix}s_1,\dots,s_l\\r_1,\dots,r_l\end{bmatrix}X_1^{s_1-1}\cdots X_l^{s_l-1}Y_1^{r_1}\cdots Y_l^{r_l}.
\end{equation*}
\end{definition}
\begin{proposition}
For an integer $n\in\N$ we define
\begin{equation*}
    E_n(X)\coloneqq e^{nX},\qquad\qquad L_n(X)\coloneqq \frac{e^Xq^n}{1-e^Xq^n}=\sum_{k>0}(e^Xq^n)^k.
\end{equation*}
Then we have the following two identities between generating functions:
\begin{align*}
    \begin{vmatrix}X_1,\dots,X_l\\Y_1,\dots,Y_l\end{vmatrix}&=\sum_{u_1>\dots>u_l>0}\prod_{j=1}^lE_{u_j}(Y_j)L_{u_j}(X_j)\\
    &=\sum_{u_1>\dots>u_l>0}\prod_{j=1}^lE_{u_j}(X_{l+1-j}-X_{l+2-j})L_{u_j}(Y_1+\dots+Y_{l-j+1}).
\end{align*}
The last relation gives us the immediate relation
\begin{equation*}
    \begin{vmatrix}X_1,\dots,X_l\\Y_1,\dots,Y_l\end{vmatrix}=\begin{vmatrix}Y_1+\dots+Y_l,\dots,Y_1+Y_2,Y_1\\X_l,X_{l-1}-X_l,\dots,X_1-X_2\end{vmatrix}.
\end{equation*}
\end{proposition}
\begin{proof}
We have
\begin{align*}
    \begin{vmatrix}X_1,\dots,X_l\\Y_1,\dots,Y_l\end{vmatrix}&=\sum_{\substack{s_1,\dots,s_l>0\\r_1,\dots,r_l\geq 0}}\sum_{\substack{u_1>\dots>u_l>0\\v_1,\dots,v_l>0}}\frac{u_1^{r_1}\cdots u_l^{r_l}}{r_1!\cdots r_l!}\frac{v_1^{s_1-1}\cdots v_l^{s_l-1}}{(s_1-1)!\cdots(s_l-1)!}q^{u_1v_1+\dots+u_lv_l}X_1^{s_1-1}\cdots X_l^{s_l-1}Y_1^{r_1}\cdots Y_l^{r_l}\\
    &=\sum_{\substack{u_1>\dots>u_l>0\\v_1,\dots,v_l>0}}\sum_{\substack{s_1,\dots,s_l>0\\r_1,\dots,r_l\geq 0}}\prod_{j=1}^l\frac{u_j^{r_j}}{r_j!}\frac{v_j^{s_j-1}}{(s_j-1)!}q^{u_jv_j}X_j^{s_j-1}Y_j^{r_j}\\
    &=\sum_{\substack{u_1>\dots>u_l>0\\v_1,\dots,v_l>0}}e^{u_jY_j}e^{v_jX_j}q^{u_jv_j}\\
    &=\sum_{\substack{u_1>\dots>u_l>0\\v_1,\dots,v_l>0}}e^{u_jY_j}\left(e^{X_j}q^{u_j}\right)^{v_j}\\
    &=\sum_{u_1>\dots>u_l>0}E_{u_j}(Y_j)L_{v_j}(X_j).
\end{align*}
This proves the first identity. For the second identity, we apply the transformations $u_j=u_1'+\dots+u_{l-j+1}'$ and $v_j=v_{l-j+1}'-v_{l-j+2}'$ to
\begin{align*}
    \begin{vmatrix}X_1,\dots,X_l\\Y_1,\dots,Y_l\end{vmatrix}&=\sum_{\substack{u_1>\dots>u_l>0\\v_1,\dots,v_l>0}}e^{u_jY_j}e^{v_jX_j}q^{u_jv_j}.
\end{align*}
Under these transformations, we have $v'_j=v_1+\dots+v_{l-j+1}$, so that
\begin{align*}
    q^{u_1v_1+\dots+u_lv_l}&=q^{(u_1'+\dots+u_l')v_1+(u_1'+\dots+u_{l-1}')v_1+\dots+(u_1'+u_2')v_{l-1}+u_1'v_l}\\
    &=q^{u_1'(v_1+\dots+v_l)+u_2'(v_1+\dots+v_{l-1})+\dots+u_{l-1}'(v_1+v_2)+u_l'v_l}\\
    &=q^{u_1'v_1'+u_2'v_2'+\dots+u_l'v_l'}.
\end{align*}
Additionally, the conditions $u_1>\dots>u_l>0$ and $v_1,\dots,v_l>0$ become $u_1',\dots,u_l'>0$ and $v_1'>\dots>v_l'>0$. So we have
\begin{align*}
    \begin{vmatrix}X_1,\dots,X_l\\Y_1,\dots,Y_l\end{vmatrix}&=\sum_{\substack{v_1'>\dots>v_l'>0\\u_1',\dots,u_l'>0}}e^{(v_{l-j+1}'-v_{l-j+2}')X_j}e^{(u_1'+\dots+u_{l-j+1}')Y_j}q^{u_j'v_j'}\\
    &=\sum_{\substack{v_1'>\dots>v_l'>0\\u_1',\dots,u_l'>0}}e^{v_j'(X_{l-j+1}-X_{l-j+2})}e^{u_j'(Y_1+\dots+Y_{l-j+1})}q^{u_j'v_j'}\\
    &=\sum_{\substack{v_1'>\dots>v_l'>0\\u_1',\dots,u_l'>0}}E_{v_j}(X_{l-j+1}-X_{l-j+2})L_{u_j}(Y_1+\dots+Y_{l-j+1})\\
    &=\begin{vmatrix}Y_1+\dots+Y_l,\dots,Y_1+Y_2,Y_1\\X_l,X_{l-1}-X_l,\dots,X_1-X_2\end{vmatrix}.
\end{align*}
\end{proof}

\begin{corollary}
For length $l=1$ and $l=2$, respectively, we have
\begin{equation*}
    \begin{vmatrix}X\\Y\end{vmatrix}=\begin{vmatrix}Y\\X\end{vmatrix},\qquad\qquad \begin{vmatrix}X_1,X_2\\Y_1,Y_2\end{vmatrix}=\begin{vmatrix}Y_1+Y_2,Y_1\\X_2,X_1-X_2\end{vmatrix}.
\end{equation*}
\end{corollary}

==> Print.tex <==
0& 1& 2& 3& 4& 5& 6& 7& 8& 9& 10& 11& 12& 13& 14& 15& 16& 17& 18& 19& 20& 21& 22& 23& 24& 25

Hey Maaike,

Bedankt voor ons gesprek maandag! Ik heb hierdoor een beter beeld gekregen van het traineeship en van Nedap zelf. Het lijkt me ook leuk om te horen hoe de ervaringen zijn van een huidig trainee. Ik denk dat dit waardevol kan zijn voor mijn beroepskeuze. Zou het mogelijk zijn om in contact te komen met een trainee? Ik ben benieuwd hoe hij/zij dit traject ervaart.

Alvast bedankt!

Groeten,
Abel

==> Proberen/Nieuw.tex <==
\subsection{Alternative proof}
\noindent For two integers $S,R\geq l$ we define the generating functions
\begin{align*}
    \sgen{X_1,\dots,X_l\\Y_1,\dots,Y_l}&=\sum_{\substack{s_1,\dots,s_l>0\\ s_1+\dots+s_l=S\\r_1,\dots,r_l\geq 0\\r_1+\dots+r_l=R}}\bbracket{s_1,\dots,s_l\\r_1,\dots,r_l}X_1^{s_1-1}\cdots X_l^{s_l-1}Y_1^{r_1}\cdots Y_l^{r_l},\\
    \pgen{X_1,X_2\\Y_1,Y_2}&=\sum_{\substack{s_1,s_2>0\\ s_1+s_2=S\\r_1,r_2\geq 0\\r_1+r_2=R}}\bbracket{s_1\\r_1}\bbracket{s_2\\r_2}X_1^{s_1-1}X_2^{s_2-1}Y_1^{r_1} Y_2^{r_2}.
\end{align*}
These functions satisfy the following relations (modulo length $1$ bi-brackets)
\begin{align*}
    \pgen{X_1,X_2\\Y_1,Y_2}&=\sgen{X_1,X_2\\Y_1,Y_2}+\sgen{X_2,X_1\\Y_2,Y_1}\\
    \pgen{X_1,X_2\\Y_1,Y_2}&=\sgen{X_1+X_2,X_1\\Y_2,Y_1-Y_2}+\sgen{X_1+X_2,X_2\\Y_1,Y_2-Y_1},
\end{align*}
for integers $n_1+n_2=S$ and $m_1+m_2=R$. Let us assume that $S+R$ is odd, so that
\begin{equation*}
    \sgen{-X_1,-X_2\\-Y_1,-Y_2}=-\sgen{X_1,X_2\\Y_1,Y_2}.
\end{equation*}
We calculate
\begin{align*}
    &\hphantom{=}\pgen{X_1,X_2\\Y_1,Y_2}-\pgen{-X_1,X_2\\-Y_1,Y_2}+\pgen{X_2-X_1,X_2\\-Y_1,Y_2+Y_1}+\pgen{X_2-X_1,-X_1\\Y_2,-Y_1-Y_2}
    \\&\qquad+\pgen{X_1-X_2,X_2\\Y_1,Y_1+Y_2}-\pgen{X_2-X_1,X_1\\Y_2,Y_1+Y_2}\\
    % 
    &=\pgen{X_1,X_2\\Y_1,Y_2}-\pgen{-X_1,X_2\\-Y_1,Y_2}+\pgen{X_2-X_1,X_2\\-Y_1,Y_2+Y_1}+\pgen{X_2-X_1,-X_1\\Y_2,-Y_1-Y_2}
    \\&\qquad+\sgen{X_1,X_1-X_2\\Y_1+Y_2,-Y_2}+\sgen{X_1,X_2\\Y_1,Y_2}-\sgen{X_2,X_2-X_1\\Y_1+Y_2,-Y_1}-\sgen{X_2,X_1\\Y_2,Y_1}\\
    % 
    &=\pgen{X_1,X_2\\Y_1,Y_2}-\pgen{-X_1,X_2\\-Y_1,Y_2}+\pgen{X_2-X_1,X_2\\-Y_1,Y_2+Y_1}+\pgen{X_2-X_1,-X_1\\Y_2,-Y_1-Y_2}
    \\&\qquad+\sgen{X_1,X_1-X_2\\Y_1+Y_2,-Y_2}+2\sgen{X_1,X_2\\Y_1,Y_2}-\sgen{X_2,X_2-X_1\\Y_1+Y_2,-Y_1}-\pgen{X_1,X_2\\Y_1,Y_2}\\
    % 
    &=-\sgen{X_2-X_1,-X_1\\Y_2,-Y_1-Y_2}-\sgen{X_2-X_1,X_2\\-Y_1,Y_2+Y_1}+\pgen{X_2-X_1,X_2\\-Y_1,Y_2+Y_1}+\pgen{X_2-X_1,-X_1\\Y_2,-Y_1-Y_2}
    \\&\qquad+\sgen{X_1,X_1-X_2\\Y_1+Y_2,-Y_2}+2\sgen{X_1,X_2\\Y_1,Y_2}-\sgen{X_2,X_2-X_1\\Y_1+Y_2,-Y_1},
\end{align*}
which is
\begin{align*}
    &=-\pgen{X_2-X_1,-X_1\\Y_2,-Y_1-Y_2}+\sgen{-X_1,X_2-X_1\\-Y_1-Y_2,Y_2}-\pgen{X_2-X_1,X_2\\-Y_1,Y_2+Y_1}+\sgen{X_2,X_2-X_1\\Y_2+Y_1,-Y_1}\\&\quad+\pgen{X_2-X_1,X_2\\-Y_1,Y_2+Y_1}+\pgen{X_2-X_1,-X_1\\Y_2,-Y_1-Y_2}+\sgen{X_1,X_1-X_2\\Y_1+Y_2,-Y_2}+2\sgen{X_1,X_2\\Y_1,Y_2}-\sgen{X_2,X_2-X_1\\Y_1+Y_2,-Y_1}\\
    % 
    % &=-\pgen{X_2-X_1,-X_1\\Y_2,-Y_1-Y_2}-\pgen{X_2-X_1,X_2\\-Y_1,Y_2+Y_1}\\&\quad+\pgen{X_2-X_1,X_2\\-Y_1,Y_2+Y_1}+\pgen{X_2-X_1,-X_1\\Y_2,-Y_1-Y_2}+2\sgen{X_1,X_2\\Y_1,Y_2}\\
    % % 
    &=2\sgen{X_1,X_2\\Y_1,Y_2}.
\end{align*}
This means that we have
\begin{align*}
    \sgen{X_1,X_2\\Y_1,Y_2}&=\frac{1}{2}\left(\pgen{X_1,X_2\\Y_1,Y_2}-\pgen{-X_1,X_2\\-Y_1,Y_2}+\pgen{X_2-X_1,X_2\\-Y_1,Y_2+Y_1}+\pgen{X_2-X_1,-X_1\\Y_2,-Y_1-Y_2}\right.
    \\&\left.\qquad+\pgen{X_1-X_2,X_2\\Y_1,Y_1+Y_2}-\pgen{X_2-X_1,X_1\\Y_2,Y_1+Y_2}\right),
\end{align*}
which also proves the odd-weight theorem:
\begin{theorem}
For integers $s_1,s_2>0$ and $r_1,r_2\geq 0$ so that $s_1+s_2+r_1+r_2$ is odd, we have
\begin{equation*}
    \bbracket{s_1,s_2\\r_1,r_2}\in \MD.
\end{equation*}
\end{theorem}

























% Let $S$ be odd. For $1\leq n\leq S-1$ we have
% \begin{equation*}
%     \bbracket{S-n,n}\equiv\bbracket{S-n}\bbracket{n}-\bbracket{n,S-n}-\bbracket{S}
% \end{equation*}
% and
% \begin{align*}
%     \bbracket{S-n}\bbracket{n}\equiv\sum_{1\leq l\leq S-1}{S-1-l\choose n-1}\bbracket{S-l,l}+\sum_{1\leq l\leq S-1}{S-1-l\choose S-1-n}\bbracket{S-l,l}.
% \end{align*}
% Here, ``$\equiv$" means modulo brackets of weight $<S$. Filling in gives us
% \begin{align*}
%     \bbracket{S-n}\bbracket{n}&\equiv\sum_{1\leq l\leq S-1}{S-1-l\choose n-1}\bbracket{S-l,l}+\sum_{1\leq l\leq S-1}{S-1-l\choose S-1-n}\big(\bbracket{S-l}\bbracket{l}-\bbracket{l,S-l}-\bbracket{S}\big)\\
%     &=\sum_{1\leq l\leq S-1}{S-1-l\choose n-1}\bbracket{S-l,l}-\sum_{1\leq l\leq S-1}{S-1-l\choose n-l}\bbracket{l,S-l}\\
%     &\qquad+\sum_{1\leq l\leq S-1}{S-1-l\choose n-l}\bbracket{l}\bbracket{S-l}-\bbracket{S}{S-1 \choose n-1}.
% \end{align*}
% So we have
% \begin{align*}
%     \bbracket{S-n}\bbracket{n}&+{S-1 \choose n-1}\bbracket{S}-\sum_{1\leq l\leq S-1}{S-1-l\choose n-l}\bbracket{l}\bbracket{S-l}\\&\equiv\sum_{1\leq l\leq S-1}{S-1-l\choose n-1}\bbracket{S-l,l}-\sum_{1\leq l\leq S-1}{S-1-l\choose n-l}\bbracket{l,S-l}.
% \end{align*}
% This means that
% \begin{align*}
%     \vec{y}=(P_{S-1}-P_{S-1}^\sr)\vec{x},
% \end{align*}
% with
% \begin{equation*}
%     \vec{y}_n=\bbracket{S-n}\bbracket{n}+{S-1 \choose n-1}\bbracket{S}-\sum_{1\leq l\leq S-1}{S-1-l\choose n-l}\bbracket{l}\bbracket{S-l}
% \end{equation*}
% so that
% \begin{equation*}
%     \frac{1}{2}\big(J_{S-1}+Q_{S-1}-Q_{S-1}^\sr\big)\vec{y}=\vec{x}.
% \end{equation*}
% \clearpage
% \noindent We have
% \begin{align*}
%     (J_{S-1}\vec{y})_n=(-1)^{n+1}\left(\bbracket{S-n}\bbracket{n}+{S-1 \choose n-1}\bbracket{S}-\sum_{1\leq l\leq S-1}{S-1-l\choose n-l}\bbracket{l}\bbracket{S-l}\right)
% \end{align*}
% and
% \begin{align*}
%     (Q_{S-1}\vec{y})_n&=\sum_{k=1}^{S-1}(-1)^{S+n+k}{k-1\choose S-1-n}\left(\bbracket{S-k}\bbracket{k}+{S-1 \choose k-1}\bbracket{S}-\sum_{1\leq l\leq S-1}{S-1-l\choose k-l}\bbracket{l}\bbracket{S-l}\right)\\
%     &=\sum_{k=1}^{S-1}(-1)^{S+n+k}{k-1\choose S-1-n}\bbracket{S-k}\bbracket{k}+\bbracket{S}\sum_{k=1}^{S-1}(-1)^{S+n+k}{k-1\choose S-1-n}-(Q_{S-1}P^\sr_{S-1}\vec{z})_n\\
%     &=\sum_{k=1}^{S-1}(-1)^{S+n+k}{k-1\choose S-1-n}\bbracket{S-k}\bbracket{k}+\bbracket{S}\sum_{k=1}^{S-1}(-1)^{S+n+k}{k-1\choose S-1-n}\\
%     &\qquad-\sum_{k=1}^{S-1}(-1)^{n+1}{S-1-k\choose n-1}\bbracket{S-k}\bbracket{k}
% \end{align*}
% and
% \begin{align*}
%     (Q_{S-1}^\sr\vec{y})_n&=\sum_{k=1}^{S-1}(-1)^{S+n+k}{S-1-k\choose n-1}\left(\bbracket{S-k}\bbracket{k}+{S-1 \choose k-1}\bbracket{S}-\sum_{1\leq l\leq S-1}{S-1-l\choose k-l}\bbracket{l}\bbracket{S-l}\right)\\
%     &=\sum_{k=1}^{S-1}(-1)^{S+n+k}{S-1-k\choose n-1}\bbracket{S-k}\bbracket{k}+\bbracket{S}\sum_{k=1}^{S-1}(-1)^{S+n+k}{S-1-k\choose n-1}-(Q^\sr_{S-1}P^\sr_{S-1}\vec{z})_n\\
%     &=\sum_{k=1}^{S-1}(-1)^{S+n+k}{S-1-k\choose n-1}\bbracket{S-k}\bbracket{k}+\bbracket{S}\sum_{k=1}^{S-1}(-1)^{S+n+k}{S-1-k\choose n-1}-\bbracket{S-n}\bbracket{n}
% \end{align*}
% Summary:
% \begin{align*}
%     (J_{S-1}\vec{y})_n&=(-1)^{n+1}\left(\bbracket{S-n}\bbracket{n}+{S-1 \choose n-1}\bbracket{S}-\sum_{k=1}^{S-1}{S-1-k\choose n-k}\bbracket{k}\bbracket{S-k}\right)\\
%     % 
%     (Q_{S-1}\vec{y})_n&=\sum_{k=1}^{S-1}(-1)^{n+k+1}{k-1\choose S-1-n}\bbracket{S-k}\bbracket{k}+\bbracket{S}\sum_{k=1}^{S-1}(-1)^{n+k+1}{k-1\choose S-1-n}\\
%     &\qquad-\sum_{k=1}^{S-1}(-1)^{n+1}{S-1-k\choose n-1}\bbracket{S-k}\bbracket{k}\\
%     % 
%     (Q_{S-1}^\sr\vec{y})_n&=\sum_{k=1}^{S-1}(-1)^{n+k+1}{S-1-k\choose n-1}\bbracket{S-k}\bbracket{k}+\bbracket{S}\sum_{k=1}^{S-1}(-1)^{n+k+1}{S-1-k\choose n-1}-\bbracket{S-n}\bbracket{n}
% \end{align*}




==> Proberen/ToDo.tex <==
\section{To-Do}
\begin{enumerate}
    % \item Het geval $S=3$ en $R=1$ (of $S=R=2$) uitwerken. Welke relaties hebben we nog nodig? 
    % \item Uitrekenen wat voor extra term(en) $T(\hat{X_1},\hat{X_2})\cdot T(X_1,\dots,X_l)$ geeft (en vergelijk deze met de $R_l$ termen en de derivatives). Waarschijnlijk met de operator $\restr{c\frac{\del}{\del \hat{X_1}} +c'\frac{\del}{\del \hat{X_2}}}{X_1=X_2=0}$ ipv $\restr{\frac{\del}{\del X}}{X=0}$.\label{iets3}
    % \item \label{iets1}Reken $\begin{vmatrix}X\\Y\end{vmatrix}\cdot\begin{vmatrix}X_1,\dots,X_l\\Y_1,\dots,Y_l\end{vmatrix}$ uit, en kijk of de operator $c\del X+c'\del Y$ iets interessants geeft (of een andere operator).
    \item Geef een alternatief bewijs voor het binomiaal lemma, met de hypergeometrische functies $_2F_1$. 
    \item Bepaal de rang van de even weight gevallen, en vind er een formule bij.\label{iets2}
    \item Verbeter de notes van Wadim.
    \item Schrijf een \textit{long introduction of $\MD$ and $\BD$ algebras}.
\end{enumerate}


\ref{iets1}: Dit lijkt niet te werken, voornamelijk omdat de termen waar nieuwe relaties uit zouden moeten komen, altijd in het 
\begin{equation*}
    \begin{bmatrix}X,x\\Y,y\end{bmatrix}+\begin{bmatrix}x,X\\y,Y\end{bmatrix}
\end{equation*}
gedeelte voorkomen (maar dit is symmetrisch, en alle symmetrische relaties hebben we al).\\

\ref{iets2} Voor de Dim(Ker) van zowel Tess($i,j$) als Red($i,j$) zijn er patronen te vinden. De dimensie van de kern van Red($i,j$) stijgt met ...

\ref{iets3} Geprobeerd te berekenen: $T(X,Y)\cdot T(Z)$: Je hebt 
\begin{equation*}
    R_2(Z,X,Y)=\sum_{n_1,n_2>0}e^{n_1(Z+X)+n_2Y}\frac{q^{n_1}}{(1-q^{n_1})^2}\frac{q^{n_1+n_2}}{1-q^{n_1+n_2}}+\sum_{n_1,n_2>0}e^{n_1(Z+X)+n_2(Z+Y)}\frac{q^{n_1}}{1-q^{n_1}}\frac{q^{n_1+n_2}}{(1-q^{n_1+n_2})^2}
\end{equation*}

\subsubsection{Introductie}
Dingen die ge\"introduceerd moeten worden:
\begin{enumerate}
    \item De multiple zeta values $\zeta(s_1,\dots,s_l)$ and the relations between them and the shuffle and stuffle algebras.
    \item Relaties tussen multiple zeta values, problemen stellen over multiple zeta values. Waarom hebben we de $q$-analogen nodig?
    \item Verscheidene $q$-analogen: $\tilde{\zeta_q},\zeta_q\mathfrak{z}_q$. Ook de brackets van Wadim introduceren en de directe link tussen de brackets bewijzen. Zie MZF dictaat p83.
    \item Introductie over $\MD$ en $\BD$ (geintroduceerd door Bachmann). Laten zien dat dit ook een $q$-analoog is.
    \item Probleemstelling: $\MD=\BD$. Wat is er al bekend?
    \item Wat heb ik gevonden: $l=2$ en odd total weight.
\end{enumerate}
\subsection{Nog te bewijzen}
\begin{enumerate}
    \item De invariance van vermenigvuldiging in de monobracket case. Zie paper 2 (1309.3920), hoofdstuk 2.
    
\end{enumerate}



Ideeen:
\begin{enumerate}
    \item Misschien het bewijs van $l=2$, odd weight, aanpassen naar de algebra $Z=\{z_{s_1,r_1}\mid s_i,r_i\geq 1\}$. Vragen aan Wadim of dit netter is.
\end{enumerate}

==> Proberen/Uitleg.tex <==
\subsection*{Length $2$, Odd weight}
We know that bi-brackets of lenght $1$ are in $\MD$. The stuffle and shuffle analogues (modulo length $1$) for the bi-brackets give rise to the following equations
\begin{align*}
    0&=\begin{bmatrix}
    s_1,s_2\\
    r_1,r_2
    \end{bmatrix}+\begin{bmatrix}
    r_1,r_2\\
    s_1,s_2
    \end{bmatrix},\tag{1}\\
    0&=\sum_{\substack{1\leq j\leq s_1\\ 0\leq k\leq r_2}}{s_1+s_2-j-1 \choose s_1-j}{r_1+r_2-k \choose r_1}(-1)^{r_2-k}\begin{bmatrix}
    s_1+s_2-j,j\\
    k,r_1+r_2-k
    \end{bmatrix}\tag{2}\\
    &+\sum_{\substack{1\leq j\leq s_2\\ 0\leq k\leq r_1}}{s_1+s_2-j-1 \choose s_2-j}{r_1+r_2-k \choose r_2}(-1)^{r_1-k}\begin{bmatrix}
    s_1+s_2-j,j\\
    k,r_1+r_2-k
    \end{bmatrix}.
\end{align*}
Then, by considering all products of fixed upper and lower weight
\begin{equation*}
    \begin{bmatrix}
    s_1+s_2-n\\
    k
    \end{bmatrix}\begin{bmatrix}
    n\\
    r_1+r_2-k
    \end{bmatrix}
\end{equation*}
for $1\leq n \leq s_1+s_2-1$ and $0\leq k\leq r_1+r_2$, we get a system of linear equations, with `unknowns' 
\begin{equation*}
    \begin{bmatrix}
    s_1+s_2-n, n\\
    k, r_1+r_2-k
    \end{bmatrix}.
\end{equation*}
Computer calculations suggest that this system of linear equations can be solved for these unknowns, if the total weight $s_1+s_2+r_1+r_2$ is odd.
The matrix corresponding to this system of linear equations is given by 
\begin{equation*}
    \begin{pmatrix}
&&&&&&\\
&&&P_{n-1}\otimes Q_{m+1}+(P_{n-1}\otimes Q_{m+1})^\rho&&&\\
&&&&&&\\
\hline&&&\vline&&&\\
&&&I\quad\qquad\qquad\ \ \vline\quad\qquad\qquad I^\rho&&&\\
&&&\vline&&&
\end{pmatrix},
\end{equation*}
where $P_k$ is the matrix $(P_k)_{i,j}={k-j\choose i-1}$, $Q_k$ is the matrix $(Q_k)_{i,j}=(-1)^{i+j+1+k}{j-1\choose k-i}$ and $A^\rho$ is the horizontal reflection $A_{i,j}=A_{n+1-i,j}$, where $n$ is the number of rows of $A$. \clearpage

For example, for $s_1+s_2=7$ and $r_1+r_2=4$, we get the matrix above.\\
\begin{figure}
    \begin{center}
        \includegraphics[scale=0.75]{Knipsel.PNG}
    \end{center}
\end{figure}

Clearly, this matrix is not square, so that there are many relations between the rows (the upper part is symmetric). To remove these symmetries, I have considered the following: apply $(1)$ to $(P_{n-1}\otimes Q_{m+1})^\rho$ (i.e., a vertical reflection). The computer then suggests that we do not need the relations $(1)$ anymore (the $I\ |\ I^\rho$ part), so that we are left with a square matrix for which we have to show independence. If this matrix is proven full in rank, then the system of linear equations has a solution.\clearpage
\begin{figure}
    \begin{center}
        \includegraphics[scale=0.75]{Knipsel2.PNG}
    \end{center}
\end{figure}
Using upper weight $7$ and lower weight $4$, after the vertical reflection induced by $(1)$, we get the matrix above.

==> Proberen/Uitproberen.tex <==
\section{}
% Define the operator $D=\restr{\left(\frac{\del}{\del X}+\frac{\del}{\del Y}\right)}{X=Y=0}$. We will calculate
% \begin{equation*}
%     D\begin{vmatrix}X\\Y\end{vmatrix}\cdot\begin{vmatrix}x\\y\end{vmatrix}=D\left(\begin{vmatrix}X,x\\Y,y\end{vmatrix}+\begin{vmatrix}x,X\\y,Y\end{vmatrix}+T_2+T_3\right),
% \end{equation*}
% with 
% \begin{equation*}
%     T_2=\sum_{\substack{s_1,s_2>0\\r_1,r_2\geq 0}}{r_1+r_2\choose r_1}\begin{bmatrix}s_1+s_2\\r_1+r_2\end{bmatrix}X^{s_1-1}x^{s_2-1}Y^{r_1}y^{r_2}
% \end{equation*}
% and
% \begin{equation*}
%     T_3=\sum_{k=1}^\infty \frac{B_k}{k!}(X-x)^{k-1}\left(\begin{vmatrix}X\\Y+y\end{vmatrix}+(-1)^{k-1}\begin{vmatrix}x\\Y+y\end{vmatrix}\right).
% \end{equation*}
% We have
% \begin{align*}
%     D\begin{vmatrix}X,x\\Y,y\end{vmatrix}=\sum_{\substack{s_2>0\\r_2\geq 0}}\left(\begin{bmatrix}1,s_2\\1,r_2\end{bmatrix}+\begin{bmatrix}2,s_2\\0,r_2\end{bmatrix}\right)x^{s_2-1}y^{r_2},
% \end{align*}
% and
% \begin{align*}
%     D\begin{vmatrix}x,X\\y,Y\end{vmatrix}=\sum_{\substack{s_1>0\\r_1\geq 0}}\left(\begin{bmatrix}s_1,1\\r_1,1\end{bmatrix}+\begin{bmatrix}s_1,2\\r_1,0\end{bmatrix}\right)x^{s_1-1}y^{r_1},
% \end{align*}
% and
% \begin{align*}
%     DT_2&=D\sum_{\substack{s_1,s_2>0\\r_1,r_2\geq 0}}{r_1+r_2\choose r_1}\begin{bmatrix}s_1+s_2\\r_1+r_2\end{bmatrix}X^{s_1-1}x^{s_2-1}Y^{r_1}y^{r_2}\\
%     &=\sum_{\substack{s_2>0\\r_2\geq 0}}\left(\begin{bmatrix}s_2+2\\r_2\end{bmatrix}+(r_2+1)\begin{bmatrix}s_2+1\\r_1+1\end{bmatrix}\right)x^{s_2-1}y^{r_2},
% \end{align*}
% and
% \begin{align*}
%     D\begin{vmatrix}X\\Y+y\end{vmatrix}
% \end{align*}

We willen 
\begin{equation*}
    S_1=\frac{q^n}{(1-q^n)^2}\frac{q^{n+m}}{1-q^{n+m}}
\end{equation*}
of
\begin{equation*}
    S_2=\frac{q^n}{1-q^n}\frac{q^{n+m}}{(1-q^{n+m})^2}
\end{equation*}
omschrijven tot iets zinnigs (iets waar we $T(\ldots)$ uit kunnen halen). Deze termen komen voort uit het het product $T(X,Y)\cdot T(Z)$.\\

Het probleem: 
\begin{equation*}
    \sum_{n,m>0}e^{n(X+Z)+mY}\frac{q^n}{(1-q^n)^2}\frac{q^{n+m}}{1-q^{n+m}}+\sum_{n,m>0}e^{n(X+Z)+m(Y+Z)}\frac{q^n}{1-q^n}\frac{q^{n+m}}{(1-q^{n+m})^2}.
\end{equation*}
We hebben
\begin{align*}
    S_1&=-\frac{q^{n+m}}{(1-q^n)(1-q^m)^2} + \frac{q^{n+m}}{(1-q^m) (1-q^n)^2} + \frac{q^m\cdot q^{n+m}}{(1-q^m)^2(1-q^{m + n})}\\
    S_2&=-\frac{q^{n+m}}{(1-q^m)(1-q^{n+m})^2}+\frac{q^{n+m}}{(1-q^m)^2(1-q^n)}-\frac{q^{n+m}q^m}{(1-q^m)^2(1-q^{n+m})}
\end{align*}

\begin{align*}
    \frac{q^n}{1-q^n}\frac{q^{n+m}}{1-q^{n+m}}&=\frac{q^{n+m}}{(1-q^n)(1-q^m)}-\frac{q^{n+m}}{(1-q^m)(1-q^{n+m})}\\
    &=\frac{q^n}{(1-q^n)(1-q^{n+m})}-\frac{q^n}{1-q^n}
\end{align*}

\begin{align*}
    \frac{q^n}{1-q^n}\frac{q^{n+m}}{(1-q^{n+m})^2}&=\frac{q^{n+m}}{(1-q^n)(1-q^m)(1-q^{n+m})}-\frac{q^{n+m}}{(1-q^m)(1-q^{n+m})^2}\\
    &=\frac{q^n}{(1-q^n)(1-q^{n+m})^2}-\frac{q^n}{(1-q^n)(1-q^{n+m})}
\end{align*}

\begin{align*}
    \frac{q^n}{(1-q^n)^2}\frac{q^{n+m}}{1-q^{n+m}}&=\frac{q^{n+m}}{(1-q^n)^2(1-q^m)}-\frac{q^{n+m}}{(1-q^m)(1-q^n)(1-q^{n+m})}\\
    &=\frac{q^n}{(1-q^n)^2(1-q^{n+m})}-\frac{q^n}{(1-q^n)^2}
\end{align*}





% https://www.wolframalpha.com/input/?i=decompose+q%5E%28n%2Bm%29%2F%28%281-q%5En%29%5E2*%281-q%5E%28n%2Bm%29%29%29
% https://www.wolframalpha.com/input/?i=decompose+q%5E%28n%2Bm%29%2F%28%281-q%5En%29*%281-q%5E%28n%2Bm%29%29%5E2%29
% https://www.wolframalpha.com/input/?i=decompose+q%5E%28n%2Bm%29%2F%28%281-q%5Em%29*%281-q%5E%28n%2Bm%29%29%29
% https://www.wolframalpha.com/input/?i=q%5E%28n%2Bm%29%2F%28%281-q%5En%29%281-q%5Em%29%29-q%5E%28n%2Bm%29%2F%28%281-q%5Em%29%281-q%5E%28n%2Bm%29%29%29
% https://www.math.ru.nl/~wzudilin/MZFs2019.html


% DIE

Shufflep := function(S,R)
	s1:=S[1];
	s2:=R[1];
	r1:=S[2];
	r2:=R[2];
	
	Sum:=[];
	for j:=1 to s1 do
		for k:=0 to r2 dohttps://www.overleaf.com/project/5d84e300baccba0001792549
			Append(~Sum,<Binomial(s1+s2-j-1,s1-j)*Binomial(r1+r2-k,r1)*(-1)^(r2-k),[s1+s2-j,j],[k,r1+r2-k]>);
		end for;
	end for;
	for j:=1 to s2 do
		for k:=0 to r1 do
			Append(~Sum,<Binomial(s1+s2-j-1,s2-j)*Binomial(r1+r2-k,r2)*(-1)^(r1-k),[s1+s2-j,j],[k,r1+r2-k]>);
		end for;
	end for;
	return Sum;
end function;

Cleanup:= function(Sum)
	T:=Sum;
	sum:=[];
	for w in Sum do
		e:=0;
		for v in T do
			if v[2] eq w[2] and v[3] eq w[3] then
				e:=e+v[1];
				Exclude(~T,v);
			end if;
		end for;
		if e ne 0 then
			Append(~sum,<e,w[2],w[3]>);
		end if;
	end for;
	return sum;
end function;

Shuffle := function(S,R)
	return Cleanup(Shufflep(S,R));
end function;

Stuffle := function(S,R)
	return [<1,[S[1],R[1]],[S[2],R[2]]>,<1,[R[1],S[1]],[R[2],S[2]]>];
end function;


Stuffle2 := function(S,R)
	X:=[<RationalField()!1,[S[1],R[1]],[S[2],R[2]]>,<RationalField()!1,[R[1],S[1]],[R[2],S[2]]>];
	Append(~X,<Binomial(S[2]+R[2],S[2]),[S[1]+R[1]],[S[2]+R[2]]>);
	for j:=1 to S[1] do
		Append(~X,<Binomial(S[2]+R[2],S[2])*Binomial(S[1]+R[1]-j-1,S[1]-j)*(-1)^(R[1]-1)*Bernoulli(S[1]+R[1]-j)/Factorial(S[1]+R[1]-j),[j],[S[2]+R[2]]>);
	end for;
	for j:=1 to R[1] do
		Append(~X,<Binomial(S[2]+R[2],S[2])*Binomial(S[1]+R[1]-j-1,R[1]-j)*(-1)^(S[1]-1)*Bernoulli(S[1]+R[1]-j)/Factorial(S[1]+R[1]-j),[j],[S[2]+R[2]]>);
	end for;
	return Cleanup(X);
end function;


Shuffle2 := function(S,R)
	X:=Shuffle(S,R);
	Append(~X,<Binomial(S[1]+S[2]-2,S[1]-1),[S[1]+S[2]-1],[R[1]+R[2]+1]>);
	return X;
end function;
	


Bas := function(n,m)
	list:=[];
	for j:=1 to n-1 do
		for k:=0 to m do
			Append(~list, <[n-j,m-k],[j,k]>);
		end for;
	end for;
	list;
	list2:=[];
	for j:=1 to n-1 do
		for k:=0 to m do
			Append(~list2, <[n-j,j],[m-k,k]>);
		end for;
	end for;
	list2;
	T:=[];
	for v in list do
		Append(~T,Shuffle(v[1],v[2]));
	end for;
	for v in list do
		Append(~T,Stuffle(v[1],v[2]));
	end for;
	
	X:=[];
	for i:=1 to #list2 do
		Append(~X,0);
	end for;
	//list2;
	Z:=[];
	for t in T do
		Y:=X;
		for u in t do
			Y[Index(list2,<u[2],u[3]>)]:=u[1];
		end for;
		Append(~Z,Y);
	end for;
	
	
	return Matrix(RationalField(),#T,#list2,Z);
	
end function;

Diff := function(S,R)
	return [<S[1]*(R[1]+1),[S[1]+1,S[2]],[R[1]+1,R[2]]>,<S[2]*(R[2]+1),[S[1],S[2]+1],[R[1],R[2]+1]>];
end function;




Bas2:= function(n,m);
	M:=Bas(n,m);
	list:=[];
	for j:=1 to n-2 do
		for k:=0 to m-1 do
			Append(~list, <[n-1-j,j],[m-1-k,k]>);
		end for;
	end for;
	
	list2:=[];
	for j:=1 to n-1 do
		for k:=0 to m do
			Append(~list2, <[n-j,j],[m-k,k]>);
		end for;
	end for;
	
	X:=[];
	for i:=1 to #list2 do
		Append(~X,0);
	end for;
	Z:=[];
	//list2;
	for t in list do
		Y:=X;
		for u in Diff(t[1],t[2]) do
			Y[Index(list2,<u[2],u[3]>)]:=u[1];
		end for;
		Append(~Z,Y);
	end for;
	
	N:=Matrix(RationalField(),#list,#list2,Z);
	return VerticalJoin(M,N);
end function;
	
	
	
Partition := function(S,R)
	Part:=[];
	for j:=0 to R[1] do
		for k:=0 to S[2]-1 do
			Append(~Part,<(-1)^k*Binomial(S[1]-1+k,k)*Binomial(R[2]+j,j),[R[2]+j+1,R[1]-j+1],[S[2]-1-k,S[1]-1+k]>);
		end for;
	end for;
	return Part;
end function;



Bas3:= function(n,m)
	M:=DiagonalJoin(Bas2(n,m),Bas2(m+2,n-2));
	
	list2:=[];
	for j:=1 to n-1 do
		for k:=0 to m do
			Append(~list2, <[n-j,j],[m-k,k]>);
		end for;
	end for;
	for j:=1 to m+1 do
		for k:=0 to n-2 do
			Append(~list2, <[m+2-j,j],[n-2-k,k]>);
		end for;
	end for;
	
	X:=[];
	for i:=1 to #list2 do
		Append(~X,0);
	end for;
	
	Z:=[];
	for t in list2 do
		Y:=X;
		for u in Partition(t[1],t[2]) do
			Y[Index(list2,<u[2],u[3]>)]:=-u[1];
		end for;
		Y[Index(list2,t)]:=1;
		Append(~Z,Y);
	end for;
	
	N:=Matrix(RationalField(),#list2,#list2,Z);

	return VerticalJoin(M,N);
end function;



Toetsje := function(M)
	return Ncols(M)-Rank(M);
end function;

DECIMALEN:=50;


Bie := function(n,m)
	list2:=[];
	for j:=1 to n-1 do
		for k:=0 to m do
			Append(~list2, <[n-j,j],[m-k,k]>);
		end for;
	end for;
	//list2;
	X:=[];
	for u in list2 do
		p:=BIB(u[1],u[2]);
		for i:=0 to DECIMALEN do
			Append(~X,Coefficient(p,i));
		end for;
	end for;
	M:=Matrix(RationalField(),#list2,DECIMALEN+1,X);
	return M;
end function;

Bie2 :=function(n,m)
	return KernelMatrix(Bie(n,m));
end function;


	
Bas4 := function(n,m)
	return VerticalJoin(Bas(n,m),KernelMatrix(Bie(n,m)));
end function;
	
	
	
Totaal := function(n)
	M:=Matrix(RationalField(),0,0,[]);
	
	for i:=2 to n do
		M:=DiagonalJoin(M,Bas2(i,n-i));
	end for;

	//M;
	list2:=[];
	for N:=2 to n do
		for j:=1 to N-1 do
			for k:=0 to n-N do
				Append(~list2, <[N-j,j],[n-N-k,k]>);
			end for;
		end for;
	end for;
	//list2;
	X:=[];
	for u in list2 do
		p:=BIB(u[1],u[2]);
		for i:=0 to DECIMALEN do
			Append(~X,Coefficient(p,i));
		end for;
	end for;
	N:=KernelMatrix(Matrix(RationalField(),#list2,DECIMALEN+1,X));
	
	
	return VerticalJoin(M,N);
end function;
	
	
Totaal2 := function(n)
	M:=Matrix(RationalField(),0,0,[]);
	for j:=n-1 to n do
		for i:=2 to j do
			M:=DiagonalJoin(M,Bas2(i,j-i));
		end for;
	end for;
	//M;
	list2:=[];
	for K:=n-1 to n do
		for N:=2 to K do
			for j:=1 to N-1 do
				for k:=0 to K-N do
					Append(~list2, <[N-j,j],[K-N-k,k]>);
				end for;
			end for;
		end for;
	end for;
	list2;
	X:=[];
	for u in list2 do
		p:=BIB(u[1],u[2]);
		for i:=0 to DECIMALEN do
			Append(~X,Coefficient(p,i));
		end for;
	end for;
	N:=KernelMatrix(Matrix(RationalField(),#list2,DECIMALEN+1,X));
	
	
	return VerticalJoin(M,N);
end function;




Totaal3 := function(n)
	M:=Matrix(RationalField(),0,0,[]);
	
	for i:=2 to n do
		M:=DiagonalJoin(M,Bas2(i,n-i));
	end for;

	//M;
	list2:=[];
	for N:=2 to n do
		for j:=1 to N-1 do
			for k:=0 to n-N do
				Append(~list2, <[N-j,j],[n-N-k,k]>);
			end for;
		end for;
	end for;
	for i:=3 to n do
		K:=[<[s1,s2,s3],[r1,r2,r3]> : s1,s2,s3,r1,r2,r3 in [0..Min(i,n-i)] | r1+r2+r3 eq n-i and s1+s2+s3 eq i and s1 ge 1 and s2 ge 1 and s3 ge 1];
		list2:=list2 cat K;
	end for;
	list2;
	X:=[];
	for u in list2 do
		p:=BIB(u[1],u[2]);
		for i:=0 to DECIMALEN do
			Append(~X,Coefficient(p,i));
		end for;
	end for;
	N:=KernelMatrix(Matrix(RationalField(),#list2,DECIMALEN+1,X));
	M,N;
	
	return VerticalJoin(M,N);
end function;





S:=5;
R:=2;

//K:=[<[s1,s2,s3],[r1,r2,r3]> : s1,s2,s3,r1,r2,r3 in [0..10] | s1 ge 1 and s2 ge 1 and s3 ge 1 and s1+s2+s3 eq S and r1+r2+r3 eq R];


Tet := function(n,m)
	M:=DiagonalJoin(Bas2(n,m),Bas2(m+2,n-2));
	list2:=[];
	for j:=1 to n-1 do
		for k:=0 to m do
			Append(~list2, <[n-j,j],[m-k,k]>);
		end for;
	end for;
	for j:=1 to m+1 do
		for k:=0 to n-2 do
			Append(~list2, <[m+2-j,j],[n-2-k,k]>);
		end for;
	end for;
	
	X:=[];
	for i:=1 to #list2 do
		Append(~X,0);
	end for;
	
	Z:=[];
	for t in list2 do
		Y:=X;
		for u in Partition(t[1],t[2]) do
			Y[Index(list2,<u[2],u[3]>)]:=-u[1];
		end for;
		Y[Index(list2,t)]:=1;
		Append(~Z,Y);
	end for;
	
	N:=Matrix(RationalField(),#list2,#list2,Z);
	N:=VerticalJoin(M,N);
	
	X:=[];
	for u in list2 do
		p:=BIB(u[1],u[2]);
		for i:=0 to DECIMALEN do
			Append(~X,Coefficient(p,i));
		end for;
	end for;
	K:=KernelMatrix(Matrix(RationalField(),#list2,DECIMALEN+1,X));
	
	return VerticalJoin(N,K);
end function;

/*
for i:=2 to 10 do
	for j:=0 to 8 do
		if IsEven(i+j) then
			<i,j>;
			Toetsje(Tet(i,j));
		end if;
	end for;
end for;
*/

//let op, de S en R werken hier anders dan in Stuffle2!
Stuffle3 := function(s,r)
	X:=[<RationalField()!1,[s[1],s[2],s[3]],[r[1],r[2],r[3]]>,<RationalField()!1,[s[1],s[3],s[2]],[r[1],r[3],r[2]]>,<RationalField()!1,[s[3],s[1],s[2]],[r[3],r[1],r[2]]>];
	Append(~X,<Binomial(r[1]+r[3],r[1]),[s[1]+s[3],s[2]],[r[1]+r[3],r[2]]>);
	Append(~X,<Binomial(r[3]+r[2],r[2]),[s[1],s[2]+s[3]],[r[1],r[2]+r[3]]>);
	
	for j:=1 to s[1] do
		Append(~X,<Binomial(r[1]+r[3],r[1])*Binomial(s[1]+s[3]-j-1,s[1]-j)*(-1)^(s[3]-1)*Bernoulli(s[1]+s[3]-j)/Factorial(s[1]+s[3]-j),[j,s[2]],[r[1]+r[3],r[2]]>);
	end for;
	
	for j:=1 to s[3] do
		Append(~X,<Binomial(r[1]+r[3],r[1])*Binomial(s[1]+s[3]-j-1,s[2]-j)*(-1)^(s[1]-1)*Bernoulli(s[1]+s[3]-j)/Factorial(s[1]+s[3]-j),[j,s[2]],[r[1]+r[3],r[2]]>);
	end for;
	
	for j:=1 to s[2] do
		Append(~X,<Binomial(r[2]+r[3],r[2])*Binomial(s[2]+s[3]-j-1,s[2]-j)*(-1)^(s[3]-1)*Bernoulli(s[2]+s[3]-j)/Factorial(s[2]+s[3]-j),[s[1],j],[r[1],r[2]+r[3]]>);
	end for;
	
	for j:=1 to s[3] do
		Append(~X,<Binomial(r[2]+r[3],r[2])*Binomial(s[2]+s[3]-j-1,s[2]-j)*(-1)^(s[2]-1)*Bernoulli(s[2]+s[3]-j)/Factorial(s[2]+s[3]-j),[s[1],j],[r[1],r[2]+r[3]]>);
	end for;
	
	return Cleanup(X);
end function;




% EXPANSIONS



DECIMALEN:=50;



R:=RationalField();
T<x>:=PowerSeriesRing(R);
EulerCoef := function(n,k);
	C:=0;
	for i:=0 to k do
		C:=C+(-1)^i*Binomial(n+1,i)*(k+1-i)^n;
	end for;
	return C;
end function;

Euler := function(n,N);
	P:=0;
	for k:=0 to n do
		P:=P+EulerCoef(n,k)*x^(N*k);
	end for;
	return P;
end function;

EulerP := function(n);
	P:=0;
	for k:=0 to n do
		P:=P+EulerCoef(n,k)*x^k;
	end for;
	return P;
end function;



R:=RationalField();
K<q>:=PowerSeriesRing(R);
BiB := function()
	return true;
end function;

BiB := function(BB,S1,R1,N,Precision)
	K<q>:=PowerSeriesRing(R,Precision);
	l:=#S1;
	if N lt l then
		return K!0;
	end if;
	S2:=Remove(S1,1);
	R2:=Remove(R1,1);
	if l gt 1 then
		K1:=N^(R1[1])*q^N*Euler(S1[1]-1,N);
		K2:=Factorial(R1[1])*Factorial(S1[1]-1)*(1-q^N)^(S1[1]);
		BB:=$$(BB,S1,R1,N-1,Precision)+(K1)/(K2)*$$(BB,S2,R2,N-1,Precision);
	else
		K1:=N^(R1[1])*q^N*Euler(S1[1]-1,N);
		K2:=Factorial(R1[1])*Factorial(S1[1]-1)*(1-q^N)^(S1[1]);
		BB:=$$(BB,S1,R1,N-1,Precision)+(K1)/(K2);
	end if;
	
	return BB;
end function;


BiBp := function(BB,S1,R1,N,Precision)
	K<q>:=PowerSeriesRing(R,Precision);
	l:=#S1;
	if N lt l then
		return K!0;
	end if;
	S2:=Remove(S1,1);
	R2:=Remove(R1,1);
	if l gt 2 then
		if N eq l then
			K1:=N^(R1[1])*q^N*Euler(S1[1]-1,N);
			K2:=Factorial(R1[1])*Factorial(S1[1]-1)*(1-q^N)^(S1[1]);
			BB:=$$(BB,S1,R1,N-1,Precision)+(K1)/(K2)*$$(BB,S2,R2,N-1,Precision);
		else
			S3:=Remove(S2,1);
			R3:=Remove(R2,1);
			
			K1:=N^(R1[1])*q^N*Euler(S1[1]-1,N);
			K2:=Factorial(R1[1])*Factorial(S1[1]-1)*(1-q^N)^(S1[1]);
			
			K3:=(N-1)^(R1[1])*q^(N-1)*Euler(S1[1]-1,N-1);
			K4:=Factorial(R1[1])*Factorial(S1[1]-1)*(1-q^(N-1))^(S1[1]);
			
			K5:=(N-1)^(R2[1])*q^(N-1)*Euler(S2[1]-1,N-1);
			K6:=Factorial(R2[1])*Factorial(S2[1]-1)*(1-q^(N-1))^(S2[1]);
			
			BB:=$$(BB,S1,R1,N-2,Precision)+(K1/K2+K3/K4)*$$(BB,S2,R2,N-2,Precision)+(K1/K2)*(K5/K6)*$$(BB,S3,R3,N-2,Precision);
		end if;
	elif l eq 2 then
		K1:=N^(R1[1])*q^N*Euler(S1[1]-1,N);
		K2:=Factorial(R1[1])*Factorial(S1[1]-1)*(1-q^N)^(S1[1]);
		BB:=$$(BB,S1,R1,N-1,Precision)+(K1)/(K2)*$$(BB,S2,R2,N-1,Precision);
	else
		K1:=N^(R1[1])*q^N*Euler(S1[1]-1,N);
		K2:=Factorial(R1[1])*Factorial(S1[1]-1)*(1-q^N)^(S1[1]);
		BB:=$$(BB,S1,R1,N-1,Precision)+(K1)/(K2);
	end if;
	return BB;
end function;

BiBracketsp := function(S1,R1,N)
	Precision:=N+1;
	K<q>:=PowerSeriesRing(R,Precision);
	BB:=0;
	//t:=Cputime();
	B:=BiBp(BB,S1,R1,N,Precision);
	//Cputime(t);
	return B;
end function;

BIBp:=function(S1,R1)
	return BiBracketsp(S1,R1,DECIMALEN);
end function;

MOBp:=function(S1)
	R1:=[];
	for i:=1 to #S1 do
		Append(~R1,0);
	end for;
	return BIBp(S1,R1);
end function;


BiBpp := function(BB,S1,R1,N,Precision)
	K<q>:=PowerSeriesRing(R,Precision);
	l:=#S1;
	if N lt l then
		return K!0;
	end if;
	S2:=Remove(S1,1);
	R2:=Remove(R1,1);
	if l gt 3 then
		if N eq l then
			K1:=N^(R1[1])*q^N*Euler(S1[1]-1,N);
			K2:=Factorial(R1[1])*Factorial(S1[1]-1)*(1-q^N)^(S1[1]);
			BB:=$$(BB,S1,R1,N-1,Precision)+(K1)/(K2)*$$(BB,S2,R2,N-1,Precision);
		elif N eq l+1 then
			S3:=Remove(S2,1);
			R3:=Remove(R2,1);
			
			K1:=N^(R1[1])*q^N*Euler(S1[1]-1,N);
			K2:=Factorial(R1[1])*Factorial(S1[1]-1)*(1-q^N)^(S1[1]);
			
			K3:=(N-1)^(R1[1])*q^(N-1)*Euler(S1[1]-1,N-1);
			K4:=Factorial(R1[1])*Factorial(S1[1]-1)*(1-q^(N-1))^(S1[1]);
			
			K5:=(N-1)^(R2[1])*q^(N-1)*Euler(S2[1]-1,N-1);
			K6:=Factorial(R2[1])*Factorial(S2[1]-1)*(1-q^(N-1))^(S2[1]);
			
			BB:=$$(BB,S1,R1,N-2,Precision)+(K1/K2+K3/K4)*$$(BB,S2,R2,N-2,Precision)+(K1/K2)*(K5/K6)*$$(BB,S3,R3,N-2,Precision);
		else
			S3:=Remove(S2,1);
			R3:=Remove(R2,1);
			S4:=Remove(S3,1);
			R4:=Remove(R3,1);
			//C_l^N
			K1:=N^(R1[1])*q^N*Euler(S1[1]-1,N);
			K2:=Factorial(R1[1])*Factorial(S1[1]-1)*(1-q^N)^(S1[1]);
			//C_l^N-1
			K3:=(N-1)^(R1[1])*q^(N-1)*Euler(S1[1]-1,N-1);
			K4:=Factorial(R1[1])*Factorial(S1[1]-1)*(1-q^(N-1))^(S1[1]);
			//C_l-1^N-1
			K5:=(N-1)^(R2[1])*q^(N-1)*Euler(S2[1]-1,N-1);
			K6:=Factorial(R2[1])*Factorial(S2[1]-1)*(1-q^(N-1))^(S2[1]);
			//C_l^N-2
			K7:=(N-2)^(R1[1])*q^(N-2)*Euler(S1[1]-1,N-2);
			K8:=Factorial(R1[1])*Factorial(S1[1]-1)*(1-q^(N-2))^(S1[1]);
			//C_l-1^N-2
			K9:=(N-2)^(R2[1])*q^(N-2)*Euler(S2[1]-1,N-2);
			K10:=Factorial(R2[1])*Factorial(S2[1]-1)*(1-q^(N-2))^(S2[1]);
			//C_l-2^N-2
			K11:=(N-2)^(R3[1])*q^(N-2)*Euler(S3[1]-1,N-2);
			K12:=Factorial(R3[1])*Factorial(S3[1]-1)*(1-q^(N-2))^(S3[1]);
			
			
			BB:=$$(BB,S1,R1,N-3,Precision)+(K1/K2+K3/K4+K7/K8)*$$(BB,S2,R2,N-3,Precision)+((K9/K10)*((K1/K2)+(K3/K4))+(K1/K2)*(K5/K6))*$$(BB,S3,R3,N-3,Precision)+(K1/K2)*(K5/K6)*(K11/K12)*$$(BB,S4,R4,N-3,Precision);
		end if;
	elif l eq 3 then
		S3:=Remove(S2,1);
		R3:=Remove(R2,1);
		
		K1:=N^(R1[1])*q^N*Euler(S1[1]-1,N);
		K2:=Factorial(R1[1])*Factorial(S1[1]-1)*(1-q^N)^(S1[1]);
		
		K3:=(N-1)^(R1[1])*q^(N-1)*Euler(S1[1]-1,N-1);
		K4:=Factorial(R1[1])*Factorial(S1[1]-1)*(1-q^(N-1))^(S1[1]);
		
		K5:=(N-1)^(R2[1])*q^(N-1)*Euler(S2[1]-1,N-1);
		K6:=Factorial(R2[1])*Factorial(S2[1]-1)*(1-q^(N-1))^(S2[1]);
		
		BB:=$$(BB,S1,R1,N-2,Precision)+(K1/K2+K3/K4)*$$(BB,S2,R2,N-2,Precision)+(K1/K2)*(K5/K6)*$$(BB,S3,R3,N-2,Precision);
	elif l eq 2 then
		K1:=N^(R1[1])*q^N*Euler(S1[1]-1,N);
		K2:=Factorial(R1[1])*Factorial(S1[1]-1)*(1-q^N)^(S1[1]);
		BB:=$$(BB,S1,R1,N-1,Precision)+(K1)/(K2)*$$(BB,S2,R2,N-1,Precision);
	else
		K1:=N^(R1[1])*q^N*Euler(S1[1]-1,N);
		K2:=Factorial(R1[1])*Factorial(S1[1]-1)*(1-q^N)^(S1[1]);
		BB:=$$(BB,S1,R1,N-1,Precision)+(K1)/(K2);
	end if;
	return BB;
end function;

BiBracketspp := function(S1,R1,N)
	Precision:=N+1;
	K<q>:=PowerSeriesRing(R,Precision);
	BB:=0;
	//t:=Cputime();
	B:=BiBpp(BB,S1,R1,N,Precision);
	//Cputime(t);
	return B;
end function;

BIBpp:=function(S1,R1)
	return BiBracketspp(S1,R1,DECIMALEN);
end function;

MOBpp:=function(S1)
	R1:=[];
	for i:=1 to #S1 do
		Append(~R1,0);
	end for;
	return BIBpp(S1,R1);
end function;



//S1, R1 sequences. N precision.
BiBrackets := function(S1,R1,N)
	Precision:=N+1;
	K<q>:=PowerSeriesRing(R,Precision);
	BB:=0;
	//t:=Cputime();
	B:=BiB(BB,S1,R1,N,Precision);
	//Cputime(t);
	return B;
end function;
	
DER:=function(f)
	return q*Derivative(f);
end function; 
	
	
BIB:=function(S1,R1)
	return BiBrackets(S1,R1,DECIMALEN);
end function;

MOB:=function(S1)
	R1:=[];
	for i:=1 to #S1 do
		Append(~R1,0);
	end for;
	return BIB(S1,R1);
end function;
	
	
	
Wn := function(n)
	W:=[];
	for i:=1 to n do
		for w in Partitions(i) do
			Temp:=MOBpp(w);
			Append(~W,Temp);
			//Append(~W,DER(Temp));
		end for;
	end for;
	return W;
end function;

Matrn := function(n)
	u:=[];
	WN:=Wn(n);
	for w in WN do
		v:=[];
		for i:=0 to DECIMALEN do
			Append(~v,Coefficient(w,i));
		end for;
		u:=u cat v;
	end for;
	M:=Matrix(RationalField(),#WN,DECIMALEN+1,u);
	return M;
end function;

Wnnn := function(n,S,R)
	W:=[];
	for i:=1 to n do
		for w in Partitions(i) do
			Temp:=MOBpp(w);
			Append(~W,Temp);
			//Append(~W,DER(Temp));
		end for;
	end for;
	Append(~W,BIB(S,R));
	return W;
end function;


MATRN := function(n,S,R)
	u:=[];
	WN:=Wnnn(n,S,R);
	for w in WN do
		v:=[];
		for i:=0 to DECIMALEN do
			Append(~v,Coefficient(w,i));
		end for;
		u:=u cat v;
	end for;
	M:=Matrix(RationalField(),#WN,DECIMALEN+1,u);
	return M;
end function;

Geom := function(a,b,c,N)
	K<q>:=PowerSeriesRing(R,N+1);
	A:=1;
	Sum:=1;
	for i:=1 to N+1 do
		Sum:=Sum+A*((a+i-1)*(b+i-1))/(i*(c+i-1))*q^i;
	end for;
	x:=[RationalField()!0];
	for i:=1 to N do
		Append(~x,Coefficient(Sum,i));
	end for;
	return x;
end function;


/*	
for i:=1 to 100 do
for j:=1 to 100 do
for k:=1 to 100 do
p:=Geom(i,j,k,100);
P:=Matrix(RationalField(),1,101,p);
//N:=Matrn(6);
M:=VerticalJoin(N,P);
Rank(M)-Rank(N);
end for;
end for;
end for;






X:=[];

for i:=1 to 51 do
	Append(~X,Coefficient(p,i-1));
end for;
N:=VerticalJoin(M,Matrix(RationalField(),1,51,X));


p:=p+i*q^i/(1-q^i)+q^i/((1-q^i)^2);
p:=p+i*q^i/(1-q^i)+q^i/((1-q^i)^2);

BIB([2,1],[2,0]),BIB([1,2],[1,1]),BIB([1,1,1],[1,0,0]),BIB([1,1,1],[0,1,0]),BIB([1,1,1],[0,0,1]),BIB([2,1],[1,0]),BIB([1,2],[1,0]),BIB([2,1],[0,1]),BIB([1,2],[0,1]),BIB([1,1],[1,0]),BIB([1,1],[0,1])


X:=[MOB([1]),MOB([1,1]),MOB([2]),MOB([2,1]),MOB([1,2]),MOB([3]),MOB([1,1,1]),MOB([2,1,1]),MOB([1,2,1]),MOB([1,1,2]),MOB([3,1]),MOB([2,2]),MOB([1,3]),MOB([4]),MOB([1,4]),MOB([2,3]),MOB([4,1]),MOB([5]),MOB([3,2]),MOB([1,3,1]),MOB([1,1,3]),MOB([2,2,1]),MOB([1,2,2]),MOB([2,1,2])];


u:=[];
for w in X do
	v:=[];
	for i:=0 to 50 do
		Append(~v,Coefficient(w,i));
	end for;
	u:=u cat v;
end for;

v:=[];
k:=DER(MOB([1,1]));
for i:=0 to 50 do
	Append(~v,Coefficient(k,i));
end for;
u:=v cat u;
M:=Matrix(RationalField(),#X+1,51,u);
Kernel(M);






i2:=[0, 0, 0, 1, 0, 0, 0, -8/5, -4/5, 0, 1/5, -3/5, 2, 0, -6/5, -3/5, -3/5, 0, 3, -12/5, 0, 0, 12/5, 12/5, -4/5];
i1:=[0, 0, 0, 0, 1, 0, 0, 4/5, 2/5, 0, 7/5, 9/5, -4, 0, 18/5, 9/5, 9/5, 0, -9, 36/5, 0, 0, -36/5, -36/5, 2/5];

DECIMALEN:=1000;

Y:=[];
for j:=1 to 35 do
for i:=1 to j do
Append(~Y,BIB([i],[j-i]));
end for;
end for;


Y2:=Y;
Append(~Y2,BIB([1,1],[0,3]));

u:=[];
for w in Y2 do
	v:=[];
	for i:=0 to DECIMALEN do
		Append(~v,Coefficient(w,i));
	end for;
	u:=u cat v;
end for;

M:=Matrix(RationalField(),#Y2,DECIMALEN+1,u);
Kernel(M);



*/





% RELATIONS

Shufflep := function(S,R)
	s1:=S[1];
	s2:=R[1];
	r1:=S[2];
	r2:=R[2];
	
	Sum:=[];
	for j:=1 to s1 do
		for k:=0 to r2 do
			Append(~Sum,<Binomial(s1+s2-j-1,s1-j)*Binomial(r1+r2-k,r1)*(-1)^(r2-k),[s1+s2-j,j],[k,r1+r2-k]>);
		end for;
	end for;
	for j:=1 to s2 do
		for k:=0 to r1 do
			Append(~Sum,<Binomial(s1+s2-j-1,s2-j)*Binomial(r1+r2-k,r2)*(-1)^(r1-k),[s1+s2-j,j],[k,r1+r2-k]>);
		end for;
	end for;
	return Sum;
end function;

Cleanup:= function(Sum)
	T:=Sum;
	sum:=[];
	for w in Sum do
		e:=0;
		for v in T do
			if v[2] eq w[2] and v[3] eq w[3] then
				e:=e+v[1];
				Exclude(~T,v);
			end if;
		end for;
		if e ne 0 then
			Append(~sum,<e,w[2],w[3]>);
		end if;
	end for;
	return sum;
end function;

Shuffle := function(S,R)
	return Cleanup(Shufflep(S,R));
end function;


AddSums := function(T)
	V:=[];
	for v in T do
		V:=V cat v;
	end for;
	return Cleanup(V);
end function;


Partition := function(S,R)
	Part:=[];
	//Append(~Part,<-1,[S[1],S[2]],[R[1],R[2]]>);
	for j:=0 to R[1] do
		for k:=0 to S[2]-1 do
			Append(~Part,<(-1)^k*Binomial(S[1]-1+k,k)*Binomial(R[2]+j,j),[R[2]+j+1,R[1]-j+1],[S[2]-1-k,S[1]-1+k]>);
		end for;
	end for;
	return Part;
end function;


Test := function(n,m)
	list:=[];
	for j:=1 to n-1 do
		for k:=0 to m do
			Append(~list, <[n-j,j],[m-k,k]>);
		end for;
	end for;
	
	listp:=[];
	for j:=1 to Floor(n/2) do
		if n-j ne j then
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		else
			for k:=0 to Floor(m/2) do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		end if;
	end for;


	X:=[];
	for v in listp do
		Append(~X,Shuffle(v[1],v[2]));
	end for;
	T:=[];
	for j:=1 to #list*#X do
		Append(~T,0);
	end for;
	k:=0;
	for w in X do
		for v in w do
			t:=Index(list,<v[2],v[3]>)+(#list)*(k);
			T[t]:=v[1];
		end for;
		k:=k+1;
	end for;
	for j:=1 to #X do
		Y:=[1..#list];
		for i:=1 to Ceiling(#list/2) do
			if i eq j then
				Y[i]:=1;
				Y[#list-i+1]:=1;
			else
				Y[i]:=0;
				Y[#list-i+1]:=0;
			end if;
		end for;
		T:=T cat Y;
	end for;
	//T;
	//list;
	//listp;
	M:=Matrix(RationalField(),2*#listp,#list,T);
	return M;
end function;

Testp := function(n,m)
	list:=[];
	for j:=1 to n-1 do
		for k:=0 to m do
			Append(~list, <[n-j,j],[m-k,k]>);
		end for;
	end for;
	
	listp:=[];
	for j:=1 to Floor(n/2) do
		if n-j ne j then
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		else
			for k:=0 to Floor(m/2) do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		end if;
	end for;


	X:=[];
	for v in listp do
		Append(~X,Shuffle(v[1],v[2]));
	end for;
	T:=[];
	for j:=1 to #list*#X do
		Append(~T,0);
	end for;
	k:=0;
	for w in X do
		for v in w do
			t:=Index(list,<v[2],v[3]>)+(#list)*(k);
			T[t]:=v[1];
		end for;
		k:=k+1;
	end for;
	for j:=1 to #X do
		Y:=[1..#list];
		for i:=1 to Ceiling(#list/2) do
			if i eq j then
				Y[i]:=1;
				Y[#list-i+1]:=1;
			else
				Y[i]:=0;
				Y[#list-i+1]:=0;
			end if;
		end for;
		T:=T cat Y;
	end for;
	//T;
	//list;
	//listp;
	M:=Matrix(RationalField(),2*#listp,#list,T);
	return <M,list>;
end function;

JTest := function(n,m)
	N:=Testp(n,m)[1];
	M:=Testp(m+2,n-2)[1];
	B:=DiagonalJoin(N,M);
	
	list:=[];
	for j:=1 to m+1 do
		for k:=0 to n-2 do
			Append(~list, <[m+2-j,j],[n-2-k,k]>);
		end for;
	end for;
	
	listp:=[];
	for j:=1 to Floor(n/2) do
		if n-j ne j then
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		else
			for k:=0 to Floor(m/2) do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		end if;
	end for;
	
	X:=[];
	for v in listp do
		Append(~X,Partition(v[1],v[2]));
	end for;
	T:=[];
	for j:=1 to #list*#X do
		Append(~T,0);
	end for;
	k:=0;
	LIST:=Testp(n,m)[2] cat Testp(m+2,n-2)[2];
	//LIST;
	//T;
	for w in X do
		//w;
		for v in w do
			t:=Index(LIST,<v[2],v[3]>)+#LIST*k;
			//t;
			T[t]:=v[1];
		end for;
		k:=k+1;
	end for;
	lengte:=Integers()!(#T/Ncols(B));//HIER GAAT HET FOUT.
	//lengte;
	//T;
	//list;
	//listp;
	K:=Matrix(RationalField(),lengte,Ncols(B),T);
	//K;
	
	//B;
	return VerticalJoin(B,K);
end function;

RowElim := function(M)
	X:=M;
	n:=Floor(Nrows(M)/2);
	
	for i:=1 to n do
		for j:=1 to n do
			AddRow(~X,-M[i,j+n],2*n-j+1,i);
		end for;
	end for;
	return X;
end function;

LL:=function(n,m)
	M:=RowElim(Test(n,m));
	k:=Floor(Nrows(M)/2);
	N:=ExtractBlockRange(M,1,1,k,k);
	return N;
end function;

MOD := function(M,p)
	for i:=1 to Nrows(M) do
		for j:=1 to Ncols(M) do
			M[i,j]:=RationalField()!(Integers()!M[i,j] mod p);
		end for;
	end for;
	return M;
end function;






/*
AddSums([Shuffle([1,0],[2,2]),Shuffle([2,1],[1,1]),Shuffle([2,0],[1,2])]);
list1:=[<[ 2, 1 ], [ 0, 2 ]>,<[ 2, 1 ], [ 1, 1 ]>,<[ 2, 1 ], [ 2, 0 ]>,<[ 1, 2 ], [ 0, 2 ]>,< [ 1, 2 ], [ 1, 1 ]>,<[ 1, 2 ], [ 2, 0 ]>];
list2:=[<[ 3, 1 ], [ 1, 0 ]>, < [ 2, 2 ], [ 0, 1 ]>, <[ 2, 2 ], [ 1, 0 ]>, < [ 1, 3 ], [ 0, 1 ]>, <[ 1, 3 ], [ 1, 0 ]>];

T:=[];
for i:=1 to 18 do
	Append(~T,0);
end for;
X1:=[Shuffle([1,0],[2,2]),Shuffle([2,1],[1,1]),Shuffle([2,0],[1,2])];
X2:=[Shuffle([3,1],[1,0]),Shuffle([2,1],[2,0]),Shuffle([1,1],[3,0])];
T;
for w in X2 do
	for v in w do
		T[Index(list2,<v[2],v[3]>)+6*(Index(X2,w)-1)]:=v[1];
	end for;
end for;
T;
Y:=[[1,0,0,0,0,1],[0,1,0,0,1,0],[0,0,1,1,0,0]];
for i:=1 to 3 do
	T:=T cat Y[i];
end for;
T;
M:=Matrix(RationalField(),6,6,T);



for j:=1 to 20 do
for i:=2 to 20 do

x:=Testpp(i,j);
if not Rank(x) eq Ncols(x) then //and IsOdd(i+j)
<false,i,j>;
//Dimension(Kernel(x));
Ncols(x)-Rank(x);
end if;
end for;
end for;


*/



Testpp := function(n,m)
	list:=[];
	for j:=1 to n-1 do
		for k:=0 to m do
			Append(~list, <[n-j,j],[m-k,k]>);
		end for;
	end for;
	
	listp:=[];
	for j:=1 to n do
		if n-j ne j then
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		else
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		end if;
	end for;


	X:=[];
	for v in listp do
		Append(~X,Shuffle(v[1],v[2]));
	end for;
	T:=[];
	for j:=1 to #list*#X do
		Append(~T,0);
	end for;
	k:=0;
	for w in X do
		for v in w do
			t:=Index(list,<v[2],v[3]>)+(#list)*(k);
			T[t]:=v[1];
		end for;
		k:=k+1;
	end for;
	for j:=1 to #X do
		Y:=[1..#list];
		for i:=1 to Ceiling(#list/2) do
			if i eq j then
				Y[i]:=1;
				Y[#list-i+1]:=1;
			else
				Y[i]:=0;
				Y[#list-i+1]:=0;
			end if;
		end for;
		T:=T cat Y;
	end for;
	//T;
	//list;
	//listp;
	M:=Matrix(RationalField(),2*#listp,#list,T);
	/*
	for i:=1 to Nrows(M) do
		for j:=1 to Ncols(M) do
			if M[i,j] ne 0 then
				continue i;
			end if;
		end for;
		N:=ExtractBlock(M,1,1,i,Ncols(M));
		break;
	end for;
	return N;
	*/
	return M;
end function;

/*
Red :=function(n,m)
	M:=Testpp(n,m);
	M:=ExtractBlock(M,1,1,(n-1)*(m+1),(n-1)*(m+1));
	return M;
end function;

*/


RowElimm := function(M)
	for j:=1 to Nrows(M) do
		for i:=1 to Ceiling(Ncols(M)/2) do
			M[j,i]:=M[j,i]-M[j,Nrows(M)+1-i];
			M[j,Nrows(M)+1-i]:=0;
		end for;
	end for;
	return M;
end function;


Specs := procedure(M)
	"# columns: ",Ncols(M);
	"   # rows: ",Nrows(M);
	"     Rank: ",Rank(M);
end procedure;

Flip := function(M)
	N:=M;
	for i:=1 to Ncols(M) do
		for j:=1 to Nrows(M) do
			N[i,j]:=M[Nrows(M)+1-i,j];
		end for;
	end for;
	return N;
end function;


Oper := function(M)
	M:=M+Flip(M);
	M:=ExtractBlock(M,1,1,Ceiling(Nrows(M)/2),Ncols(M));
	T:=[];
	for j:=1 to Ncols(M)*Nrows(M) do
		Append(~T,0);
	end for;
	
	N:=Matrix(RationalField(),Nrows(M),Ncols(M),T);
	for i:=1 to Nrows(M) do
		for j:=1 to Ncols(M) do
			if i eq j then
				N[i,j]:=1;
				N[i,Ncols(M)+1-j]:=1;
			end if;
		end for;
	end for;
	return VerticalJoin(M,N);
end function;

//Flap := function(M)
	

RandM := function(n)
	
	stop:=true;
	N:=Matrix(RationalField(),1,1,[0]);
	while stop or Rank(N) eq n do
		T:=[];
		stop:=false; 
		for i:=1 to n^2 do
			x:=Random([-5..5]);
			Append(~T,x);
		end for;
		N:=Matrix(RationalField(),n,n,T);
	end while;
	return N;
end function;




Testd := function(n,m)
	list:=[];
for k:=0 to m do
	for j:=1 to n-1 do
		
			Append(~list, <[n-j,j],[m-k,k]>);
		end for;
	end for;
	
	listp:=[];
	for j:=1 to Floor(n/2) do
		if n-j ne j then
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		else
			for k:=0 to Floor(m/2) do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		end if;
	end for;


	X:=[];
	for v in listp do
		Append(~X,Shuffle(v[1],v[2]));
	end for;
	T:=[];
	for j:=1 to #list*#X do
		Append(~T,0);
	end for;
	k:=0;
	for w in X do
		for v in w do
			t:=Index(list,<v[2],v[3]>)+(#list)*(k);
			T[t]:=v[1];
		end for;
		k:=k+1;
	end for;
	for j:=1 to #X do
		Y:=[1..#list];
		for i:=1 to Ceiling(#list/2) do
			if i eq j then
				Y[i]:=1;
				Y[#list-i+1]:=1;
			else
				Y[i]:=0;
				Y[#list-i+1]:=0;
			end if;
		end for;
		T:=T cat Y;
	end for;
	//T;
	//list;
	//listp;
	M:=Matrix(RationalField(),2*#listp,#list,T);
	return M;
end function;


Red := function(n,m)
	list:=[];
	for j:=1 to n-1 do
		for k:=0 to m do
			Append(~list, <[n-j,j],[m-k,k]>);
		end for;
	end for;
	
	listp:=[];
	for j:=1 to n-1 do
		if n-j ne j then
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		else
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		end if;
	end for;

	//listp;
	X:=[];
	for v in listp do
		Append(~X,Shuffle(v[1],v[2]));
	end for;
	T:=[];
	for j:=1 to #list*#X do
		Append(~T,0);
	end for;
	k:=0;
	//X;
	for w in X do
		for v in w do
			t:=Index(list,<v[2],v[3]>)+(#list)*(k);
			T[t]:=v[1];
		end for;
		k:=k+1;
	end for;
	//T;
	for j:=1 to Ceiling(#X/2) do
		Y:=[1..#list];
		for i:=1 to Ceiling(#list/2) do
			if i eq j then
				Y[i]:=1;
				Y[#list-i+1]:=1;
			else
				Y[i]:=0;
				Y[#list-i+1]:=0;
			end if;
		end for;
		T:=T cat Y;
	end for;
	//T;
	//list;
	//listp;
	M:=Matrix(RationalField(),Ceiling(1.5*#listp),#list,T);
	return M;
end function;

Shu1 := function(S,R)
	s1:=S[1];
	s2:=R[1];
	r1:=S[2];
	r2:=R[2];
	
	Sum:=[];
	for j:=1 to s1 do
		for k:=0 to r2 do
			Append(~Sum,<Binomial(s1+s2-j-1,s1-j)*Binomial(r1+r2-k,r1)*(-1)^(r2-k),[s1+s2-j,j],[k,r1+r2-k]>);
		end for;
	end for;
	
	return Sum;
end function;

Shu2 := function(S,R)
	s1:=S[1];
	s2:=R[1];
	r1:=S[2];
	r2:=R[2];
	
	Sum:=[];
	for j:=1 to s2 do
		for k:=0 to r1 do
			Append(~Sum,<Binomial(s1+s2-j-1,s2-j)*Binomial(r1+r2-k,r2)*(-1)^(r1-k),[s1+s2-j,j],[k,r1+r2-k]>);
		end for;
	end for;
	return Sum;
end function;


Shu := function(S,R)
	T1:=Cleanup(Shu1(S,R));
	T2:=Cleanup(Shu2(S,R));
	return <T1,T2>;
end function;

Tes := function(n,m)
	list:=[];
	for j:=1 to n-1 do
		for k:=0 to m do
			Append(~list, <[n-j,j],[m-k,k]>);
		end for;
	end for;
	
	listp:=[];
	for j:=1 to n-1 do
		if n-j ne j then
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		else
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		end if;
	end for;

	//listp;
	X1:=[];
	X2:=[];
	for v in listp do
		Append(~X1,Shu(v[1],v[2])[1]);
		Append(~X2,Shu(v[1],v[2])[2]);
	end for;
	T1:=[];
	T2:=[];
	for j:=1 to #list*#X1 do
		Append(~T1,0);
	end for;
	k:=0;
	for j:=1 to #list*#X2 do
		Append(~T2,0);
	end for;
	//X;
	for w in X1 do
		for v in w do
			t:=Index(list,<v[2],v[3]>)+(#list)*(k);
			T1[t]:=v[1];
		end for;
		k:=k+1;
	end for;
	//T;
	for j:=1 to Ceiling(#X1/2) do
		Y:=[1..#list];
		for i:=1 to Ceiling(#list/2) do
			if i eq j then
				Y[i]:=1;
				Y[#list-i+1]:=1;
			else
				Y[i]:=0;
				Y[#list-i+1]:=0;
			end if;
		end for;
		T1:=T1 cat Y;
	end for;
	k:=0;
	for w in X2 do
		for v in w do
			t:=Index(list,<v[2],v[3]>)+(#list)*(k);
			T2[t]:=v[1];
		end for;
		k:=k+1;
	end for;
	//T;
	for j:=1 to Ceiling(#X2/2) do
		Y:=[1..#list];
		for i:=1 to Ceiling(#list/2) do
			if i eq j then
				Y[i]:=0;
				Y[#list-i+1]:=0;
			else
				Y[i]:=0;
				Y[#list-i+1]:=0;
			end if;
		end for;
		T2:=T2 cat Y;
	end for;
	//T;
	//list;
	//listp;
	M1:=Matrix(RationalField(),Ceiling(1.5*#listp),#list,T1);
	M2:=Matrix(RationalField(),Ceiling(1.5*#listp),#list,T2);
	N:=M2;
	for i:=1 to Ncols(M2) do
		for j:=1 to Nrows(M2) do
			N[j,i]:=-M2[j,Ncols(M2)+1-i];
		end for;
	end for;
	return M1+N;
end function;

Tess:= function(n,m)
	M:=Tes(n,m);
	return ExtractBlock(M,1,1,(n-1)*(m+1),(n-1)*(m+1));
end function;

Toets := function(M)
if Ncols(M) eq Rank(M) then
	return true;
else
	return false;
end if;
end function;

/*
for i:=2 to 15 do
	for j:=0 to 15 do
		if not Toets(ExtractBlock(Tes(i,j),1,1,(i-1)*(j+1),(i-1)*(j+1))) then
			<i,j>;
		end if;
	end for;
end for;
for i:=2 to 15 do
	for j:=0 to 15 do
		if not Toets(Nieuw(i,j)) then
			<i,j>;
		end if;
	end for;
end for;
*/

Shuffleps := function(S,R,x)
	s1:=S[1];
	s2:=R[1];
	r1:=S[2];
	r2:=R[2];
	
	Sum:=[];
	if x eq "+" then
	for j:=1 to s1 do
		for k:=0 to r2 do
			Append(~Sum,<Binomial(s1+s2-j-1,s1-j)*Binomial(r1+r2-k,r1)*(-1)^(r2-k),[s1+s2-j,j],[k,r1+r2-k]>);
		end for;
	end for;
	else
	for j:=1 to s1 do
		for k:=0 to r2 do
			Append(~Sum,<Binomial(s1+s2-j-1,s1-j)*Binomial(r1+r2-k,r1)*(-1)^(s1-j),[s1+s2-j,j],[k,r1+r2-k]>);
		end for;
	end for;
	end if;


	return Sum;
end function;



Shufflee := function(S,R,x)
	return Cleanup(Shuffleps(S,R,x));
end function;

Redkk := function(n,m,x)
	list:=[];
	for j:=1 to n-1 do
		for k:=0 to m do
			Append(~list, <[n-j,j],[m-k,k]>);
		end for;
	end for;
	
	listp:=[];
	for j:=1 to n-1 do
		if n-j ne j then
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		else
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		end if;
	end for;

	//listp;
	X:=[];
	for v in listp do
		Append(~X,Shufflee(v[1],v[2],x));
	end for;
	T:=[];
	for j:=1 to #list*#X do
		Append(~T,0);
	end for;
	k:=0;
	//X;
	for w in X do
		for v in w do
			t:=Index(list,<v[2],v[3]>)+(#list)*(k);
			T[t]:=v[1];
		end for;
		k:=k+1;
	end for;

	//T;
	//list;
	//listp;
	M:=Matrix(RationalField(),#listp,#list,T);
	return M;
end function;



Rho:= function(M)
	L:=M;
	for j:=1 to Ncols(M) do
		for i:=1 to Ncols(M) do
			L[i,j]:=M[Ncols(M)+1-i,j];
		end for;
	end for;
	return L;
end function;

Sigma:= function(M)
	L:=M;
	for j:=1 to Ncols(M) do
		for i:=1 to Ncols(M) do
			L[i,j]:=M[i,Ncols(M)+1-j];
		end for;
	end for;
	return L;
end function;

SR := function(M)
	return Rho(Sigma(M));
end function;

Klopt:=function(S,R)
	P:=Partition(S,R);
	X:=[];
	for p in P do
		Q:=Partition(p[2],p[3]);
		for q in Q do
			Append(~X,<q[1]*p[1],q[2],q[3]>);
		end for;
	end for;
	return Cleanup(X);
end function;

{{ 2,  1,  1,  1,  0,  1,  2,  1,  1,  2},
{ 6,  2,  2,  1,  0,  1,  3,  2,  1,  0},
{ 0,  1,  1,  1,  3,  1,  0,  1,  1,  0},
{ 6,  1,  1,  0,  0,  0,  3,  1,  0,  0},
{ 0,  2,  2,  2,  3,  0,  0,  0,  0,  0},
{ 0,  1,  1,  1,  0,  1,  0,  1,  1,  0},
{ 2,  0,  0,  0,  0,  0,  1,  0,  0,  0},
{ 0,  1,  1,  1,  0,  0,  0,  0,  0,  0},
{ 0,  1,  0,  1,  0,  1,  0,  0,  0,  0},
{ 1,  0,  0,  0,  0,  0,  1,  0,  0,  1},
{ 3,  3,  2,  3,  2,  2,  3,  2,  2,  2},
{ 9,  7,  4,  5,  3,  2,  3,  2,  1,  0},
{ 9,  8,  5,  7,  4,  2,  6,  3,  1,  0},
{ 9,  5,  2,  3,  1,  0,  3,  1,  0,  0},
{18, 12,  6,  6,  3,  0,  0,  0,  0,  0},
{ 9,  7,  4,  6,  3,  1,  6,  3,  1,  0},
{ 3,  1,  0,  1,  0,  0,  1,  0,  0,  0},
{ 9,  4,  1,  1,  0,  0,  0,  0,  0,  0},
{ 9,  5,  2,  2,  1,  1,  0,  0,  0,  0},
{ 3,  2,  1,  2,  1,  1,  2,  1,  1,  1}}

% Relations
Shufflep := function(S,R)
	s1:=S[1];
	s2:=R[1];
	r1:=S[2];
	r2:=R[2];
	
	Sum:=[];
	for j:=1 to s1 do
		for k:=0 to r2 do
			Append(~Sum,<Binomial(s1+s2-j-1,s1-j)*Binomial(r1+r2-k,r1)*(-1)^(r2-k),[s1+s2-j,j],[k,r1+r2-k]>);
		end for;
	end for;
	for j:=1 to s2 do
		for k:=0 to r1 do
			Append(~Sum,<Binomial(s1+s2-j-1,s2-j)*Binomial(r1+r2-k,r2)*(-1)^(r1-k),[s1+s2-j,j],[k,r1+r2-k]>);
		end for;
	end for;
	return Sum;
end function;

Cleanup:= function(Sum)
	T:=Sum;
	sum:=[];
	for w in Sum do
		e:=0;
		for v in T do
			if v[2] eq w[2] and v[3] eq w[3] then
				e:=e+v[1];
				Exclude(~T,v);
			end if;
		end for;
		if e ne 0 then
			Append(~sum,<e,w[2],w[3]>);
		end if;
	end for;
	return sum;
end function;

Shuffle := function(S,R)
	return Cleanup(Shufflep(S,R));
end function;


AddSums := function(T)
	V:=[];
	for v in T do
		V:=V cat v;
	end for;
	return Cleanup(V);
end function;


Partition := function(S,R)
	Part:=[];
	//Append(~Part,<-1,[S[1],S[2]],[R[1],R[2]]>);
	for j:=0 to R[1] do
		for k:=0 to S[2]-1 do
			Append(~Part,<(-1)^k*Binomial(S[1]-1+k,k)*Binomial(R[2]+j,j),[R[2]+j+1,R[1]-j+1],[S[2]-1-k,S[1]-1+k]>);
		end for;
	end for;
	return Part;
end function;

Partit1 := function(T)

	X:=[];
	for p in T do
		k:=Partition(p[2],p[3]);
		for i:=1 to #k do
			k[i][1]:=k[i][1]*p[1];
		end for;
		X:=X cat k;
	end for;
	
	return Cleanup(X);
end function;

Partit2 := function(T)

	X:=[];
	for p in T do
		k:=Partition(p[3],p[2]);
		for i:=1 to #k do
			k[i][1]:=k[i][1]*p[1];
		end for;
		X:=X cat k;
	end for;
	
	return Cleanup(X);
end function;


Test := function(n,m)
	list:=[];
	for j:=1 to n-1 do
		for k:=0 to m do
			Append(~list, <[n-j,j],[m-k,k]>);
		end for;
	end for;
	
	listp:=[];
	for j:=1 to Floor(n/2) do
		if n-j ne j then
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		else
			for k:=0 to Floor(m/2) do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		end if;
	end for;


	X:=[];
	for v in listp do
		Append(~X,Shuffle(v[1],v[2]));
	end for;
	T:=[];
	for j:=1 to #list*#X do
		Append(~T,0);
	end for;
	k:=0;
	for w in X do
		for v in w do
			t:=Index(list,<v[2],v[3]>)+(#list)*(k);
			T[t]:=v[1];
		end for;
		k:=k+1;
	end for;
	for j:=1 to #X do
		Y:=[1..#list];
		for i:=1 to Ceiling(#list/2) do
			if i eq j then
				Y[i]:=1;
				Y[#list-i+1]:=1;
			else
				Y[i]:=0;
				Y[#list-i+1]:=0;
			end if;
		end for;
		T:=T cat Y;
	end for;
	//T;
	//list;
	//listp;
	M:=Matrix(RationalField(),2*#listp,#list,T);
	return M;
end function;

Testp := function(n,m)
	list:=[];
	for j:=1 to n-1 do
		for k:=0 to m do
			Append(~list, <[n-j,j],[m-k,k]>);
		end for;
	end for;
	
	listp:=[];
	for j:=1 to Floor(n/2) do
		if n-j ne j then
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		else
			for k:=0 to Floor(m/2) do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		end if;
	end for;


	X:=[];
	for v in listp do
		Append(~X,Shuffle(v[1],v[2]));
	end for;
	T:=[];
	for j:=1 to #list*#X do
		Append(~T,0);
	end for;
	k:=0;
	for w in X do
		for v in w do
			t:=Index(list,<v[2],v[3]>)+(#list)*(k);
			T[t]:=v[1];
		end for;
		k:=k+1;
	end for;
	for j:=1 to #X do
		Y:=[1..#list];
		for i:=1 to Ceiling(#list/2) do
			if i eq j then
				Y[i]:=1;
				Y[#list-i+1]:=1;
			else
				Y[i]:=0;
				Y[#list-i+1]:=0;
			end if;
		end for;
		T:=T cat Y;
	end for;
	//T;
	//list;
	//listp;
	M:=Matrix(RationalField(),2*#listp,#list,T);
	return <M,list>;
end function;

JTest := function(n,m)
	N:=Testp(n,m)[1];
	M:=Testp(m+2,n-2)[1];
	B:=DiagonalJoin(N,M);
	
	list:=[];
	for j:=1 to m+1 do
		for k:=0 to n-2 do
			Append(~list, <[m+2-j,j],[n-2-k,k]>);
		end for;
	end for;
	
	listp:=[];
	for j:=1 to Floor(n/2) do
		if n-j ne j then
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		else
			for k:=0 to Floor(m/2) do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		end if;
	end for;
	
	X:=[];
	for v in listp do
		Append(~X,Partition(v[1],v[2]));
	end for;
	T:=[];
	for j:=1 to #list*#X do
		Append(~T,0);
	end for;
	k:=0;
	LIST:=Testp(n,m)[2] cat Testp(m+2,n-2)[2];
	//LIST;
	//T;
	for w in X do
		//w;
		for v in w do
			t:=Index(LIST,<v[2],v[3]>)+#LIST*k;
			//t;
			T[t]:=v[1];
		end for;
		k:=k+1;
	end for;
	lengte:=Integers()!(#T/Ncols(B));//HIER GAAT HET FOUT.
	//lengte;
	//T;
	//list;
	//listp;
	K:=Matrix(RationalField(),lengte,Ncols(B),T);
	//K;
	
	//B;
	return VerticalJoin(B,K);
end function;

RowElim := function(M)
	X:=M;
	n:=Floor(Nrows(M)/2);
	
	for i:=1 to n do
		for j:=1 to n do
			AddRow(~X,-M[i,j+n],2*n-j+1,i);
		end for;
	end for;
	return X;
end function;

LL:=function(n,m)
	M:=RowElim(Test(n,m));
	k:=Floor(Nrows(M)/2);
	N:=ExtractBlockRange(M,1,1,k,k);
	return N;
end function;

MOD := function(M,p)
	for i:=1 to Nrows(M) do
		for j:=1 to Ncols(M) do
			M[i,j]:=RationalField()!(Integers()!M[i,j] mod p);
		end for;
	end for;
	return M;
end function;






/*
AddSums([Shuffle([1,0],[2,2]),Shuffle([2,1],[1,1]),Shuffle([2,0],[1,2])]);
list1:=[<[ 2, 1 ], [ 0, 2 ]>,<[ 2, 1 ], [ 1, 1 ]>,<[ 2, 1 ], [ 2, 0 ]>,<[ 1, 2 ], [ 0, 2 ]>,< [ 1, 2 ], [ 1, 1 ]>,<[ 1, 2 ], [ 2, 0 ]>];
list2:=[<[ 3, 1 ], [ 1, 0 ]>, < [ 2, 2 ], [ 0, 1 ]>, <[ 2, 2 ], [ 1, 0 ]>, < [ 1, 3 ], [ 0, 1 ]>, <[ 1, 3 ], [ 1, 0 ]>];

T:=[];
for i:=1 to 18 do
	Append(~T,0);
end for;
X1:=[Shuffle([1,0],[2,2]),Shuffle([2,1],[1,1]),Shuffle([2,0],[1,2])];
X2:=[Shuffle([3,1],[1,0]),Shuffle([2,1],[2,0]),Shuffle([1,1],[3,0])];
T;
for w in X2 do
	for v in w do
		T[Index(list2,<v[2],v[3]>)+6*(Index(X2,w)-1)]:=v[1];
	end for;
end for;
T;
Y:=[[1,0,0,0,0,1],[0,1,0,0,1,0],[0,0,1,1,0,0]];
for i:=1 to 3 do
	T:=T cat Y[i];
end for;
T;
M:=Matrix(RationalField(),6,6,T);



for j:=1 to 20 do
for i:=2 to 20 do

x:=Testpp(i,j);
if not Rank(x) eq Ncols(x) then //and IsOdd(i+j)
<false,i,j>;
//Dimension(Kernel(x));
Ncols(x)-Rank(x);
end if;
end for;
end for;


*/



Testpp := function(n,m)
	list:=[];
	for j:=1 to n-1 do
		for k:=0 to m do
			Append(~list, <[n-j,j],[m-k,k]>);
		end for;
	end for;
	
	listp:=[];
	for j:=1 to n do
		if n-j ne j then
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		else
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		end if;
	end for;


	X:=[];
	for v in listp do
		Append(~X,Shuffle(v[1],v[2]));
	end for;
	T:=[];
	for j:=1 to #list*#X do
		Append(~T,0);
	end for;
	k:=0;
	for w in X do
		for v in w do
			t:=Index(list,<v[2],v[3]>)+(#list)*(k);
			T[t]:=v[1];
		end for;
		k:=k+1;
	end for;
	for j:=1 to #X do
		Y:=[1..#list];
		for i:=1 to Ceiling(#list/2) do
			if i eq j then
				Y[i]:=1;
				Y[#list-i+1]:=1;
			else
				Y[i]:=0;
				Y[#list-i+1]:=0;
			end if;
		end for;
		T:=T cat Y;
	end for;
	//T;
	//list;
	//listp;
	M:=Matrix(RationalField(),2*#listp,#list,T);
	/*
	for i:=1 to Nrows(M) do
		for j:=1 to Ncols(M) do
			if M[i,j] ne 0 then
				continue i;
			end if;
		end for;
		N:=ExtractBlock(M,1,1,i,Ncols(M));
		break;
	end for;
	return N;
	*/
	return M;
end function;

/*
Red :=function(n,m)
	M:=Testpp(n,m);
	M:=ExtractBlock(M,1,1,(n-1)*(m+1),(n-1)*(m+1));
	return M;
end function;

*/


RowElimm := function(M)
	for j:=1 to Nrows(M) do
		for i:=1 to Ceiling(Ncols(M)/2) do
			M[j,i]:=M[j,i]-M[j,Nrows(M)+1-i];
			M[j,Nrows(M)+1-i]:=0;
		end for;
	end for;
	return M;
end function;


Specs := procedure(M)
	"# columns: ",Ncols(M);
	"   # rows: ",Nrows(M);
	"     Rank: ",Rank(M);
end procedure;

Flip := function(M)
	N:=M;
	for i:=1 to Ncols(M) do
		for j:=1 to Nrows(M) do
			N[i,j]:=M[Nrows(M)+1-i,j];
		end for;
	end for;
	return N;
end function;


Oper := function(M)
	M:=M+Flip(M);
	M:=ExtractBlock(M,1,1,Ceiling(Nrows(M)/2),Ncols(M));
	T:=[];
	for j:=1 to Ncols(M)*Nrows(M) do
		Append(~T,0);
	end for;
	
	N:=Matrix(RationalField(),Nrows(M),Ncols(M),T);
	for i:=1 to Nrows(M) do
		for j:=1 to Ncols(M) do
			if i eq j then
				N[i,j]:=1;
				N[i,Ncols(M)+1-j]:=1;
			end if;
		end for;
	end for;
	return VerticalJoin(M,N);
end function;

//Flap := function(M)
	

RandM := function(n)
	
	stop:=true;
	N:=Matrix(RationalField(),1,1,[0]);
	while stop or Rank(N) eq n do
		T:=[];
		stop:=false; 
		for i:=1 to n^2 do
			x:=Random([-5..5]);
			Append(~T,x);
		end for;
		N:=Matrix(RationalField(),n,n,T);
	end while;
	return N;
end function;




Testd := function(n,m)
	list:=[];
for k:=0 to m do
	for j:=1 to n-1 do
		
			Append(~list, <[n-j,j],[m-k,k]>);
		end for;
	end for;
	
	listp:=[];
	for j:=1 to Floor(n/2) do
		if n-j ne j then
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		else
			for k:=0 to Floor(m/2) do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		end if;
	end for;


	X:=[];
	for v in listp do
		Append(~X,Shuffle(v[1],v[2]));
	end for;
	T:=[];
	for j:=1 to #list*#X do
		Append(~T,0);
	end for;
	k:=0;
	for w in X do
		for v in w do
			t:=Index(list,<v[2],v[3]>)+(#list)*(k);
			T[t]:=v[1];
		end for;
		k:=k+1;
	end for;
	for j:=1 to #X do
		Y:=[1..#list];
		for i:=1 to Ceiling(#list/2) do
			if i eq j then
				Y[i]:=1;
				Y[#list-i+1]:=1;
			else
				Y[i]:=0;
				Y[#list-i+1]:=0;
			end if;
		end for;
		T:=T cat Y;
	end for;
	//T;
	//list;
	//listp;
	M:=Matrix(RationalField(),2*#listp,#list,T);
	return M;
end function;


Red := function(n,m)
	list:=[];
	for j:=1 to n-1 do
		for k:=0 to m do
			Append(~list, <[n-j,j],[m-k,k]>);
		end for;
	end for;
	list;
	listp:=[];
	for j:=1 to n-1 do
		if n-j ne j then
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		else
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		end if;
	end for;

	listp;
	X:=[];
	for v in listp do
		Append(~X,Shuffle(v[1],v[2]));
	end for;
	T:=[];
	for j:=1 to #list*#X do
		Append(~T,0);
	end for;
	k:=0;
	//X;
	for w in X do
		for v in w do
			t:=Index(list,<v[2],v[3]>)+(#list)*(k);
			T[t]:=v[1];
		end for;
		k:=k+1;
	end for;
	//T;
	for j:=1 to Ceiling(#X/2) do
		Y:=[1..#list];
		for i:=1 to Ceiling(#list/2) do
			if i eq j then
				Y[i]:=1;
				Y[#list-i+1]:=1;
			else
				Y[i]:=0;
				Y[#list-i+1]:=0;
			end if;
		end for;
		T:=T cat Y;
	end for;
	//T;
	//list;
	//listp;
	M:=Matrix(RationalField(),Ceiling(1.5*#listp),#list,T);
	return M;
end function;

Shu1 := function(S,R)
	s1:=S[1];
	s2:=R[1];
	r1:=S[2];
	r2:=R[2];
	
	Sum:=[];
	for j:=1 to s1 do
		for k:=0 to r2 do
			Append(~Sum,<Binomial(s1+s2-j-1,s1-j)*Binomial(r1+r2-k,r1)*(-1)^(r2-k),[s1+s2-j,j],[k,r1+r2-k]>);
		end for;
	end for;
	
	return Sum;
end function;

Shu2 := function(S,R)
	s1:=S[1];
	s2:=R[1];
	r1:=S[2];
	r2:=R[2];
	
	Sum:=[];
	for j:=1 to s2 do
		for k:=0 to r1 do
			Append(~Sum,<Binomial(s1+s2-j-1,s2-j)*Binomial(r1+r2-k,r2)*(-1)^(r1-k),[s1+s2-j,j],[k,r1+r2-k]>);
		end for;
	end for;
	return Sum;
end function;


Shu := function(S,R)
	T1:=Cleanup(Shu1(S,R));
	T2:=Cleanup(Shu2(S,R));
	return <T1,T2>;
end function;

Tes := function(n,m)
	list:=[];
	for j:=1 to n-1 do
		for k:=0 to m do
			Append(~list, <[n-j,j],[m-k,k]>);
		end for;
	end for;
	
	listp:=[];
	for j:=1 to n-1 do
		if n-j ne j then
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		else
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		end if;
	end for;

	//listp;
	X1:=[];
	X2:=[];
	for v in listp do
		Append(~X1,Shu(v[1],v[2])[1]);
		Append(~X2,Shu(v[1],v[2])[2]);
	end for;
	T1:=[];
	T2:=[];
	for j:=1 to #list*#X1 do
		Append(~T1,0);
	end for;
	k:=0;
	for j:=1 to #list*#X2 do
		Append(~T2,0);
	end for;
	//X;
	for w in X1 do
		for v in w do
			t:=Index(list,<v[2],v[3]>)+(#list)*(k);
			T1[t]:=v[1];
		end for;
		k:=k+1;
	end for;
	//T;
	for j:=1 to Ceiling(#X1/2) do
		Y:=[1..#list];
		for i:=1 to Ceiling(#list/2) do
			if i eq j then
				Y[i]:=1;
				Y[#list-i+1]:=1;
			else
				Y[i]:=0;
				Y[#list-i+1]:=0;
			end if;
		end for;
		T1:=T1 cat Y;
	end for;
	k:=0;
	for w in X2 do
		for v in w do
			t:=Index(list,<v[2],v[3]>)+(#list)*(k);
			T2[t]:=v[1];
		end for;
		k:=k+1;
	end for;
	//T;
	for j:=1 to Ceiling(#X2/2) do
		Y:=[1..#list];
		for i:=1 to Ceiling(#list/2) do
			if i eq j then
				Y[i]:=0;
				Y[#list-i+1]:=0;
			else
				Y[i]:=0;
				Y[#list-i+1]:=0;
			end if;
		end for;
		T2:=T2 cat Y;
	end for;
	//T;
	//list;
	//listp;
	M1:=Matrix(RationalField(),Ceiling(1.5*#listp),#list,T1);
	M2:=Matrix(RationalField(),Ceiling(1.5*#listp),#list,T2);
	N:=M2;
	for i:=1 to Ncols(M2) do
		for j:=1 to Nrows(M2) do
			N[j,i]:=-M2[j,Ncols(M2)+1-i];
		end for;
	end for;
	return M1+N;
end function;

Tess:= function(n,m)
	M:=Tes(n,m);
	return ExtractBlock(M,1,1,(n-1)*(m+1),(n-1)*(m+1));
end function;

Toets := function(M)
if Ncols(M) eq Rank(M) then
	return true;
else
	return false;
end if;
end function;

/*
for i:=2 to 15 do
	for j:=0 to 15 do
		if not Toets(ExtractBlock(Tes(i,j),1,1,(i-1)*(j+1),(i-1)*(j+1))) then
			<i,j>;
		end if;
	end for;
end for;
for i:=2 to 15 do
	for j:=0 to 15 do
		if not Toets(Nieuw(i,j)) then
			<i,j>;
		end if;
	end for;
end for;
*/

Shuffleps := function(S,R,x)
	s1:=S[1];
	s2:=R[1];
	r1:=S[2];
	r2:=R[2];
	
	Sum:=[];
	if x eq "+" then
	for j:=1 to s1 do
		for k:=0 to r2 do
			Append(~Sum,<Binomial(s1+s2-j-1,s1-j)*Binomial(r1+r2-k,r1)*(-1)^(r2-k),[s1+s2-j,j],[k,r1+r2-k]>);
		end for;
	end for;
	else
	for j:=1 to s1 do
		for k:=0 to r2 do
			Append(~Sum,<Binomial(s1+s2-j-1,s1-j)*Binomial(r1+r2-k,r1)*(-1)^(s1-j),[s1+s2-j,j],[k,r1+r2-k]>);
		end for;
	end for;
	end if;


	return Sum;
end function;



Shufflee := function(S,R,x)
	return Cleanup(Shuffleps(S,R,x));
end function;

Redkk := function(n,m,x)
	list:=[];
	for j:=1 to n-1 do
		for k:=0 to m do
			Append(~list, <[n-j,j],[m-k,k]>);
		end for;
	end for;
	
	listp:=[];
	for j:=1 to n-1 do
		if n-j ne j then
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		else
			for k:=0 to m do
				Append(~listp, <[n-j,m-k],[j,k]>);
			end for;
		end if;
	end for;

	//listp;
	X:=[];
	for v in listp do
		Append(~X,Shufflee(v[1],v[2],x));
	end for;
	T:=[];
	for j:=1 to #list*#X do
		Append(~T,0);
	end for;
	k:=0;
	//X;
	for w in X do
		for v in w do
			t:=Index(list,<v[2],v[3]>)+(#list)*(k);
			T[t]:=v[1];
		end for;
		k:=k+1;
	end for;

	//T;
	//list;
	//listp;
	M:=Matrix(RationalField(),#listp,#list,T);
	return M;
end function;



Rho:= function(M)
	L:=M;
	for j:=1 to Ncols(M) do
		for i:=1 to Ncols(M) do
			L[i,j]:=M[Ncols(M)+1-i,j];
		end for;
	end for;
	return L;
end function;

Sigma:= function(M)
	L:=M;
	for j:=1 to Ncols(M) do
		for i:=1 to Ncols(M) do
			L[i,j]:=M[i,Ncols(M)+1-j];
		end for;
	end for;
	return L;
end function;

SR := function(M)
	return Rho(Sigma(M));
end function;

Klopt:=function(S,R)
	P:=Partition(S,R);
	X:=[];
	for p in P do
		Q:=Partition(p[2],p[3]);
		for q in Q do
			Append(~X,<q[1]*p[1],q[2],q[3]>);
		end for;
	end for;
	return Cleanup(X);
end function;



Joe := function(n,m)
	list:=[];
	for j:=1 to n-1 do
		for k:=0 to m do
			Append(~list, <[n-j,j],[m-k,k]>);
		end for;
	end for;
	list2:=[];
	for j:=1 to m+1 do
		for k:=0 to n-2 do
			Append(~list2, <[m+2-j,j],[n-2-k,k]>);
		end for;
	end for;
	X:=[];
	for i:=1 to #list2 do
		Append(~X,0);
	end for;
	
	T:=[];
	for x in list do
		k:=Partition(x[1],x[2]);
		Y:=X;
		for u in k do
			Y[Index(list2,<u[2],u[3]>)]:=u[1];
		end for;
		T:=T cat Y;
	end for;
		
		
		
	return Matrix(RationalField(),#list,#list2,T);
end function;



Nor := function(S,R)
	P:=ZeroMatrix(RationalField(),S-1,S-1);
	Q:=ZeroMatrix(RationalField(),R+1,R+1);
	for i:=1 to S-1 do
		for j:=1 to S-1 do
			P[i,j]:=Binomial(S-1-j,i-1);
		end for;
	end for;
	for i:=1 to R+1 do
		for j:=1 to R+1 do
			Q[i,j]:=(-1)^(R+i+j)*Binomial(j-1,R+1-i);
		end for;
	end for;
	M:=KroneckerProduct(P,Q)-KroneckerProduct(SR(P),SR(Q));
	return M;
end function;

Pmatrix:=function(n)
	P:=ZeroMatrix(RationalField(),n,n);
	for i:=1 to n do
		for j:=1 to n do
			P[i,j]:=Binomial(n-j,i-1);
		end for;
	end for;
	return P;
end function;

Qmatrix:=function(n)
	Q:=ZeroMatrix(RationalField(),n,n);
	for i:=1 to n do
		for j:=1 to n do
			Q[i,j]:=(-1)^(n+i+j+1)*Binomial(j-1,n-i);
		end for;
	end for;
	return Q;
end function;


Inv:=function(S,R)
	
	J1:=ZeroMatrix(RationalField(),S-1,S-1);
	J2:=ZeroMatrix(RationalField(),R+1,R+1);
	for i:=1 to S-1 do
		J1[i,i]:=(-1)^(i+1);
	end for;
	
	for i:=1 to R+1 do
		J2[i,i]:=(-1)^(i+1);
	end for;
	J:=KroneckerProduct(J1,J2);
	//J;
	
	N:=J+KroneckerProduct(Qmatrix(S-1),Pmatrix(R+1))-KroneckerProduct(SR(Qmatrix(S-1)),SR(Pmatrix(R+1)));
	return N;
end function;































==> Proberen/Vindingen.tex <==
% De zoektocht naar sufficient relaties. Neem aan dat $s_1+s_2+r_1+r_2$ even is. Laat $S=s_1+s_2$ en $R=r_1+r_2$
% \begin{enumerate}
%     \item Alle relaties binnen $\BD_R^S$ zijn niet voldoende om $\in\MD$ aan te tonen: voorbeeld $S=R=3$.
%     \item 
% \end{enumerate}

We hebben
\begin{align*}
    \begin{vmatrix} X_1,X_2\\Y_1,Y_2\end{vmatrix}\begin{vmatrix} X_3\\Y_3\end{vmatrix}&=\begin{vmatrix} X_1,X_2,X_3\\Y_1,Y_2,Y_3\end{vmatrix}+\begin{vmatrix} X_1,X_3,X_2\\Y_1,Y_3,Y_2\end{vmatrix}+\begin{vmatrix} X_3,X_1,X_2\\Y_3,Y_1,Y_2\end{vmatrix}+\Delta,
\end{align*}
met
\begin{align*}
    \Delta&=\sum_{k>0}\frac{B_k}{k!}(X_3-X_1)^{k-1}\left(\begin{vmatrix} X_3,X_2\\Y_1+Y_3,Y_2\end{vmatrix}+(-1)^{k-1}\begin{vmatrix} X_1,X_2\\Y_1+Y_3,Y_2\end{vmatrix}\right)\\
    &\qquad+\sum_{k>0}\frac{B_k}{k!}(X_3-X_2)^{k-1}\left(\begin{vmatrix} X_1,X_3\\Y_1,Y_2+Y_3\end{vmatrix}+(-1)^{k-1}\begin{vmatrix} X_1,X_2\\Y_1,Y_2+Y_3\end{vmatrix}\right)\\
    &\qquad+\frac{1}{X_3-X_1}\left(\begin{vmatrix} X_3,X_2\\Y_1+Y_3,Y_2\end{vmatrix}-\begin{vmatrix} X_1,X_2\\Y_1+Y_3,Y_2\end{vmatrix}\right)\\
    &\qquad+\frac{1}{X_3-X_2}\left(\begin{vmatrix} X_1,X_3\\Y_1,Y_2+Y_3\end{vmatrix}-\begin{vmatrix} X_1,X_2\\Y_1,Y_2+Y_3\end{vmatrix}\right)
\end{align*}
En dus zijn de coefficienten bij de term $X_1^{s_1-1}X_2^{s_2-1}X_3^{s_3-1}Y_1^{r_1}Y_2^{r_2}Y_3^{r_3}$ dan:
\begin{equation*}
    LHS=\begin{bmatrix} s_1,s_2\\r_1,r_2\end{bmatrix} \begin{bmatrix} s_3\\r_3\end{bmatrix},
\end{equation*}
en
\begin{align*}
    RHS&=\begin{bmatrix} s_1,s_2,s_3\\r_1,r_2,r_3\end{bmatrix}+\begin{bmatrix} s_1,s_3,s_2\\r_1,r_3,r_2\end{bmatrix}+\begin{bmatrix} s_3,s_1,s_2\\r_3,r_1,r_2\end{bmatrix}\\
    &\qquad+{r_1+r_3\choose r_1}\begin{bmatrix} s_1+s_3,s_2\\r_1+r_3,r_2\end{bmatrix}+{r_2+r_3\choose r_2}\begin{bmatrix} s_1,s_2+s_3\\r_1,r_2+r_3\end{bmatrix}\\
    &\qquad+{r_1+r_3\choose r_1}\sum_{j=1}^{s_1}\frac{(-1)^{s_3-1}B_{s_1+s_3-j}}{(s_1+s_3-j)!}{s_1+s_3-j-1\choose s_1-j}\begin{bmatrix} j,&s_2\\r_1+r_3,&r_2\end{bmatrix}\\
    &\qquad+{r_1+r_3\choose r_1}\sum_{j=1}^{s_3}\frac{(-1)^{s_1-1}B_{s_1+s_3-j}}{(s_1+s_3-j)!}{s_1+s_3-j-1\choose s_3-j}\begin{bmatrix} j,&s_2\\r_1+r_3,&r_2\end{bmatrix}\\
    &\qquad+{r_2+r_3\choose r_2}\sum_{j=1}^{s_2}\frac{(-1)^{s_3-1}B_{s_2+s_3-j}}{(s_2+s_3-j)!}{s_2+s_3-j-1\choose s_2-j}\begin{bmatrix} s_1,&j\\r_1,&r_2+r_3\end{bmatrix}\\
    &\qquad+{r_2+r_3\choose r_2}\sum_{j=1}^{s_3}\frac{(-1)^{s_2-1}B_{s_2+s_3-j}}{(s_2+s_3-j)!}{s_2+s_3-j-1\choose s_3-j}\begin{bmatrix} s_1,&j\\r_1,&r_2+r_3\end{bmatrix}.
\end{align*}

We hebben gelukkig dat het $l=3$ gedeelte wegvalt in de vergelijking
\begin{equation*}
    \left(\underbrace{\begin{bmatrix} s_1,s_2\\r_1,r_2\end{bmatrix}+\begin{bmatrix} s_2,s_1\\r_2,r_1\end{bmatrix}}_{\in\MD}\right)\begin{bmatrix} s_3\\r_3\end{bmatrix}-\left(\underbrace{\begin{bmatrix} s_3,s_1\\r_3,r_1\end{bmatrix}+\begin{bmatrix} s_1,s_3\\r_1,r_3\end{bmatrix}}_{\in\MD}\right)\begin{bmatrix} s_2\\r_2\end{bmatrix},
\end{equation*}
en deze is tevens bevat in $\MD$. Dit helpt echter niet zo veel.\\

Interessante gevallen:
Als $s_1=1$, dan in sommige gevallen krijg je maar \'e\'en term die totale som even is (en de rest even). Namelijk als $s_2=s_3$.

Observatie: Als $\bbracket{s_1,s_2,s_3\\r_1,r_2,r_3}\in \MD$ als $S+R$ even, dan ook $\bbracket{s_1,s_2\\r_1,r_2}\in \MD$. Neem $s_1=1$.\\
Geldt dit voor alle $l$? Dus als $l+1$ klopt, dan ook $l$?




\section{Partitie relatie in $l=3$}
We hebben
\begin{equation*}
    \begin{vmatrix} X_1,X_2,X_3\\Y_1,Y_2,Y_3\end{vmatrix}=\begin{vmatrix}Y_1+Y_2+Y_3,Y_1+Y_2,Y_1\\X_3,X_2-X_3,X_1-X_2\end{vmatrix}.
\end{equation*}
En dus
\begin{align*}
    LHS&=\sum_{\substack{s_1,s_2,s_3>0\\r_1,r_2,r_3\geq0}}\begin{bmatrix} s_1,s_2,s_3\\r_1,r_2,r_3\end{bmatrix}(Y_1+Y_2+Y_3)^{s_1-1}(Y_1+Y_2)^{s_2-1}Y_1^{s_3-1}X_3^{r_1}(X_2-X_3)^{r_2}(X_1-X_2)^{r_3}\\
    &=\sum_{\substack{s_1,s_2,s_3>0\\r_1,r_2,r_3\geq0}}C^{\mathbf{s}}_\mathbf{r}\begin{bmatrix} s_1,s_2,s_3\\r_1,r_2,r_3\end{bmatrix}X_1^{s_1-1}X_2^{s_2-1}X_3^{s_3-1}Y_1^{r_1}Y_1^{r_2}Y_1^{r_3},
\end{align*}
waarbij we de termen van $X_1,X_2,X_3$ kunnen expanden (en $C^{\mathbf{s}}_\mathbf{r}$ kunnen berekenen):
\begin{align*}
    X_3^{r_1}\left(\sum_{j=0}^{r_2}{r_2\choose j}X_2^{r_2-j}X_3^j\right)\left(\sum_{k=0}^{r_3}{r_3\choose k}X_2^kX_1^{r_3-k}\right)=\sum_{j=0}^{r_2}\sum_{k=0}^{r_3}{r_2\choose j}{r_3\choose k}X_1^{r_3-k}X_2^{r_2-j+k}X_3^{j+r_1}
\end{align*}
Mogelijke oplossing:
\begin{equation*}
    \sum_{j=0}^{s_3-1}\sum_{k=0}^{s_2+j-1}{s_2+j-k-1\choose j}{s_1+k-1\choose k}\begin{bmatrix} \dots\\s_3-j-1,s_2+j-k-1,s_1+k-1\end{bmatrix}(-1)^{j+k}.
\end{equation*}
Verder hebben we bij de termen $Y_1,Y_2,Y_3$
\begin{equation*}
    Y_1^{s_2-1}\sum_{l=0}^{s_1-1}{s_1-1\choose l}(Y_1+Y_2)^{s_2-1+l}Y_3^{s_1-1-l}=\sum_{l=0}^{s_1-1}\sum_{n=0}^{s_2+l-1}{s_1-1\choose l}{s_2+l-1\choose n}Y_1^{s_3-1+n}Y_2^{s_2+l-n-1}Y_3^{s_1-1-l}
\end{equation*}
met als mogelijke oplossig:
\begin{equation*}
    \sum_{n=0}^{r_1}\sum_{l=0}^{r_2+n}{r_3+l\choose l}{r_2+n\choose n}\begin{bmatrix} r_3+l+1,r_2+n-l+1,r_1+1-n\\\dots\end{bmatrix}.
\end{equation*}
We hebben dus
\begin{equation*}
    \sum_{j=0}^{s_3-1}\sum_{k=0}^{s_2+j-1}\sum_{n=0}^{r_1}\sum_{l=0}^{r_2+n}(-1)^{j+k}{s_2+j-k-1\choose j}{s_1+k-1\choose k}{r_3+l\choose l}{r_2+n\choose n}\begin{bmatrix} r_3+l+1,r_2+n-l+1,r_1+1-n\\s_3-j-1,s_2+j-k-1,s_1+k-1\end{bmatrix}
\end{equation*}

Testen:
\begin{align*}
    &P\left(\begin{bmatrix} s_1,s_2\\r_1,r_2\end{bmatrix}\begin{bmatrix} s_3\\r_3\end{bmatrix}\right)=P\left(\begin{bmatrix} s_1,s_2,s_3\\r_1,r_2,r_3\end{bmatrix}+\begin{bmatrix} s_1,s_3,s_2\\r_1,r_3,r_2\end{bmatrix}+\begin{bmatrix} s_3,s_1,s_2\\r_3,r_1,r_2\end{bmatrix}\right)=\\
    &\sum_{j=0}^{s_3-1}\sum_{k=0}^{s_2+j-1}\sum_{n=0}^{r_1}\sum_{l=0}^{r_2+n}(-1)^{j+k}{s_2+j-k-1\choose j}{s_1+k-1\choose k}{r_3+l\choose l}{r_2+n\choose n}\begin{bmatrix} r_3+l+1,r_2+n-l+1,r_1+1-n\\s_3-j-1,s_2+j-k-1,s_1+k-1\end{bmatrix}\\
    &\sum_{j=0}^{s_2-1}\sum_{k=0}^{s_3+j-1}\sum_{n=0}^{r_1}\sum_{l=0}^{r_3+n}(-1)^{j+k}{s_3+j-k-1\choose j}{s_1+k-1\choose k}{r_2+l\choose l}{r_3+n\choose n}\begin{bmatrix} r_2+l+1,r_3+n-l+1,r_1+1-n\\s_2-j-1,s_3+j-k-1,s_1+k-1\end{bmatrix}\\
    &\sum_{j=0}^{s_2-1}\sum_{k=0}^{s_1+j-1}\sum_{n=0}^{r_3}\sum_{l=0}^{r_1+n}(-1)^{j+k}{s_1+j-k-1\choose j}{s_3+k-1\choose k}{r_2+l\choose l}{r_1+n\choose n}\begin{bmatrix} r_2+l+1,r_1+n-l+1,r_3+1-n\\s_2-j-1,s_1+j-k-1,s_3+k-1\end{bmatrix}
\end{align*}
To-Do:
\begin{enumerate}
    \item programmeer dit en check of het klopt: Klopt!
    \item kijk met even/oneven of het uitkomt: flipt bij $l=3$
    \item kijk of het eventueel relaties oplevert voor $l=2$:???
    \item kijk of het ook oplosbaar is als we bijvoorbeeld de even gevallen eruit halen, we berekenen namelijk
    \begin{equation*}
        \begin{bmatrix} s_1,s_2\\r_1,r_2\end{bmatrix}\begin{bmatrix} s_3\\r_3\end{bmatrix},
    \end{equation*}
    maar we weten niet of $\begin{bmatrix} s_1,s_2\\r_1,r_2\end{bmatrix}\in\MD$. Dus checken of het voldoende is voor $\begin{bmatrix} s_1,s_2\\r_1,r_2\end{bmatrix}$ met $s_1+s_2+r_1+r_2$ oneven: Klopt niet.
\end{enumerate}

Nu willen we weten of ook deze systemen (van lengte $l=3$) op te lossen zijn. Onder de aanname dat het opgelost is voor $l=2$. Omdat de dubbele partitie
\begin{equation*}
    \begin{bmatrix} s_1,s_2\\r_1,r_2\end{bmatrix}\begin{bmatrix} s_3\\r_3\end{bmatrix}=P\left(P\left(\begin{bmatrix} s_1,s_2\\r_1,r_2\end{bmatrix}\right)\cdot P\left(\begin{bmatrix} s_3\\r_3\end{bmatrix}\right)\right)
\end{equation*}
berekenen, wordt dit vlug nasty (in ieder geval voor met de hand). Dus we kunnen ook de relaties tussen
\begin{equation*}
    P\left(\begin{bmatrix} s_1,s_2\\r_1,r_2\end{bmatrix}\begin{bmatrix} s_3\\r_3\end{bmatrix}\right)=P\left(\begin{bmatrix} s_1,s_2\\r_1,r_2\end{bmatrix}\right)\cdot P\left(\begin{bmatrix} s_3\\r_3\end{bmatrix}\right)
\end{equation*}
bekijken.

Het lijkt erop dat de statement geldt als de total weight \textbf{even} is, in het geval $l=3$. Dat betekent dat er relaties zijn voor oneven total weight. Zijn deze relaties bekend?\\

We hebben ook het system
\begin{align*}
    0\equiv& \bbracket{r_1+1,r_2+1\\s_1-1,s_2-1}+\bbracket{r_2+1,r_1+1\\s_2-1,s_1-1}\\
    0\equiv& \sum_{\substack{1\leq j\leq r_1\\ 0\leq k\leq s_2-1}}(-1)^{k}{s_1-1+k \choose k}{r_2+j \choose j}\bbracket{r_2+1+j,r_1+1-j\\ s_2-1-k,s_1-1+k}\\
    +&\sum_{\substack{1\leq j\leq r_2\\ 0\leq k\leq s_1-1}}(-1)^{k}{s_2-1+k \choose k}{r_1+j \choose j}\bbracket{r_1+1+j,r_2+1-j\\ s_1-1-k,s_2-1+k}
\end{align*}
en
\begin{align*}
    &P\left(\begin{bmatrix} s_1,s_2\\r_1,r_2\end{bmatrix}\begin{bmatrix} s_3\\r_3\end{bmatrix}\right)=P\left(\begin{bmatrix} s_1,s_2,s_3\\r_1,r_2,r_3\end{bmatrix}+\begin{bmatrix} s_1,s_3,s_2\\r_1,r_3,r_2\end{bmatrix}+\begin{bmatrix} s_3,s_1,s_2\\r_3,r_1,r_2\end{bmatrix}\right)=\\
    &\sum_{j=0}^{s_3-1}\sum_{n=0}^{r_1}(-1)^{j}{s_2+j-k-1\choose j}{r_2+n\choose n}\sum_{k=0}^{s_2+j-1}\sum_{l=0}^{r_2+n}(-1)^k{s_1+k-1\choose k}{r_3+l\choose l}\begin{bmatrix} r_3+l+1,r_2+n-l+1,r_1+1-n\\s_3-j-1,s_2+j-k-1,s_1+k-1\end{bmatrix}\\
    &\sum_{j=0}^{s_2-1}\sum_{k=0}^{s_3-1+j}\sum_{n=0}^{r_1}\sum_{l=0}^{r_3+n}(-1)^{j+k}{s_3-1+j-k\choose j}{s_1-1+k\choose k}{r_2+l\choose l}{r_3+n\choose n}\begin{bmatrix} r_2+l+1,r_3+n-l+1,r_1+1-n\\s_2-j-1,s_3+j-k-1,s_1+k-1\end{bmatrix}\\
    &\sum_{j=0}^{s_2-1}\sum_{k=0}^{s_1-1+j}\sum_{n=0}^{r_3}\sum_{l=0}^{r_1+n}(-1)^{j+k}{s_1-1+j-k\choose j}{s_3-1+k\choose k}{r_2+l\choose l}{r_1+n\choose n}\begin{bmatrix} r_2+l+1,r_1+n-l+1,r_3+1-n\\s_2-j-1,s_1+j-k-1,s_3+k-1\end{bmatrix}
\end{align*}
en
\begin{align*}
    P\left(\bbracket{s_1,s_2\\r_1,r_2}\right)P\left(\bbracket{s_3\\r_3}\right)&=\left(\sum_{\substack{1\leq j\leq r_1\\ 0\leq k\leq s_2-1}}(-1)^{k}{s_1-1+k \choose k}{r_2+j \choose j}\bbracket{r_2+1+j,r_1+1-j\\ s_2-1-k,s_1-1+k}\right.\\
    +&\left.\sum_{\substack{1\leq j\leq r_2\\ 0\leq k\leq s_1-1}}(-1)^{k}{s_2-1+k \choose k}{r_1+j \choose j}\bbracket{r_1+1+j,r_2+1-j\\ s_1-1-k,s_2-1+k}\right)P\left(\bbracket{s_3\\r_3}\right)
\end{align*}



\clearpage
\subsection{Breakdown of $l=2$, odd weigth proposition}
We prove that the system
\begin{align*}
    0\equiv \bbracket{z_{s_1,r_1}\diam z_{s_2,r_2}}&=\bbracket{z_{s_1,r_1}z_{s_2,r_2}} +\bbracket{z_{s_2,r_2}z_{s_1,r_1}}\\
    0\equiv \bbracket{z_{s_1,r_1}\shaf z_{s_2,r_2}}&=\sum_{\substack{1\leq l\leq s_1\\ 0\leq k\leq r_2}}{s_1+s_2-l-1 \choose s_2-1}{r_1+r_2-k \choose r_1}(-1)^{r_2-k}\bbracket{z_{s_1+s_2-l,k}z_{l,r_1+r_2-k}}\nonumber\\
    &\quad+\sum_{\substack{1\leq l\leq s_2\\ 0\leq k\leq r_1}}{s_1+s_2-l-1 \choose s_1-1}{r_1+r_2-k \choose r_2}(-1)^{r_1-k}\bbracket{z_{s_1+s_2-l,k}z_{l,r_1+r_2-k}}.
\end{align*}
can be solved for $\bbracket{z_{s_1,r_1}z_{s_2,r_2}}$. I will try and figure out what is happening here. For a word $z_{s_1,r_1}z_{s_2,r_2}$ we know that the partition relation is given by  
\begin{equation*}
    P(z_{s_1,r_1}z_{s_2,r_2})=\sum_{\substack{0\leq l\leq r_1\\0\leq k\leq s_2-1}}(-1)^k{s_1-1+k\choose k}{r_2+l\choose l} z_{r_2+1+l,s_2-1-k}z_{r_1+1-l,s_1-1+k}.
\end{equation*}
Consider the space $Z(S,R)\subseteqq\Q\langle A_\BD\rangle$ to be the set of all words $z_{s_1,r_1}\cdots z_{s_l,r_l}$ with $s_1+\dots+s_l=S$ and $r_1+\dots+r_l=R$. Then $P$ acts as a map $P\colon Z(S,R)\to Z(R+2,S-2)$. Furthermore, since we have $P^2=\id$, we know that $P$ is a bijection. Now consider the system 
\begin{align*}
    0\equiv \bbracket{P(z_{s_1,r_1}\diam z_{s_2,r_2})}\\
    0\equiv \bbracket{P(z_{s_1,r_1})\diam P(z_{s_2,r_2})},
\end{align*}
which is
\begin{align*}
    0\equiv \bbracket{P(z_{s_1,r_1}z_{s_2,r_2})+P(z_{s_2,r_2}z_{s_1,r_1})}\\
    0\equiv \bbracket{z_{r_1+1,s_1-1}z_{r_2+1,s_1-1}+z_{r_2+1,s_1-1}z_{r_1+1,s_1-1}}.
\end{align*}
We differentiate between two partition-like maps $P_i\colon Z(S,R)\to Z(R+2,S-2)$, for $i=1,2$, defined by $P_1=P$ and $P_2(z_{s_1,r_1}z_{s_2,r_2})=P(z_{s_2,r_2}z_{s_1,r_1})$. So we have
\begin{align*}
    0\equiv \bbracket{P_1(z_{s_1,r_1}z_{s_2,r_2})+P_2(z_{s_1,r_1}z_{s_2,r_2})}\\
    0\equiv \bbracket{z_{r_1+1,s_1-1}z_{r_2+1,s_1-1}+z_{r_2+1,s_1-1}z_{r_1+1,s_1-1}}.
\end{align*}
We again have $P_i^2=\id$.\\

The inverse of $$P_{S-1}\otimes Q_{R+1}-P_{S-1}^{\rho\sigma}\otimes Q_{R+1}^{\rho\sigma}$$ is $$\frac{1}{2}\big(M_{S,R}+Q_{S-1}\otimes P_{R+1}-Q_{S-1}^{\rho\sigma}\otimes P_{R+1}^{\rho\sigma}\big).$$
So we have
\begin{align*}
    \bbracket{z_{S-n,R+1-m} z_{n,m-1}}&=\frac{1}{2}(-1)^{n+m}\bbracket{z_{s-n,R+1-m}\shuf z_{n,m-1}}\\
    &+\frac{1}{2}\sum_{\substack{1\leq l \leq S-1\\ 1\leq k\leq R+1}}{R+1-k\choose m-1}{l-1\choose S-1-n}(-1)^{S+n+l}\bbracket{z_{s-l,R+1-k}\shuf z_{l,k-1}}\\
    &-\frac{1}{2}\sum_{\substack{1\leq l \leq S-1\\ 1\leq k\leq R+1}}{R+1-k\choose m-k}{l-1\choose n}(-1)^{n+l+1}\bbracket{ z_{l,k-1}\shuf z_{s-l,R+1-k}}.
\end{align*}
Original system:
\begin{align}
    0&\equiv\sum_{\substack{1\leq l\leq S-1\\ 1\leq k\leq R+1}}{S-1-l \choose n-1}{k-1 \choose R+1-m}(-1)^{R+m+k}\begin{bmatrix}z_{S-l,R+1-k}z_{l,k-1}\end{bmatrix}\nonumber\\
    &\quad-\sum_{\substack{1\leq l\leq S-1\\ 1\leq k\leq R+1}}{S-1-l \choose n-l}{k-1 \choose m}(-1)^{m+k+1}\begin{bmatrix}z_{l,k-1}z_{S-l,R+1-k}\end{bmatrix}.
\end{align}
\newpage

\section{Alternatives of the proof of the odd-weight theorem}
Consider the space $Z(S,R;l)\subseteq\Q\langle A_\BD\rangle$ to be the set of all words $z_{s_1,r_1}\cdots z_{s_l,r_l}$ of length $l$ with $s_1+\dots+s_l=S$ and $r_1+\dots+r_l=R$. Then the partition relation $P$ is a map $P\colon Z(S,R;l)\to Z(R+l,S-l;l)$. Fix $l=2$.
Define the map $\nu\bbracket{s_1,s_2\\r_1,r_2}=\bbracket{s_2,s_1\\r_2,r_1}$. We have
\begin{align*}
    0\equiv P\bbracket{s_1,s_2\\r_1,r_2}+P\nu\bbracket{s_1,s_2\\r_1,r_2}\\
    0\equiv \bbracket{s_1,s_2\\r_1,r_2}+\nu\bbracket{s_1,s_2\\r_1,r_2}.
\end{align*}
Then the odd-weight proposition states that the system $0\equiv \big(P-\nu P\nu\big) \bbracket{s_1,s_2\\r_1,r_2}$ has a solution if $s_1+s_2+r_1+r_2$ is odd. I.e., the map $P-\nu P\nu$ has an inverse. \\

We know that $P^2=\id$ and $\nu^2=\id$, so that $(-\nu P\nu)^2=\nu P\nu\nu P\nu=\id$. 
We can explicitly prove (see proof of odd-weight thereom) the relations 
\begin{align}
    P\nu P\nu&=-\nu P\nu J\hphantom{\nu P\nu P = PJ}\text{(when $S+R$ odd)}\label{PnuPnu}\\
    \nu P\nu P &= PJ \hphantom{P\nu P\nu=-\nu P\nu J}\text{(always)}\label{nuPnuP}
\end{align}
Here, we defined
\begin{equation*}
    J\bbracket{s_1,s_2\\r_1,r_2}=(-1)^{s_2+r_2}\bbracket{s_1,s_2\\r_1,r_2}.
\end{equation*}
(Even de factor $(-1)^{\dots}$ checken). We have
\begin{align*}
    J\nu\bbracket{s_1,s_2\\r_1,r_2}&=J\bbracket{s_2,s_1\\r_2,r_1}=(-1)^{s_1+r_1}\bbracket{s_2,s_1\\r_2,r_1},\\
    \nu J\bbracket{s_1,s_2\\r_1,r_2}&=\nu (-1)^{s_2+r_2}\bbracket{s_1,s_2\\r_1,r_2}=(-1)^{s_2+r_2}\bbracket{s_2,s_1\\r_2,r_1}.
\end{align*}
This means that $\nu J\bbracket{s_1,s_2\\r_1,r_2}=(-1)^{s_1+s_2+r_1+r_2}J \nu\bbracket{s_1,s_2\\r_1,r_2}$ (useful?). Hence relation (\ref{PnuPnu}) follows from relation (\ref{nuPnuP}). Question: can we prove relation (\ref{nuPnuP}) (in a perhaps not explicit way)?\\

Let $l=3$. Let $P$ be the partition relation. Define the maps $y_i$ for $i=1,2,3$ to be 
\begin{align*}
    y_1(z_{s_1,r_1}z_{s_2,r_2}z_{s_3,r_3})&=z_{s_3,r_3}z_{s_1,r_1}z_{s_2,r_2}\\
    y_2(z_{s_1,r_1}z_{s_2,r_2}z_{s_3,r_3})&=z_{s_1,r_1}z_{s_3,r_3}z_{s_2,r_2}\\
    y_3(z_{s_1,r_1}z_{s_2,r_2}z_{s_3,r_3})&=z_{s_1,r_1}z_{s_2,r_2}z_{s_3,r_3}.
\end{align*}
Define the fixed partition $P_i$ to be
\begin{align*}
    P_i(z_{s_1,r_1}z_{s_2,r_2}z_{s_3,r_3})=y_i(P(z_{s_1,r_1}z_{s_2,r_2})z_{s_3,r_3}).
\end{align*}
This means that we have
\begin{equation*}
    P(z_{s_1,r_1}z_{s_2,r_2})P(z_{s_3,r_3})=(P_1+P_2+P_3)(z_{s_1,r_1}z_{s_2,r_2}z_{s_3,r_3})
\end{equation*}





































\newpage
The idea:\\
Define $K^l_{even}/K^l_{odd}$ to be the statement: "If $s_1+\dots+s_l+r_1+\dots+r_l$ is even/odd, then the bi-bracket $\bbracket{s_1,\dots,s_l\\r_1,\dots,r_l}$ can be written as a linear combination of mono-brackets". We know that $K^1_{even}, K_{odd}^1$ and $K_{odd}^2$ are true.

\begin{proposition}
Assume that $K^3_{odd}$ is true. Then we know that $K^2_{even}$ is true.
\end{proposition}
\begin{proof}
Consider the integers $s_1,s_2,r_1,r_2$ with $s_1+s_2+r_1+r_2$ even. We have
\begin{align*}
    \bbracket{s_1,s_2\\r_1,r_2}\bbracket{1\\0}&=\bbracket{s_1,s_2,1\\r_1,r_2,0}+\bbracket{s_1,1,s_2\\r_1,0,r_2}+\bbracket{1,s_1,s_2\\0,r_1,r_2}+\bbracket{s_1+1,s_2\\r_1,r_2}+\bbracket{s_1,s_2+1\\r_1,r_2}\\
    &+\sum_{j=1}^{s_1}\frac{B_{s_1+1-j}}{(s_1+1-j)!}\bbracket{j,s_2\\r_1,r_2}+(-1)^{s_1-1}\frac{B_{s_1}}{s_1!}\bbracket{1,s_2\\r_1,r_2}\\
    &+\sum_{j=1}^{s_2}\frac{B_{s_2+1-j}}{(s_2+1-j)!}\bbracket{s_1,j\\r_1,r_2}+(-1)^{s_2-1}\frac{B_{s_2}}{s_2!}\bbracket{s_1,1\\r_1,r_2}.
\end{align*}
Since we assumed that $K^3_{odd}$ holds, we see that the first three terms are in $\MD$. We also know that $K^2_{odd}$ holds, which means that the fourth and fifth term are also in $\MD$. Now consider the first term of the remaining terms. Note that $B_k=0$ if $k>1$ is odd. This means that for $j\neq s_1$ we either have that $B_{s_1+1-j}=0$ (because $s_1+1-j>1$ is odd), or that $j+s_2+r_1+r_2$ has the same parity as $s_1+s_2+r_1+r_2$. In the latter case, we again note that we have $K_{odd}^2$. If $j=s_1$, we obtain the term
\begin{equation*}
    -\frac{1}{2}\bbracket{s_1,s_2\\r_1,r_2}.
\end{equation*}
The same argument holds for the other remaining terms. And hence we have
\begin{align*}
    \bbracket{s_1,s_2\\r_1,r_2}&=\bbracket{s_1,s_2\\r_1,r_2}\bbracket{1\\0}-\bbracket{s_1,s_2,1\\r_1,r_2,0}-\bbracket{s_1,1,s_2\\r_1,0,r_2}-\bbracket{1,s_1,s_2\\0,r_1,r_2}-\bbracket{s_1+1,s_2\\r_1,r_2}-\bbracket{s_1,s_2+1\\r_1,r_2}\\
    &-\sum_{j=1}^{s_1-1}\frac{B_{s_1+1-j}}{(s_1+1-j)!}\bbracket{j,s_2\\r_1,r_2}+(-1)^{s_1}\frac{B_{s_1}}{s_1!}\bbracket{1,s_2\\r_1,r_2}\\
    &-\sum_{j=1}^{s_2-1}\frac{B_{s_2+1-j}}{(s_2+1-j)!}\bbracket{s_1,j\\r_1,r_2}+(-1)^{s_2}\frac{B_{s_2}}{s_2!}\bbracket{s_1,1\\r_1,r_2},
\end{align*}
which can be written (assuming $K^3_{odd}$ and $K^2_{odd}$) as a linear combination of mono-brackets.
\end{proof}
\textbf{Problem:}
Of course we do not know whether $\bbracket{s_1,s_2\\r_1,r_2}\bbracket{1\\0}$ can be written as a combination of mono-brackets.
\newpage
Let $l=3$. Let $P$ be the partition relation. Define the maps $y_i$ for $i=1,2,3$ to be 
\begin{align*}
    y_1(z_{s_1,r_1}z_{s_2,r_2}z_{s_3,r_3})&=z_{s_3,r_3}z_{s_1,r_1}z_{s_2,r_2}\\
    y_2(z_{s_1,r_1}z_{s_2,r_2}z_{s_3,r_3})&=z_{s_1,r_1}z_{s_3,r_3}z_{s_2,r_2}\\
    y_3(z_{s_1,r_1}z_{s_2,r_2}z_{s_3,r_3})&=z_{s_1,r_1}z_{s_2,r_2}z_{s_3,r_3}.
\end{align*}
% Define the fixed partition $P_i$ to be
% \begin{align*}
%     P_i(z_{s_1,r_1}z_{s_2,r_2}z_{s_3,r_3})=y_i(P(z_{s_1,r_1}z_{s_2,r_2})P(z_{s_3,r_3})).
% \end{align*}
% This means that we have
% \begin{equation*}
%     P(z_{s_1,r_1}z_{s_2,r_2})P(z_{s_3,r_3})=(P_1+P_2+P_3)(z_{s_1,r_1}z_{s_2,r_2}z_{s_3,r_3})
% \end{equation*}
The system (modulo length $2$) in length $l=3$ looks like
\begin{align*}
    \bbracket{z_{s_1,r_1}z_{s_2,r_2}}\bbracket{z_{s_3,r_3}}&\equiv \bbracket{z_{s_1,r_1}z_{s_2,r_2}z_{s_3,r_3}}+\bbracket{z_{s_1,r_1}z_{s_3,r_3}z_{s_2,r_2}}+\bbracket{z_{s_3,r_3}z_{s_1,r_1}z_{s_2,r_2}}\\
    &\equiv \bbracket{(y_1+y_2+y_3)z_{s_1,r_1}z_{s_2,r_2}z_{s_3,r_3}}\\
    \bbracket{z_{s_1,r_1}z_{s_2,r_2}}\bbracket{z_{s_3,r_3}}&\equiv\bbracket{(Py_1+Py_2+Py_3)P(z_{s_1,r_1}z_{s_2,r_2})P(z_{s_3,r_3})}.
\end{align*}


\subsection{Length $3$}
In length $3$ things are more complicated. Consider the system generated by the stuffle products $z_{s_1,r_1}z_{s_2,r_2}\ast z_{s_3,r_3}$ and shuffle products $z_{s_1,r_1}z_{s_2,r_2}\shuffle z_{s_3,r_3}$. In length $2$, we knew that these products were $\equiv0$ mod $\MD$. However, we only know that bi-brackets of length $2$ with even total weight are $\equiv0$ mod $\MD$.
For example, if $S=4$ and $R=0$, we have the system
\begin{alignat*}{3}
    z_{2,0}z_{1,0}\ast z_{1,0}&=2z_{2,0}z_{1,0}z_{1,0}+&&\phantom{2}z_{1,0}z_{2,0}z_{1,0}\\
    z_{1,0}z_{2,0}\ast z_{1,0}&=&&\phantom{2}z_{1,0}z_{2,0}z_{1,0}+&&2z_{1,0}z_{1,0}z_{2,0}\\
    z_{1,0}z_{1,0}\ast z_{2,0}&=\phantom{2}z_{2,0}z_{1,0}z_{1,0}+&&\phantom{2}z_{1,0}z_{2,0}z_{1,0}+&&\phantom{2}z_{1,0}z_{1,0}z_{2,0}\\
    z_{2,0}z_{1,0}\shuffle z_{1,0}&=3z_{2,0}z_{1,0}z_{1,0}+&&\phantom{2}z_{1,0}z_{2,0}z_{1,0}\\
    z_{1,0}z_{2,0}\shuffle z_{1,0}&=&&2z_{1,0}z_{2,0}z_{1,0}+&&2z_{1,0}z_{1,0}z_{2,0}\\
    z_{1,0}z_{1,0}\shuffle z_{2,0}&=3z_{2,0}z_{1,0}z_{1,0}+&&2z_{1,0}z_{2,0}z_{1,0}+&&\phantom{2}z_{1,0}z_{1,0}z_{2,0},
\end{alignat*}
which corresponds to the matrix
\begin{equation*}
\begin{pmatrix}
2& 1& 0\\
0& 1& 2\\
1& 1& 1\\
3& 1& 0\\
0& 2& 2\\
3& 2& 1
\end{pmatrix}.
\end{equation*}
This system of equations can be solved for $z_{2,0}z_{1,0}z_{1,0},z_{1,0}z_{2,0}z_{1,0}$ and $z_{1,0}z_{1,0}z_{2,0}$, so that they can be expressed as a linear combination of the stuffle/shuffle products.\\

A computer search $S,R\leq 10$ shows that this system can be solved if $S+R$ is even. \\

We have the relation
\begin{equation*}
    z_{s_2,r_2}z_{s_3,r_3}\ast z_{s_1,r_1}-z_{s_2,r_2}z_{s_1,r_1}\ast z_{s_3,r_3}=z_{s_1,r_1}z_{s_2,r_2}z_{s_3,r_3}-z_{s_3,r_3}z_{s_2,r_2}z_{s_1,r_1},
\end{equation*}
or
\begin{equation*}
    \bbracket{s_2,s_3\\r_2,r_3}\bbracket{s_1\\r_1}- \bbracket{s_2,s_1\\r_2,r_1}\bbracket{s_3\\r_3}=
    \bbracket{s_1,s_2,s_3\\r_1,r_2,r_3}-\bbracket{s_3,s_2,s_1\\r_3,r_2,r_1}.
\end{equation*}
Note that this is similar to the stuffle product in length $2$:
\begin{equation*}
    z_{s_1,r_1}\ast z_{s_2,r_2}=z_{s_1,r_1}z_{s_2,r_2}+z_{s_2,r_2}z_{s_1,r_1},
\end{equation*}
or
\begin{equation*}
    \bbracket{s_1\\r_1} \bbracket{s_2\\r_2}=\bbracket{s_1,s_2\\r_1,r_2}+\bbracket{s_2,s_1\\r_2,r_1}.
\end{equation*}
If we instead assume the relation $z_{s_1,r_1}z_{s_2,r_2}z_{s_3,r_3}-z_{s_3,r_3}z_{s_2,r_2}z_{s_1,r_1}$, we obtain the alternative system
\begin{align}
\label{system:l3 alternative}
    \bbracket{z_{s_2,r_2}z_{s_3,r_3}}\bbracket{z_{s_1,r_1}}-\bbracket{z_{s_2,r_2}z_{s_1,r_1}}\bbracket{z_{s_3,r_3}}&\equiv \bbracket{z_{s_1,r_1}z_{s_2,r_2}z_{s_3,r_3}}+\bbracket{z_{s_3,r_3}z_{s_2,r_2}z_{s_1,r_1}}\\
    \bbracket{z_{s_1,r_1}z_{s_2,r_2}}\bbracket{z_{s_3,r_3}}&\equiv\bbracket{P(P(z_{s_1,r_1}z_{s_2,r_2})P(z_{s_3,r_3}))}.\nonumber
\end{align}
% \begin{alignat*}{3}
%     z_{2,0}z_{1,0}\ast z_{1,0}&=2z_{2,0}z_{1,0}z_{1,0}+&&\phantom{2}z_{1,0}z_{2,0}z_{1,0}\\
%     z_{1,0}z_{2,0}\ast z_{1,0}&=&&\phantom{2}z_{1,0}z_{2,0}z_{1,0}+&&2z_{1,0}z_{1,0}z_{2,0}\\
%     z_{1,0}z_{1,0}\ast z_{2,0}&=\phantom{2}z_{2,0}z_{1,0}z_{1,0}+&&\phantom{2}z_{1,0}z_{2,0}z_{1,0}+&&\phantom{2}z_{1,0}z_{1,0}z_{2,0}\\
%     z_{2,0}z_{1,0}\shuffle z_{1,0}&=3z_{2,0}z_{1,0}z_{1,0}+&&\phantom{2}z_{1,0}z_{2,0}z_{1,0}\\
%     z_{1,0}z_{2,0}\shuffle z_{1,0}&=&&2z_{1,0}z_{2,0}z_{1,0}+&&2z_{1,0}z_{1,0}z_{2,0}\\
%     z_{1,0}z_{1,0}\shuffle z_{2,0}&=3z_{2,0}z_{1,0}z_{1,0}+&&2z_{1,0}z_{2,0}z_{1,0}+&&\phantom{2}z_{1,0}z_{1,0}z_{2,0},
% \end{alignat*}
In our example, this corresponds to the matrix
\begin{equation*}
\begin{pmatrix}
 1&  0& -1\\
 0&  0&  0\\
-1&  0&  1\\
 3&  1&  0\\
 0&  2&  2\\
 3&  2&  1
\end{pmatrix},
\end{equation*}
which is full in rank. A computer search shows ($S,R\leq 10$) that this system is full in rank if $S+R$ is even. Because system \ref{system:l3 alternative} is similar to the one we studied in the case of length $2$, there perhaps is a similar way of proving that this system has a solution.

==> Proberen/adfa.tex <==
% {{0, 0, 1, 0, 0, 1, 0, 0, 1, -1, 1, 0}, {0, 1, -2, 0, 1, -2, 0, 1, -2,
%   2, 0, -2}, {, -1, 1, 1, -1, 1, 1, -1, 1, 0, -1, 1}, {0, 0, 3, 0, 
%   0, 2, -1, 1, 0, -3, 3, -3}, {0, 3, -6, 0, 2, -4, 2, 0, -2, 6, -3, 
%   0}, {, -3, 3, 2, -2, 2, 0, -1, 1, -3, 0, 0}, {0, 0, 3, -1, 1, 
%   0, -2, 2, -2, -3, 3, -3}, {0, 3, -6, 2, 0, -2, 4, -2, 0, 6, -3, 
%   0}, {, -3, 3, 0, -1, 1, -2, 0, 0, -3, 0, 0}, {-1, 1, 0, -1, 
%   1, -1, -1, 1, -1, -1, 1, -1}, {2, 0, -2, 2, -1, 0, 2, -1, 0, 2, -1, 
%   0}, {, -1, 1, -1, 0, 0, -1, 0, 0, -1, 0, 0}}
  
%   {
%     { 0, 0, 0, 0, 1, 0, 0, 0, 0, 1, 0, 0, 0, 0, 1, -1, 1, -1, 1, 0 },
%     { 0, 0, 0, 1, -4, 0, 0, 0, 1, -4, 0, 0, 0, 1, -4, 4, -3, 2, 0, -4 },
%     { 0, 0, 1, -3, 6, 0, 0, 1, -3, 6, 0, 0, 1, -3, 6, -6, 3, 0, -3, 6 },
%     { 0, 1, -2, 3, -4, 0, 1, -2, 3, -4, 0, 1, -2, 3, -4, 4, 0, -2, 3, -4 },
%     { 1, -1, 1, -1, 1, 1, -1, 1, -1, 1, 1, -1, 1, -1, 1, 0, -1, 1, -1, 1 },
%     { 0, 0, 0, 0, 3, 0, 0, 0, 0, 2, -1, 1, -1, 1, 0, -3, 3, -3, 3, -3 },
%     { 0, 0, 0, 3, -12, 0, 0, 0, 2, -8, 4, -3, 2, 0, -4, 12, -9, 6, -3, 0 },
%     { 0, 0, 3, -9, 18, 0, 0, 2, -6, 12, -6, 3, 0, -3, 6, -18, 9, -3, 0, 0 },
%     { 0, 3, -6, 9, -12, 0, 2, -4, 6, -8, 4, 0, -2, 3, -4, 12, -3, 0, 0, 0 },
%     { 3, -3, 3, -3, 3, 2, -2, 2, -2, 2, 0, -1, 1, -1, 1, -3, 0, 0, 0, 0 },
%     { 0, 0, 0, 0, 3, -1, 1, -1, 1, 0, -2, 2, -2, 2, -2, -3, 3, -3, 3, -3 },
%     { 0, 0, 0, 3, -12, 4, -3, 2, 0, -4, 8, -6, 4, -2, 0, 12, -9, 6, -3, 0 },
%     { 0, 0, 3, -9, 18, -6, 3, 0, -3, 6, -12, 6, -2, 0, 0, -18, 9, -3, 0, 0 },
%     { 0, 3, -6, 9, -12, 4, 0, -2, 3, -4, 8, -2, 0, 0, 0, 12, -3, 0, 0, 0 },
%     { 3, -3, 3, -3, 3, 0, -1, 1, -1, 1, -2, 0, 0, 0, 0, -3, 0, 0, 0, 0 },
%     { -1, 1, -1, 1, 0, -1, 1, -1, 1, -1, -1, 1, -1, 1, -1, -1, 1, -1, 1, -1 },
%     { 4, -3, 2, 0, -4, 4, -3, 2, -1, 0, 4, -3, 2, -1, 0, 4, -3, 2, -1, 0 },
%     { -6, 3, 0, -3, 6, -6, 3, -1, 0, 0, -6, 3, -1, 0, 0, -6, 3, -1, 0, 0 },
%     { 4, 0, -2, 3, -4, 4, -1, 0, 0, 0, 4, -1, 0, 0, 0, 4, -1, 0, 0, 0 },
%     { 0, -1, 1, -1, 1, -1, 0, 0, 0, 0, -1, 0, 0, 0, 0, -1, 0, 0, 0, 0 }
% }


{
    { 0, 0, 0, 0, 1, 0, 0, 0, 0, 1, -1, 1, -1, 1, 0 },
    { 0, 0, 0, 1, -4, 0, 0, 0, 1, -4, 4, -3, 2, 0, -4 },
    { 0, 0, 1, -3, 6, 0, 0, 1, -3, 6, -6, 3, 0, -3, 6 },
    { 0, 1, -2, 3, -4, 0, 1, -2, 3, -4, 4, 0, -2, 3, -4 },
    { 1, -1, 1, -1, 1, 1, -1, 1, -1, 1, 0, -1, 1, -1, 1 },
    { 0, 0, 0, 0, 2, -1, 1, -1, 1, 0, -2, 2, -2, 2, -2 },
    { 0, 0, 0, 2, -8, 4, -3, 2, 0, -4, 8, -6, 4, -2, 0 },
    { 0, 0, 2, -6, 12, -6, 3, 0, -3, 6, -12, 6, -2, 0, 0 },
    { 0, 2, -4, 6, -8, 4, 0, -2, 3, -4, 8, -2, 0, 0, 0 },
    { 2, -2, 2, -2, 2, 0, -1, 1, -1, 1, -2, 0, 0, 0, 0 },
    { -1, 1, -1, 1, 0, -1, 1, -1, 1, -1, -1, 1, -1, 1, -1 },
    { 4, -3, 2, 0, -4, 4, -3, 2, -1, 0, 4, -3, 2, -1, 0 },
    { -6, 3, 0, -3, 6, -6, 3, -1, 0, 0, -6, 3, -1, 0, 0 },
    { 4, 0, -2, 3, -4, 4, -1, 0, 0, 0, 4, -1, 0, 0, 0 },
    { 0, -1, 1, -1, 1, -1, 0, 0, 0, 0, -1, 0, 0, 0, 0 }
}

{
    { 0, 0, 0, 1, 1, -1, 1, 0 },
    { 0, 0, 1, -3, -3, 2, 0, -3 },
    { 0, 1, -2, 3, 3, 0, -2, 3 },
    { 1, -1, 1, -1, 0, -1, 1, -1 },
    { 1, -1, 1, 0, 1, -1, 1, -1 },
    { -3, 2, 0, -3, -3, 2, -1, 0 },
    { 3, 0, -2, 3, 3, -1, 0, 0 },
    { 0, -1, 1, -1, -1, 0, 0, 0 }
}


{
    { 0, 0, 0, 0, 0, 1, 0, 0, 0, 0, 0, 1, 1, -1, 1, -1, 1, 0 },
    { 0, 0, 0, 0, 1, -5, 0, 0, 0, 0, 1, -5, -5, 4, -3, 2, 0, -5 },
    { 0, 0, 0, 1, -4, 10, 0, 0, 0, 1, -4, 10, 10, -6, 3, 0, -4, 10 },
    { 0, 0, 1, -3, 6, -10, 0, 0, 1, -3, 6, -10, -10, 4, 0, -3, 6, -10 },
    { 0, 1, -2, 3, -4, 5, 0, 1, -2, 3, -4, 5, 5, 0, -2, 3, -4, 5 },
    { 1, -1, 1, -1, 1, -1, 1, -1, 1, -1, 1, -1, 0, -1, 1, -1, 1, -1 },
    { 0, 0, 0, 0, 0, 2, 1, -1, 1, -1, 1, 0, 2, -2, 2, -2, 2, -2 },
    { 0, 0, 0, 0, 2, -10, -5, 4, -3, 2, 0, -5, -10, 8, -6, 4, -2, 0 },
    { 0, 0, 0, 2, -8, 20, 10, -6, 3, 0, -4, 10, 20, -12, 6, -2, 0, 0 },
    { 0, 0, 2, -6, 12, -20, -10, 4, 0, -3, 6, -10, -20, 8, -2, 0, 0, 0 },
    { 0, 2, -4, 6, -8, 10, 5, 0, -2, 3, -4, 5, 10, -2, 0, 0, 0, 0 },
    { 2, -2, 2, -2, 2, -2, 0, -1, 1, -1, 1, -1, -2, 0, 0, 0, 0, 0 },
    { 1, -1, 1, -1, 1, 0, 1, -1, 1, -1, 1, -1, 1, -1, 1, -1, 1, -1 },
    { -5, 4, -3, 2, 0, -5, -5, 4, -3, 2, -1, 0, -5, 4, -3, 2, -1, 0 },
    { 10, -6, 3, 0, -4, 10, 10, -6, 3, -1, 0, 0, 10, -6, 3, -1, 0, 0 },
    { -10, 4, 0, -3, 6, -10, -10, 4, -1, 0, 0, 0, -10, 4, -1, 0, 0, 0 },
    { 5, 0, -2, 3, -4, 5, 5, -1, 0, 0, 0, 0, 5, -1, 0, 0, 0, 0 },
    { 0, -1, 1, -1, 1, -1, -1, 0, 0, 0, 0, 0, -1, 0, 0, 0, 0, 0 }
}


{
{  1,  -1,   1,  -1,   1,   0,   0,   0,   0,   0,   0,   1,   0,   0,   0,   0,   0,   1},
{  0,   1,  -2,   3,  -3,   0,   0,   0,   0,   0,   1,  -5,   0,   0,   0,   0,   1,  -5},
{  0,   0,   1,  -2,   2,   0,   0,   0,   0,   1,  -4,  10,   0,   0,   0,   1,  -4,  10},
{  0,   0,   1,  -2,   2,   0,   0,   0,   1,  -3,   6, -10,   0,   0,   1,  -3,   6, -10},
{  0,   1,  -2,   3,  -3,   0,   0,   1,  -2,   3,  -4,   5,   0,   1,  -2,   3,  -4,   5},
{  1,  -1,   1,  -1,   1,   0,   1,  -1,   1,  -1,   1,  -1,   1,  -1,   1,  -1,   1,  -1},
{  2,  -2,   2,  -2,   2,   0,   1,  -1,   1,  -1,   1,   0,   0,   0,   0,   0,   0,   0},
{  0,   2,  -4,   6,  -6,   0,   0,   1,  -2,   3,  -3,   0,   0,   0,   0,   0,   0,   0},
{  0,   0,   2,  -4,   4,   0,   0,   0,   1,  -2,   2,   0,   0,   0,   0,   0,   0,   0},
{  0,   0,   2,  -4,   4,   0,   0,   0,   1,  -2,   2,   0,   0,   0,   0,   0,   0,   0},
{  0,   2,  -4,   6,  -6,   0,   0,   1,  -2,   3,  -3,   0,   0,   0,   0,   0,   0,   0},
{  2,  -2,   2,  -2,   2,   0,   1,  -1,   1,  -1,   1,   0,   0,   0,   0,   0,   0,   0},
{  1,  -1,   1,  -1,   1,   0,   1,  -1,   1,  -1,   1,  -1,   1,  -1,   1,  -1,   1,  -1},
{  0,   1,  -2,   3,  -3,   0,   0,   1,  -2,   3,  -4,   5,   0,   1,  -2,   3,  -4,   5},
{  0,   0,   1,  -2,   2,   0,   0,   0,   1,  -3,   6, -10,   0,   0,   1,  -3,   6, -10},
{  0,   0,   1,  -2,   2,   0,   0,   0,   0,   1,  -4,  10,   0,   0,   0,   1,  -4,  10},
{  0,   1,  -2,   3,  -3,   0,   0,   0,   0,   0,   1,  -5,   0,   0,   0,   0,   1,  -5},
{  1,  -1,   1,  -1,   1,   0,   0,   0,   0,   0,   0,   1,   0,   0,   0,   0,   0,   1},
{  1,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   1},
{  0,   1,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   1,   0},
{  0,   0,   1,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   1,   0,   0},
{  0,   0,   0,   1,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   1,   0,   0,   0},
{  0,   0,   0,   0,   1,   0,   0,   0,   0,   0,   0,   0,   0,   1,   0,   0,   0,   0},
{  0,   0,   0,   0,   0,   1,   0,   0,   0,   0,   0,   0,   1,   0,   0,   0,   0,   0},
{  0,   0,   0,   0,   0,   0,   1,   0,   0,   0,   0,   1,   0,   0,   0,   0,   0,   0},
{  0,   0,   0,   0,   0,   0,   0,   1,   0,   0,   1,   0,   0,   0,   0,   0,   0,   0},
{  0,   0,   0,   0,   0,   0,   0,   0,   1,   1,   0,   0,   0,   0,   0,   0,   0,   0}
}
{{  1,  -1,   1,  -1,   1,   0,   0,   0,   0,   0,   0,   1,   0,   0,   0,   0,   0,   1},
{  0,   1,  -2,   3,  -3,   0,   0,   0,   0,   0,   1,  -5,   0,   0,   0,   0,   1,  -5},
{  0,   0,   1,  -2,   2,   0,   0,   0,   0,   1,  -4,  10,   0,   0,   0,   1,  -4,  10},
{  0,   0,   1,  -2,   2,   0,   0,   0,   1,  -3,   6, -10,   0,   0,   1,  -3,   6, -10},
{  0,   1,  -2,   3,  -3,   0,   0,   1,  -2,   3,  -4,   5,   0,   1,  -2,   3,  -4,   5},
{  1,  -1,   1,  -1,   1,   0,   1,  -1,   1,  -1,   1,  -1,   1,  -1,   1,  -1,   1,  -1},
{  2,  -2,   2,  -2,   2,   0,   1,  -1,   1,  -1,   1,   0,   0,   0,   0,   0,   0,   0},
{  0,   2,  -4,   6,  -6,   0,   0,   1,  -2,   3,  -3,   0,   0,   0,   0,   0,   0,   0},
{  0,   0,   2,  -4,   4,   0,   0,   0,   1,  -2,   2,   0,   0,   0,   0,   0,   0,   0},
{  1,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   1},
{  0,   1,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   1,   0},
{  0,   0,   1,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   1,   0,   0},
{  0,   0,   0,   1,   0,   0,   0,   0,   0,   0,   0,   0,   0,   0,   1,   0,   0,   0},
{  0,   0,   0,   0,   1,   0,   0,   0,   0,   0,   0,   0,   0,   1,   0,   0,   0,   0},
{  0,   0,   0,   0,   0,   1,   0,   0,   0,   0,   0,   0,   1,   0,   0,   0,   0,   0},
{  0,   0,   0,   0,   0,   0,   1,   0,   0,   0,   0,   1,   0,   0,   0,   0,   0,   0},
{  0,   0,   0,   0,   0,   0,   0,   1,   0,   0,   1,   0,   0,   0,   0,   0,   0,   0},
{  0,   0,   0,   0,   0,   0,   0,   0,   1,   1,   0,   0,   0,   0,   0,   0,   0,   0}}


\begin{pmatrix}
2& 1& 0\\
0& 1& 2\\
1& 1& 1\\
2& 0& 0\\
0& 1& 1\\
1& 0& 0
\end{pmatrix}

==> Proberen/name.tex <==
1  &  1 &  1 &  3& 3& 3& 5& 5& 5& 7& 7& 7& 9& 9& 9& 11& 11& 11& 13& 13& 13& 15& 15& 15& 17&
2  &  2 &  4 &  6& 6& 8& 10& 10& 12& 14& 14& 16& 18& 18& 20& 22& 22& 24& 26& 26& 28& 30& 30& 32& 34 &
1  &  3 &  5 &  7& 9& 11& 13& 15& 17& 19& 21& 23& 25& 27& 29& 31& 33& 35& 37& 39& 41& 43& 45& 47& 49 &
2  &  6 &  8 &  10& 14& 16& 18& 22& 24& 26& 30& 32& 34& 38& 40& 42& 46& 48& 50& 54& 56& 58& 62& 64& 66 &
1  &  5 &  9 &  11& 15& 19& 21& 25& 29& 31& 35& 39& 41& 45& 49& 51& 55& 59& 61& 65& 69& 71& 75& 79& 81 &
4  & 8& 12& 16& 20& 24& 28& 32& 36& 40& 44& 48& 52& 56& 60& 64& 68& 72& 76& 80& 84& 88& 92& 96& 100 &
3  & 7& 11& 17& 21& 25& 31& 35& 39& 45& 49& 53& 59& 63& 67& 73& 77& 81& 87& 91& 95& 101& 105& 109& 115 &
6  & 10& 16& 22& 26& 32& 38& 42& 48& 54& 58& 64& 70& 74& 80& 86& 90& 96& 102& 106& 112& 118& 122& 128& 134 &
3  & 9& 15& 21& 27& 33& 39& 45& 51& 57& 63& 69& 75& 81& 87& 93& 99& 105& 111& 117& 123& 129& 135& 141& 147 &
6  & 14& 20& 26& 34& 40& 46& 54& 60& 66& 74& 80& 86& 94& 100& 106& 114& 120& 126& 134& 140& 146& 154& 160& 166 &
3  & 11& 19& 25& 33& 41& 47& 55& 63& 69& 77& 85& 91& 99& 107& 113& 121& 129& 135& 143& 151& 157& 165& 173& 179 &
8  & 16& 24& 32& 40& 48& 56& 64& 72& 80& 88& 96& 104& 112& 120& 128& 136& 144& 152& 160& 168& 176& 184& 192& 200 &
5  & 13& 21& 31& 39& 47& 57& 65& 73& 83& 91& 99& 109& 117& 125& 135& 143& 151& 161& 169& 177& 187& 195& 203& 213 &
10 & 18& 28& 38& 46& 56& 66& 74& 84& 94& 102& 112& 122& 130& 140& 150& 158& 168& 178& 186& 196& 206& 214& 224& 234 &
5  & 15& 25& 35& 45& 55& 65& 75& 85& 95& 105& 115& 125& 135& 145& 155& 165& 175& 185& 195& 205& 215& 225& 235& 255 


 0& 0& 2& 0& 0& 2& 0& 0& 2& 0& 0& 2& 0& 0& 2& 0& 0& 2& 0& 0& 2& 0& 0& 2 \\
 0& 2& 2& 0& 2& 2& 0& 2& 2& 0& 2& 2& 0& 2& 2& 0& 2& 2& 0& 2& 2& 0& 2& 2 \\
 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2& 2 \\
 4& 2& 2& 4& 2& 2& 4& 2& 2& 4& 2& 2& 4& 2& 2& 4& 2& 2& 4& 2& 2& 4& 2& 2 \\
 4& 4& 2& 4& 4& 2& 4& 4& 2& 4& 4& 2& 4& 4& 2& 4& 4& 2& 4& 4& 2& 4& 4& 2 \\
 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4& 4 \\
 4& 4& 6& 4& 4& 6& 4& 4& 6& 4& 4& 6& 4& 4& 6& 4& 4& 6& 4& 4& 6& 4& 4& 6 \\
 4& 6& 6& 4& 6& 6& 4& 6& 6& 4& 6& 6& 4& 6& 6& 4& 6& 6& 4& 6& 6& 4& 6& 6 \\
 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6& 6 \\
 8& 6& 6& 8& 6& 6& 8& 6& 6& 8& 6& 6& 8& 6& 6& 8& 6& 6& 8& 6& 6& 8& 6& 6 \\
 8& 8& 6& 8& 8& 6& 8& 8& 6& 8& 8& 6& 8& 8& 6& 8& 8& 6& 8& 8& 6& 8& 8& 6 \\
 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8& 8 \\
 8& 8& 10& 8& 8& 10& 8& 8& 10& 8& 8& 10& 8& 8& 10& 8& 8& 10& 8& 8& 10& 8& 8& 10 \\
 8& 10& 10& 8& 10& 10& 8& 10& 10& 8& 10& 10& 8& 10& 10& 8& 10& 10& 8& 10& 10& 8& 10& 10 \\
 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 10& 20 
 
 
[[ 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0 & 1  ]&
  [ 0 & 1 & 1 & 0 & 1 & 1 & 0 & 1 & 1 & 0 & 1 & 1 & 0 & 1 & 1 & 0 & 1 & 1 & 0 & 1 & 1 & 0 & 1 & 1 ]&
  [ 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1  ]&
  [ 2 & 1 & 1 & 2 & 1 & 1 & 2 & 1 & 1 & 2 & 1 & 1 & 2 & 1 & 1 & 2 & 1 & 1 & 2 & 1 & 1 & 2 & 1 & 1 ]&
  [ 2 & 2 & 1 & 2 & 2 & 1 & 2 & 2 & 1 & 2 & 2 & 1 & 2 & 2 & 1 & 2 & 2 & 1 & 2 & 2 & 1 & 2 & 2 & 1  ]&
  [ 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 ]&
  [ 2 & 2 & 3 & 2 & 2 & 3 & 2 & 2 & 3 & 2 & 2 & 3 & 2 & 2 & 3 & 2 & 2 & 3 & 2 & 2 & 3 & 2 & 2 & 3  ]&
  [ 2 & 3 & 3 & 2 & 3 & 3 & 2 & 3 & 3 & 2 & 3 & 3 & 2 & 3 & 3 & 2 & 3 & 3 & 2 & 3 & 3 & 2 & 3 & 3 ]&
  [ 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3  ]&
  [ 4 & 3 & 3 & 4 & 3 & 3 & 4 & 3 & 3 & 4 & 3 & 3 & 4 & 3 & 3 & 4 & 3 & 3 & 4 & 3 & 3 & 4 & 3 & 3 ]&
  [ 4 & 4 & 3 & 4 & 4 & 3 & 4 & 4 & 3 & 4 & 4 & 3 & 4 & 4 & 3 & 4 & 4 & 3 & 4 & 4 & 3 & 4 & 4 & 3  ]&
  [ 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 ]&
  [ 4 & 4 & 5 & 4 & 4 & 5 & 4 & 4 & 5 & 4 & 4 & 5 & 4 & 4 & 5 & 4 & 4 & 5 & 4 & 4 & 5 & 4 & 4 & 5 ]]
  
  
  
  -1& 1& -2& 1& 1& 2\\-2& 4& -4& -2& 0& 4\\-2& 2& -2& 0& 0& 
  2\\2& -2& 4& 0& 0& -2\\2& -2& 4& 2& 0& -4\\3& -1& 
  2& -1& -1& -2

==> TODO.tex <==
\section{To-do}
\begin{enumerate}
    \item \st{Include Henrik's comment on the motivation for $\MD=\BD$. Ref:  \ref{subsection:motivationmd=bd}}
    \item \st{Personally acknowledge Henrik. En dan Isabelle en Maarten ook samen (apart) bedanken.}
    \item \st{Explain the names ``stuffle" and ``shuffle".}
    \item \st{Include the stuffle and shuffle formula between length $1$ MZVs.}
    \item \st{Incorporate the thesis' presentation `facts' into the thesis. (I.e. mono-brackets = divisor, etc).}
    \begin{enumerate}
        \item \st{$\ker(\zeta)$}=\dots.
        \item \st{Brackets = divisor generating function.}
    \end{enumerate}
    \item \st{Include the remark that dependent relations in length $3$ actually give relations in lower length.}
    \item \st{Talk about Magma.}
    \item Check EVERYTHING:
    \begin{enumerate}
        \item References.
        \item Lemma, Theorem, Proposition, Equation names \& internal references.
        \item Typos.
    \end{enumerate}
\end{enumerate}

==> Volgorde.tex <==



\begin{enumerate}
    \item Inleiding.
    \item MZV introductie. Definitie, wat eigenschappen ($\zeta(2,1)=\zeta(3)$.
    \item Shuffle/stuffle bij MZV.
    \item Bewijs MZV stuffle relatie, dit is natural (multiple harmonic sums).
    \item Bewijs shuffle relatie MZV (generalised polylogarithms).
    \begin{enumerate}
        \item iets over convergentie zeggen?
    \end{enumerate}
    \item Misschien: dualiteit.
    \item Monobrackets: $\MD$.
    \begin{enumerate}
        \item $\lim_{q\to 1}\MD$= MZV.
        \item $\MD$ heeft een stuffle relatie.
        \item $\MD$ heeft geen shuffle relatie.
        \item $\MD$ invariant onder $q\frac{d}{dq}$.
    \end{enumerate}
    \item Bibrackets $\BD$.
    \begin{enumerate}
        \item Shuffle relatie (m.b.v. partitie).
        \item 
    \end{enumerate}
    \item Vermoeden dat $\MD=\BD$. Bewijzen wat er al bekend is.
    \begin{enumerate}
        \item Voorbeelden.
        \item $\BD_{l=1}\subseteq \MD$.
        \item 
    \end{enumerate}
    \item Aanpak van eigen propositie. Dit bewijzen.
    \item Vermoedens over whats next.
\end{enumerate}


\noindent Nog gedaan worden:
\begin{enumerate}
    \item[4.] Geef het voorbeeld voor bijvoorbeeld $l=k=1$. Dat de methodes natuurlijk zijn.
    \item[]
\end{enumerate}

==> qZetabrackets.tex <==
We define the multiple q-zeta brackets to be the q-power (=FOUT) series
\begin{align*}
    \zbracket{s_1,\dots,s_l\\r_1,\dots,r_l}\coloneqq\sum_{\substack{m_1,\dots,m_l>0\\d_1,\dots,d_l>0}}\frac{m_1^{r_1-1}\cdots m_l^{r_l-1}}{(r_1-1)!\cdots (r_l-1)!}q^{(m_l+\dots+m_1)d_1+(m_l+\dots+m_2)d_2+\dots+m_ld_l}.
\end{align*}
And its generating series
\begin{align*}
    \zgen{X_1,\dots,X_l\\Y_1,\dots,Y_l}&=\sum_{\substack{s_1,\dots,s_l>0\\r_1,\dots,r_l>0}}\zbracket{s_1,\dots,s_l\\r_1,\dots,r_l}X_1^{s_1-1}\cdots X_l^{s_l-1}Y_1^{r_1-1}\cdots Y_l^{r_l-1}.
\end{align*}
\begin{lemma}
We have
\begin{align*}
    \zgen{X_1,\dots,X_l\\Y_1,\dots,Y_l}&=\sum_{m_1,\dots,m_l>0}\prod_{j=1}^l \frac{e^{m_jY_j}e^{X_j}q^{m_l+\dots+m_j}}{1-e^{X_j}q^{m_l+\dots+m_j}}\\
    &=\sum_{m_1,\dots,m_l>0}\prod_{j=1}^l E_{m_j}(Y_j)L_{m_l+\dots+m_j}(X_j),
\end{align*}
where 
\begin{equation*}
    E_n(X)\coloneqq e^{nX},\qquad\qquad L_n(X)\coloneqq \frac{e^Xq^n}{1-e^Xq^n}=\sum_{k>0}(e^Xq^n)^k.
\end{equation*}
\end{lemma}
\noindent\textbf{Example.} We have
\begin{align*}
    \zgen{X\\Y}&=\sum_{m>0}\frac{e^{mY}e^Xq^m}{1-e^Xq^m},\\
    \zgen{X_1,X_2\\Y_1,Y_2}&=\sum_{m_1,m_2>0}e^{m_1Y_1}e^{m_2Y_1}\frac{e^{X_1}q^{m_1+m_2}}{1-e^{X_1}q^{m_1+m_2}}\;\frac{e^{X_2}q^{m_2}}{1-e^{X_2}q^{m_2}}.
\end{align*}
\begin{lemma}
We have
\begin{align*}
    \zgen{X_1\\Y_1}\zgen{X_2\\Y_2}=\zgen{X_1\;,\;X_2\\Y_1, Y_1+Y_2}+\zgen{X_2\;,\;X_1\\Y_2, Y_1+Y_2}+\sum_{m>0}e^{m(Y_1+Y_2)}\frac{e^{X_1}q^m}{1-e^{X_1}q^m}\;\frac{e^{X_2}q^m}{1-e^{X_2}q^m}
\end{align*}
\end{lemma}
The lemma above states that, by putting $X_1=X_2=X$ and applying $\big(\frac{x}{1-x}\big)^2=\frac{x}{(1-x)^2}-\frac{x}{1-x}$, we obtain
\begin{align*}
    \zgen{X\\Y_1}\zgen{X\\Y_2}&=\zgen{X\;,\;X\\Y_1, Y_1+Y_2}+\zgen{X\;,\;X\\Y_2, Y_1+Y_2}+\sum_{m>0}e^{m(Y_1+Y_2)}\left(\frac{e^Xq^m}{1-e^Xq^m}\right)^2\\
    &=\zgen{X\;,\;X\\Y_1, Y_1+Y_2}+\zgen{X\;,\;X\\Y_2, Y_1+Y_2}-\zgen{X\\Y_1+Y_2}+\sum_{m>0}e^{m(Y_1+Y_2)}\frac{e^Xq^m}{(1-e^Xq^m)^2}.
\end{align*}

We have following identity regarding the last term:
\begin{align*}
    \frac{d}{dY_1}\sum_{m>0}e^{m(Y_1+Y_2)}\frac{e^Xq^m}{(1-e^Xq^m)^2}&=\sum_{m>0}me^{m(Y_1+Y_2)}\frac{e^Xq^m}{(1-e^Xq^m)^2}\\
    &=q\frac{d}{dq}\sum_{m>0}e^{m(Y_1+Y_2)}\frac{e^Xq^m}{1-e^Xq^m}\\
    &=q\frac{d}{dq}\zgen{X\\Y_1+Y_2}.
\end{align*}

\begin{align*}
    \zbracket{s_1\\r_1}\zbracket{s_2\\r_2}&=\sum_{k=0}^{r_2-1}{r_2-1+k\choose k}\zbracket{s_1,s_2\\r_1-k,r_2+k}+\sum_{k=0}^{r_1-1}{r_1-1+k\choose k}\zbracket{s_2,s_1\\r_2-k,r_1+k}\\
    &=\sum_{k=0}^{s_2-1}{s_2-1+k\choose k}\zbracket{s_2+k,s_1-k\\r_2,r_1}+\sum_{k=0}^{s_1-1}{s_1-1+k\choose k}\zbracket{s_1+k,s_2-k\\r_1,r_2}
\end{align*}
Dan is het systeem gelijk aan
\begin{align*}
    \begin{pmatrix}
    I_{S-1}\otimes T_{R-1}+I_{S-1}^\rho\otimes T_{R-1}^\rho\\
    \hline
    T_{S-1}^\sigma\otimes I_{R-1}^\sigma +T_{S-1}^{\sigma\rho}\otimes T_{R-1}^{\sigma\rho}
    \end{pmatrix},
\end{align*}
met
\begin{equation*}
    (T_N)_{i,j}={j-1\choose i-1}.
\end{equation*}





\newpage
The identity 
\begin{equation}
\label{eq:derbgen}
    \bgen{X\\Y_1}\bgen{X\\Y_2}=\bgen{X, X\\Y_1,Y_2}+\bgen{X,X\\Y_2,Y_1}-\bgen{X\\Y_1+Y_2}+\sum_{m>0}e^{m(Y_1+Y_2)}\frac{e^Xq^m}{(1-e^xq^m)^2}
\end{equation}
holds. By considering the case where $Y_1+Y_2=Y$, i.e. letting $Y_1=pY$ and $Y_2=(1-p)Y$, we obtain the formula
\begin{align*}
    \frac{1}{r+1}\cdot q\frac{d}{dq}\bbracket{s\\r}&=\bbracket{s\\r+1}+\sum_{k=1}^s\sum_{l=0}^{r+1}p^{r+1-l}(1-p)^{l}\bbracket{k\\l}\bbracket{s+1-k\\r+1-l}\\
    &\quad+\sum_{k=1}^s\sum_{l=0}^{r+1}\big(p^l(1-p)^{r+1-l}+(1-p)^lp^{r+1-l}\big)\bbracket{k,s+1-k\\l,r+1-l}.
\end{align*}
By taking the symmetric case $p=1/2$ the coefficients $p^{r+1-l}(1-p)^{l}$ and $$p^l(1-p)^{r+1-l}+(1-p)^lp^{r+1-l}$$ do not depend on $l$. We get
\begin{align*}
    q\frac{d}{dq}\bbracket{s\\r}&=(r+1)\bbracket{s\\r+1}-\frac{r+1}{2^r}\sum_{k=1}^{s}\sum_{l=0}^{r+1}\bbracket{k,s+1-k\\l,r+1-l}+\frac{r+1}{2^{r+1}}\sum_{k=1}^{s}\sum_{l=0}^{r+1}\bbracket{k\\l}\bbracket{s+1-k\\r+1-l}.
\end{align*}
Another identity, which arises from interpreting $d/dY\left(\bgen{X\\Y/2}\bgen{X\\Y/2}\right)$ in two different ways, is
\begin{equation*}
    (r+1)\sum_{k=1}^{s}\sum_{l=0}^{r+1}\bbracket{k\\l}\bbracket{s+1-k\\r+1-l}=2\sum_{k=1}^{s}\sum_{l=0}^{r+1}l\cdot\bbracket{k\\l}\bbracket{s+1-k\\r+1-l}.
\end{equation*}

Define the operator $D=\alpha \frac{d}{dY_1}+\beta \frac{d}{dY_2}$. Then we have
\begin{align*}
    D\bgen{X\\Y_1}&=D\sum_{s>0,r\geq0}\bbracket{s\\r}X^{s-1}Y_1^{r}\\
    &=\sum_{s_1>0,r_1\geq1}\alpha r_1\bbracket{s_1\\r_1}X^{s_1-1}Y_1^{r_1-1}\\
    &=\sum_{s_1>0,r_1\geq0}\alpha (r_1+1)\bbracket{s_1\\r_1+1}X^{s_1-1}Y_1^{r_1}.
\end{align*}

This gives
\begin{align*}
    \bgen{X\\Y_2}D\bgen{X\\Y_1}&=\sum_{\substack{s_1,s_2\\r_1,r_2}}\alpha(r_1+1)\bbracket{s_1\\r_1+1}X^{s_1+s_2-2}Y_1^{r_1}Y_2^{r_2},
\end{align*}
so that
\begin{align*}
    D\left(\bgen{X\\Y_1}\bgen{X\\Y_2}\right)&=\sum_{\substack{s_1,s_2\\r_1,r_2}}\left(\alpha(r_1+1)\bbracket{s_1\\r_1+1}\bbracket{s_2\\r_2}+\beta(r_2+1)\bbracket{s_1\\r_1}\bbracket{s_2\\r_2+1}\right)X^{s_1+s_2-2}Y_1^{r_1}Y_2^{r_2}.
\end{align*}
We also have
\begin{align*}
    D\bgen{X,X\\Y_1,Y_2}&=\sum_{\substack{s_1,s_2\\r_1,r_2}}\left(\alpha(r_1+1)\bbracket{s_1,s_2\\r_1+1,r_2}+\beta(r_2+1)\bbracket{s_1,s_2\\r_1,r_2+1}\right)X^{s_1+s_2-2}Y_1^{r_1}Y_2^{r_2}
\end{align*}
and
\begin{align*}
    D\bgen{X,X\\Y_2,Y_1}&=\sum_{\substack{s_2,s_1\\r_2,r_1}}\left(\alpha(r_2+1)\bbracket{s_2,s_1\\r_2+1,r_1}+\beta(r_1+1)\bbracket{s_2,s_1\\r_2,r_1+1}\right)X^{s_1+s_2-2}Y_1^{r_1}Y_2^{r_2}.
\end{align*}
We have
\begin{align*}
    D\bgen{X\\Y_1+Y_2}&=\sum_{s,r}\bbracket{s\\r+1}(\alpha+\beta)(r+1)X^{s-1}(Y_1+Y_2)^{r}.
\end{align*}
Finally, we have
\begin{align*}
    D\sum_{m>0}e^{m(Y_1+Y_2)}\frac{e^Xq^m}{(1-e^Xq^m)^2}=(\alpha+\beta)q\frac{d}{dq}\bgen{X\\Y_1+Y_2}.
\end{align*}
When we apply $D$ to (\ref{eq:derbgen}), and consider the coefficient at $X^{s-1}Y_1^{r_1}Y_2^{r_2}$ we obtain
\begin{align*}
    \alpha(r_1+1)\sum_{k=1}^{s}&\bbracket{k\\r_1+1}\bbracket{s+1-k\\r_2}+\beta(r_2+1)\sum_{k=1}^{s}\bbracket{k\\r_1}\bbracket{s+1-k\\r_2+1}=\\
    &\quad+\alpha(r_1+1)\sum_{k=1}^{s}\bbracket{k,s+1-k\\r_1+1,r_2}+\beta(r_2+1)\sum_{k=1}^{s}\bbracket{k,s+1-k\\r_1,r_2+1}+\\
    &\quad+\beta(r_2+1)\sum_{k=1}^{s}\bbracket{k,s+1-k\\r_2+1,r_1}+\alpha(r_1+1)\sum_{k=1}^{s}\bbracket{k,s+1-k\\r_2,r_1+1}+\\
    &\quad-(\alpha+\beta)(r_1+r_2+1){r_1+r_2\choose r_1}\bbracket{s\\r_1+r_2+1}+(\alpha+\beta){r_1+r_2\choose r_1}q\frac{d}{dq}\bbracket{s\\r_1+r_2}.
\end{align*}


% \begin{lemma}
% The stuffle product:
% \begin{align*}
%     \zbracket{s_1\\r_1}\zbracket{s_2\\r_2}&=\sum_{k=0}^{r_1-1}{r_2-1+k\choose k}\zbracket{s_1\;,\;s_2\\r_1-k,r_2+k}+\sum_{k=0}^{r_2-1}{r_1-1+k\choose k}\zbracket{s_2\;,\;s_1\\r_2-k,r_1+k}\\
%     &\quad+\dots\zbracket{l=1}\dots\\
% \intertext{and the shuffle product:}
%     &=\sum_{k=0}^{s_1-1}{s_2-1+k\choose k}\zbracket{s_2+k,s_1-k\\r_2\;,\;r_1}+\sum_{k=0}^{s_2-1}{s_1-1+k\choose k}\zbracket{s_1+k,s_2-k\\r_1\;,\;r_2}\\
%     &\quad+\dots\zbracket{l=1}\dots\\
% \end{align*}
% \end{lemma}

